A Latent Variable Model Approach to PMI-based Word Embeddings

Semantic word embeddings represent the meaning of a word via a vector, and are created by diverse methods. Many use nonlinear operations on co-occurrence statistics, and have hand-tuned hyperparameters and reweighting methods. This paper proposes a new generative model, a dynamic version of the log-linear topic model of~\citet{mnih2007three}. The methodological novelty is to use the prior to compute closed form expressions for word statistics. This provides a theoretical justification for nonlinear models like PMI, word2vec, and GloVe, as well as some hyperparameter choices. It also helps explain why low-dimensional semantic embeddings contain linear algebraic structure that allows solution of word analogies, as shown by~\citet{mikolov2013efficient} and many subsequent papers. Experimental support is provided for the generative model assumptions, the most important of which is that latent word vectors are fairly uniformly dispersed in space.

==> arxivjul22 copy/conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}
\vspace{-.05in}
%Our loglinear generative model can be seen as an analog of topic modeling that works well with the logarithm.
A simple generative model has been introduced to explain
the classical PMI based word embedding models, as well as recent variants involving
energy-based models and matrix factorization. The model yields an optimization objective with essentially \textquotedblleft no knobs to turn\textquotedblright, yet the embeddings lead to good 
performance on analogy tasks, and fit other predictions of our  generative model. A model with fewer knobs to turn should be seen as a better scientific explanation ({\em Occam's razor}), and certainly makes the embeddings more interpretable. 

The  spatial isotropy of word vectors is both an assumption in our model, and also a
new empirical finding of our paper. We feel it may help with further development of language models.  It is important for explaining the success of solving analogies via low dimensional 
vectors ({\sc relations=lines}). It also implies that semantic relationships among words manifest themselves as special directions among word embeddings (Section~\ref{sec:interpretability}), which lead to a cheater algorithm for solving analogy testbeds.
%We used this fact
%to design a \textquotedblleft cheating \textquotedblright way to do better on 
%current analogy testbeds which contains lessons for future design of testbeds ---no semantic relation should be tested more than %a few times.  

%The model and its analysis begin to unify diverse past work on word embeddings, including %disparate-looking ones such as VSMs and neural nets.
%As a side product it provides intuitive explanations for the success of analogy solvers, and begins %to provide new linear algebraic insight into word meanings. 


Our model is tailored to capturing semantic similarity, more akin to a log-linear dynamic topic model. In particular, local word order is unimportant. Designing similar generative models (with provable and
interpretable properties) with linguistic features is left for future work. 

\section*{Acknowledgements}

We thank the editors of TACL for granting a special relaxation of the page limit for our paper.  We thank Yann LeCun, Christopher D. Manning, and Sham Kakade for helpful
discussions at various stages of this work. 
%\Tnote{To check below} This was supported by the NSF, Simons Foundation,
%and Office of Naval Research. 

This work was supported in part by NSF grants %CCF-08327, 
%CCF-1117309, CCF-1302518, 
CCF-1527371, DMS-1317308, Simons Investigator Award, Simons Collaboration Grant,
and ONR-N00014-16-1-2329. Tengyu Ma was supported in addition by Simons Award in Theoretical Computer Science and IBM PhD Fellowship.

\iffalse 
Finally, we cannot resist returning to a philosophical question raised in Section~\ref{sec:related}: why logarithm? A priori, taking logs of word cooccurrences seems to interfere with capturing meaning. 
We think that taking log helps---as it does for the human brain for understanding sounds, visual signals, etc.---because {\em meaning} has high dynamic range. 
The frequent meaning of a word may be $1000$ times more common than an infrequent meaning. Taking logs seems to lead to representations where the dominant meaning does not swamp out the infrequent one. 
This can be explained to some extent in our theoretical model, but a more direct experiment is more illuminating:
we took pairs of unrelated words $w, w'$, where $w$ is $100$'s of times more common in the corpus than $w'$. 
Then we declared these to be a new word $w_{new}$, and trained a new vector for it using our method (while dropping the vectors for $v_w, v_w'$ and keeping all other word vectors unchanged). 
This new vector turns out to be something like $0.7 v_{w} + 0.2 v_{w'} + \mbox{noise}$: in other words, the infrequent meaning $w'$ has a significant component.

One wonders if such representation of meaning will have relevance to neuroscience---there is evidence that human and primate brains store frequencies internally on a logarithmic scale~\cite{buzsaki2014log}.

\fi 

==> arxivjul22 copy/cooccurence.tex <==

\section{Proofs of Theorem 1} \label{sec:proofmain}


In this section we prove Theorem~\ref{thm:main} and Lemma~\ref{thm:Z_c} (restated below). 

%\Anote{TODO: We should define $\mathcal{C}$ -- the uniform distribution over unit sphere  somewhere in the main body... } 
\begin{oneshot}{Theorem~\ref{thm:main}}
	Suppose the word vectors satisfy equation~\eqref{eqn:lem_zc}, and window size $q = 2$. Then, 
	%  \begin{eqnarray}
	%  \log p(w,w')   & = & \frac{\|v_w + v_{w'}\|_2^2 }{2d}- 2\log Z  \nonumber \\
	%	&& + \log \left(\frac{q(q-1)}{2}\right) \pm \epsilon,  \label{eqn:twowords_cooc} \\
	%  	\log p(w) & = & \frac{\nbr{v_{w}}_2^2}{2d}  - \log Z \pm \epsilon. \label{eqn:singleword}
	%  \end{eqnarray}
	\begin{align}
	\log p(w,w')   & =  \frac{\|v_w + v_{w'}\|_2^2 }{2d}- 2\log Z  \pm \epsilon,  \label{eqn:twowords_cooc_app} \\
	\log p(w) & =  \frac{\nbr{v_{w}}_2^2}{2d}  - \log Z \pm \epsilon. \label{eqn:singleword_app}
	\end{align}
	for $\epsilon = O(\epsilon_z) +\widetilde{O}(1/d) + O(\epsilon_2)$. %+\exp(-\Omega(\log^{1.8} n))$. 
	Jointly these imply: 
	%  \begin{equation}
	%   \mbox{PMI}~(w, w') = \frac{\langle v_w, v_{w'}\rangle}{d}  + \log \left(\frac{q(q-1)}{2}\right) \pm O(\epsilon). \label{eqn:PMI}
	%   \end{equation}
	\begin{equation}
	\mbox{PMI}~(w, w') = \frac{\langle v_w, v_{w'}\rangle}{d}  \pm O(\epsilon). \label{eqn:PMI_app}
	\end{equation}
%\end{thm}
\end{oneshot}

%Bearing in mind the generative model we just defined above, let's proceed to calculating the word-word co-occurrence probabilities. More precisely, our goal will be to show that up to an additive error which we'll explicitly bound, the word-word co-occurrence probabilities can be expressed in a form which is a special case of the form that the GloVe system attempts to fit. Since GloVe ends up only fitting the model up to some non-negligible error, this will offer some explanation for it's success.  

%B %y definition of our HMM model, the word-word co-occurrence can be computed by first marginalizing over $C_t,C_{t+1}$ and then decomposing using the conditional independence as defined in the HMM, 

%%\begin{align}
%& \Pr[W_t = w,W_{t+1} = w'] \nonumber\\& = \sum_{c,c'}\Pr(C_{t+1} = c'|C_t=c)\Pr(c)\Pr[W_t = w\mid C_t  = c]\Pr[W_{t+1} = w' \mid C_{t+1} = c']  \nonumber \\
%& = \sum_{c,c'}\Pr(C_{t+1} = c'|C_t=c)\Pr(c)\frac{\expinner{v_w,c}}{Z_c}\frac{\expinner{v_w,c'}}{Z_{c'}}   \label{eqn:factorize}%&= \sum_{c,c'} \Pr[W_t = w,W_{t+1} = w', C_t = c, C_{t+1} = c']\nonumber\\
% %&= \sum_{c,c'} \Pr[W_t = w\mid C_t  = c]\Pr[W_{t+1} = w' \mid C_{t+1} = c'] \Pr[C_t = c, C_{t+1} = c'] \nonumber\\
% % &= \sum_{c,c'} \Pr[W_t = w\mid C_t  = c]\Pr[W_{t+1} = w' \mid C_{t+1} = c'] \Pr[C_t = c]\Pr[C_{t+1} = c'\mid C_t] \label{eqn:factorize}
% %& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
% %& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
%\end{align}


%We prove that this mysterious log word-word cooccurrence is  approximately proportional to $\| v_w+v_{w'}\|^2$, and it follows that the ground truth PMI is approximately $\langle v_w, v_{w'}\rangle$. The key to understanding this is to show that the partition function $Z_c$ is approximately the same for all contexts $c$.  %so that 

%\begin{thm}\label{thm:Z_c}
%	There exists $Z$ such that for any fixed context $c$, with high probability $(1-4\exp(-d ^{0.8}))$ over the choice of $v_w$'s we have that 
%	
%	$$(1-\epsilon_z)Z\le Z_c\le (1+\epsilon_z) Z $$%\ge 1 - 2e^{- 2n^{0.4}}$$
%	with $\epsilon_z  = o(1)$.
%\end{thm}

%The proof essentially uses the facts that $c$ is uniformly bounded vector and $Z_c$ is a sum of exponential forms over the random generated words, and therefore concentrated around its mean. The full proof is deferred to Section~\ref{sec:zc}. 

%Actually, we will care about the logarithm of the above values. As is, the expression above is still too opaque so we will make a sequence of transformations that don't change it's value too much, but are much more transparent. 

%For notational convenience, let $\Delta(v, v')$ denote the $l_0$ distance between two vectors $v,v'$. 

%First, we show that the above expression can be well approximated by a situation where two words are emitted from each context. More formally: 
%Even though we this formula looks crazy, (It is a sum of products that involve partition function), we show that under our assumption, $\log( \Pr[W_t = w,W_{t+1} = w'])$ is indeed of certain ``linear" form approximately, which can be fitted by SDP programming and which justifies our choice of objective. 
%\begin{thm}
%\label{l:pairs} 
%
%Assuming that $C_t$ is at stationary distribution $\mathcal{C}$,  we have that 
%% is large enough so that the markov chain is at stationary distribution, we have 
%
%%Suppose that for all the partition constants, $Z_c \leq (1+\epsilon_z) Z$ and $Z_c \geq (1-\epsilon_z) Z$ holds; furthermore, suppose that assumptions \emph{1-3} hold.  Then, 
%%\[
%%	   \abr{ \log \rbr{\Pr[W_t = w,W_{t+1} = w'] }- \frac{p}{2d} \nbr{v_{w} + v_{w'}}_2^2  + 2\log(Z)  } \leq O(\frac{p}{d^2} \nbr{v_{w}+v_{w'}}_4^4) + 2\epsilon_z + 2\epsilon_2 + O(\epsilon^2_z) + O(\epsilon^2_2).
%%\]
%\begin{align*}
%	\log \Pr[W_{t}=w, W_{t+1} = w'] %&= \sum_{c,c'} \Pr[W_t = w,W_{t+1} = w', C_t = c, C_{t+1} = c']\nonumber\\
%	%&= \sum_{c,c'} \Pr[W_t = w\mid C_t  = c]\Pr[W_{t+1} = w' \mid C_{t+1} = c'] \Pr[C_t = c, C_{t+1} = c'] \nonumber\\
%	%&= \log\left( \sum_{c}\expinner{v_w,\tilde{v}_c}p(c)A(c,c')\right) - 2\log Z + \log(1\pm \epsilon_z)\\
%	%& = \log\left( \sum_{c}\expinner{v_w,\tilde{v}_c}p(c)(1\pm \epsilon_2)\expinner{v_{w'},\tilde{v}_{c}}\right) - 2\log Z + \log(1\pm \epsilon_z)\\
%	%& = \log\left( \sum_{c}\expinner{v_w,\tilde{v}_c}p(c)\expinner{v_{w'},\tilde{v}_{c}}\right) - 2\log Z + \log(1\pm \epsilon_z) + \log(1\pm \epsilon_2)\\
%	%& = \log\left( \sum_{c}\expinner{v_w+v_{w'},\tilde{v}_c}p(c)\right) - 2\log Z + \log(1\pm \epsilon_z) + \log(1\pm \epsilon_2)\\
%	%& = \log\left( \Exp_{\tilde{v}_c}[\expinner{v_w+v_{w'},\tilde{v}_c}]\right) - 2\log Z + \log(1\pm \epsilon_z) + \log(1\pm \epsilon_2)\\
%	%&  = (1 \pm \delta)\|v_w + v_{w'}\|^2/(2d) - 2\log Z \pm 3\epsilon_z\pm \epsilon_2\\
%	&  = (1 \pm \delta)\|v_w + v_{w'}\|^2/(2d) - 2\log Z \pm 3\epsilon_z\pm \epsilon_2 \pm o(1)\\
%	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
%	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
%	%&= \log\left( \sum_{c}\expinner{v_w,\tilde{v}_c}p(c)\sum_{c'}\expinner{v_{w'},v_{c'}} p(c'\vert c)\right) - 2\log Z + \log(1\pm \epsilon_z)
%\end{align*}
%with $\delta = o(1)$, $\epsilon_z = o(1)$, and $\epsilon_2$ as defined in the model assumption. 
%%with $\delta =  d^{-0.6}, %\epsilon_z = o(1)$, and $\epsilon_2$ as defined in assumption ??. 
%\end{thm}
%\Tnote{I am not sure how to state $C_t$ is at stationary distribution}

%\Tnote{The proof is a bit long. So we can extract certain part of the proof out to a separate lemma. But this theorem is the main theorem that we want to present. Treat other lemmas as techincal lemma. }
\begin{oneshot}{Lemma~\ref{thm:Z_c}}
	%\begin{thm}\label{thm:Z_c}
		If the word vectors satisfy the bayesian prior $v =  s \cdot \hat{v}$, where $\hat{v}$ is from the spherical Gaussian distribution, and $s$ is a scalar random variable, then with high probability the entire
		ensemble of word vectors satisfies that
		\begin{equation}
		\Pr_{c\sim \mathcal{C}}\left[(1-\epsilon_z)Z\le Z_c\le (1+\epsilon_z) Z\right]\ge 1-\delta \label{eqn:lem_zc_app},
		\end{equation}
		%for any fixed unit vector $c\in \R^d$,  with probability $1-\exp(-\Omega(\log^2 n))$ over the choices of $v_w$'s, we have
		%Let $Z = \Exp[\exp(\inner{v_w,c})\mid |\inner{v_w}{c}| < \frac{1}{2}\log n] $
		%	
		%	
		%	Suppose $\sqrt{n} > d > n^{.01}$, there exists $Z$ such that for any context $c$ with $|\|c\| - 1| \le d^{-0.4}$ , with probability $1-\exp(-\Omega(\log^2 n))$ over the choice of $v_w$'s, 
		%	\begin{eqnarray}
		%	(1-\epsilon_z)Z\le Z_c\le (1+\epsilon_z) Z\label{eqn:lem_zc}, 
		%	\end{eqnarray}
		for $\epsilon_z = \widetilde{O}(1/\sqrt{n})$, and $\delta = \exp(-\Omega(\log^2 n)) $.
\end{oneshot}



%Note that for typical choice of $v_w$ and $v_{w'}$, $\|v_w + v_{w'}\|^2/d = \Theta(1)$, and $\epsilon_z, \epsilon_2 = o(1)$. 

We first prove Theorem~\ref{thm:main} using Lemma~\ref{thm:Z_c}, and Lemma~\ref{thm:Z_c} will be proved in Section~\ref{sec:zc}. Please see Section~\ref{sec:model} of the main paper for the intuition of the proof and a cleaner sketch without too many technicalities. 
\begin{proof}[Proof of Theorem~\ref{thm:main}]

Let $c$ be the hidden discourse that determines the probability of word $w$, and $c'$ be the next one that determines $w'$. We use $p(c'\vert c)$ to denote the Markov kernel (transition matrix) of the Markov chain.  Let $\mathcal{C}$ be the stationary distribution of discourse vector $c$, and $\mathcal{D}$ be the joint distribution of $(c,c')$. 
We marginalize over the contexts $c,c'$ and then use the independence of $w,w'$ conditioned on $c,c'$, 


\begin{equation}
p(w,w') = \Exp_{(c,c')\sim \mathcal{D}}\left[\frac{\expinner{v_w,c}}{Z_c}\frac{\expinner{v_{w'},c'}}{Z_{c'}}\right]\label{eqn:eqn20}\end{equation}

	
We first get rid of the partition function $Z_c$ using Lemma~\ref{thm:Z_c}. As sketched in the main paper, essentially we will replace $Z_c$ by $Z$ in equation~\eqref{eqn:eqn20}, though a very careful control of the approximation error is required. Formally, 
Let $\mathcal{F}_1$ be the event that $c$ satisfies
\begin{equation}
	(1-\epsilon_z)Z\le Z_c\le (1+\epsilon_z)Z\,.\label{eqn:inter10}
\end{equation} Similarly, let $\mathcal{F}_2$ be the even that $c'$ satisfies	$(1-\epsilon_z)Z\le Z_{c'}\le (1+\epsilon_z)Z$, and let $\mathcal{F} = \mathcal{F}_1\cap \mathcal{F}_2$, and $\overline{\mathcal{F}}$ be its negation. Moreover, let $\mathbf{1}_{\mathcal{F}}$ be the indicator function for the event $\mathcal{F}$. Therefore by Lemma~\ref{thm:Z_c} and union bound, we have $\Exp[\mathbf{1}_{\mathcal{F}}] = \Pr[\mathcal{F}] \ge 1-\exp(-\Omega(\log^2 n))$.  %where $(1-\epsilon_z)Z\le Z_c\le (1+\epsilon_z)Z$ and $\set{C}_2 = \set{C}_1^c$. 
%Note that $\Pr[c \in \set{C}_2] \le 2 e^{- 2n^{0.4}}$. 

We first decompose the integral (\ref{eqn:eqn20}) into the two parts according to whether event $\mathcal{F}$ happens, 

\begin{align}
p(w,w') \nonumber%&= \sum_{c,c'} \Pr[W_t = w,W_{t+1} = w', C_t = c, C_{t+1} = c']\nonumber\\
%&= \sum_{c,c'} \Pr[W_t = w\mid C_t  = c]\Pr[W_{t+1} = w' \mid C_{t+1} = c'] \Pr[C_t = c, C_{t+1} = c'] \nonumber\\
&=  \Exp_{(c,c')\sim \mathcal{D}}\left[ \frac{1}{Z_cZ_{c'}}\expinner{v_w,c}\expinner{v_{w'},c'} \mathbf{1}_{\mathcal{F}}\right]
\nonumber\\
& + \Exp_{(c,c')\sim \mathcal{D}}\left[\frac{1}{Z_cZ_{c'}}\expinner{v_w,c}\expinner{v_{w'},c'}\mathbf{1}_{\overline{\mathcal{F}}}\right]
\label{eqn:inter3}
%& \le (1+\epsilon_z)^2 \frac{1}{Z^2} \int_{c,c'}\expinner{v_w,c}\expinner{v_{w'},c'} p(c)p(c'\vert c)\mathbf{1}_{\mathcal{F}}dcdc' + \Pr[\overline{\mathcal{F}}]\cdot \exp()
%	\frac{2 \exp(4 \kappa \sqrt{d} - 2 n^{0.4})}{n^2} 
%& \le (1+\epsilon_z)^2 \frac{1}{Z^2} \int_{c,c'}\expinner{v_w,c}\expinner{v_{w'},c'} p(c)p(c'\vert c)\mathbf{1}_{\mathcal{F}}dcdc' + \frac{2 \exp(4 \kappa \sqrt{d} - 2 n^{0.4})}{n^2} 
%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
\end{align}
%\begin{align}
%	p(w,w') \nonumber%&= \sum_{c,c'} \Pr[W_t = w,W_{t+1} = w', C_t = c, C_{t+1} = c']\nonumber\\
%	%&= \sum_{c,c'} \Pr[W_t = w\mid C_t  = c]\Pr[W_{t+1} = w' \mid C_{t+1} = c'] \Pr[C_t = c, C_{t+1} = c'] \nonumber\\
%	&=  \int_{c,c'}\frac{1}{Z_cZ_{c'}}\expinner{v_w,c}\expinner{v_{w'},c'} p(c)p(c'\vert c)\mathbf{1}_{\mathcal{F}}dcdc'
%	\nonumber\\
%	& + \int_{c,c'} \frac{1}{Z_cZ_{c'}}\expinner{v_w,c}\expinner{v_{w'},c'} p(c)p(c'\vert c)\mathbf{1}_{\overline{\mathcal{F}}}dcdc'
%	\label{eqn:inter3}
%	%& \le (1+\epsilon_z)^2 \frac{1}{Z^2} \int_{c,c'}\expinner{v_w,c}\expinner{v_{w'},c'} p(c)p(c'\vert c)\mathbf{1}_{\mathcal{F}}dcdc' + \Pr[\overline{\mathcal{F}}]\cdot \exp()
%%	\frac{2 \exp(4 \kappa \sqrt{d} - 2 n^{0.4})}{n^2} 
%	%& \le (1+\epsilon_z)^2 \frac{1}{Z^2} \int_{c,c'}\expinner{v_w,c}\expinner{v_{w'},c'} p(c)p(c'\vert c)\mathbf{1}_{\mathcal{F}}dcdc' + \frac{2 \exp(4 \kappa \sqrt{d} - 2 n^{0.4})}{n^2} 
%	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
%	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
%\end{align}
We bound the first quantity on the right hand side using (\ref{eqn:lem_zc}) and the definition of $\mathcal{F}$. 
%Note that all the quantities in the integrals are nonnegative, therefore, using $Z_c \ge n$ and 
\newcommand{\superexp}[1]{\Exp_{(c,c')\sim \mathcal{D}}\left[#1\right]}
\newcommand{\littleexp}[1]{\Exp\left[#1\right]}
\newcommand{\outexpc}[1]{\Exp_{c}\left[#1\right]}
\newcommand{\outexpcp}[1]{\Exp_{c'}\left[#1\right]} 
\newcommand{\innerexpc}[1]{\Exp_{c' \mid c}\left[#1\right]} 
\newcommand{\innerexpcp}[1]{\Exp_{c \mid c'}\left[#1\right]}
\begin{align}
	& \Exp_{(c,c')\sim \mathcal{D}}\left[\frac{1}{Z_cZ_{c'}}\expinner{v_w,c}\expinner{v_{w'},c'} \mathbf{1}_{\mathcal{F}}\right]\nonumber \\
	& \le (1+\epsilon_z)^2 \frac{1}{Z^2} \superexp{\expinner{v_w,c}\expinner{v_{w'},c'} \mathbf{1}_{\mathcal{F}}}\label{eqn:inter1}
\end{align}
For the second quantity of the right hand side of~\eqref{eqn:inter3}, we have by Cauchy-Schwartz, 
\begin{align}
	&\left(\superexp{\frac{1}{Z_cZ_{c'}}\expinner{v_w,c}\expinner{v_{w'},c'} \mathbf{1}_{\overline{\mathcal{F}}}}\right)^2\nonumber\\
	& \le \left(\superexp{\frac{1}{Z_c^2}\expinner{v_w,c}^2\mathbf{1}_{\overline{\mathcal{F}}}}\right)\left(\superexp{\int_{c,c'} \frac{1}{Z_{c'}^2}\expinner{v_{w'},c'}^2\mathbf{1}_{\overline{\mathcal{F}}} }\right)\nonumber\\
	%& \le \left(\littleexp{\frac{1}{Z_c^2}\expinner{v_w,c}^2\Exp[\mathbf{1}_{\overline{\mathcal{F}}}\mid c]}\right)\left(\Exp\left[{ \frac{1}{Z_{c'}^2}\expinner{v_{w'},c'}^2\Exp[\mathbf{1}_{\overline{\mathcal{F}}} \mid c']}\right]\right)\label{eqn:eqn9}
	& \le \left(\outexpc{\frac{1}{Z_c^2}\expinner{v_w,c}^2\innerexpc{\mathbf{1}_{\overline{\mathcal{F}}}}}\right)\left(\outexpcp{ \frac{1}{Z_{c'}^2}\expinner{v_{w'},c'}^2\innerexpcp{\mathbf{1}_{\overline{\mathcal{F}}}}}\right)\,.\label{eqn:eqn9}
%	& = \left(\int_{c} \frac{1}{Z_c^2}\expinner{v_w,c}^2p_1(c)dc\right)\left(\int_{c'} \frac{1}{Z_{c'}^2}\expinner{v_{w'},c'}^2p_2(c')dc'\right)\label{eqn:eqn9}
\end{align}
%
%\Anote{ The notation in \ref{eqn:eqn9} is a little unclear. Maybe change the expectations to be $\Exp_{c}$ and $\Exp_{c'}$ so it's clear with respect to what,  and change the expectation of the indicator $\mathbf{1}_{\overline{\mathcal{F}}}$ to a probability?}

%\Tnote{Sure. Though this is standard notation I guess. (One needs to write $\Exp_{c\mid c'}$ for the inner expectation otherwise). I am fine with using probability but please have another line -- it's not so clear to get a probability notation directedly.. }
%where at the last line we defined $p_1(c) = \int_{c'}p(c)p(c'|c)\indicator{\overline{\mathcal{F}}}dc'\le p(c)$, and $p_2(c') = \int_{c}p(c)p(c|c')\indicator{\overline{\mathcal{F}}}dc \le p(c')$.  We note that $\int p_1(c) dc = \int p(c,c')\indicator{\overline{\mathcal{F}}}dcdc' = \Pr[\overline{\mathcal{F}}] \le \Pr[\overline{\mathcal{F}}_1] + \Pr[\overline{\mathcal{F}}_2]\le \exp(-\Omega(\log^2n)). $ Similarly we have $\int_{c'} p_2(c')dc' \le \exp(-\Omega(\log^2n))$. 

Using the fact that $Z_c\ge 1$, then we have that 
\begin{equation*}
\outexpc{\frac{1}{Z_c^2}\expinner{v_w,c}^2\innerexpc{\mathbf{1}_{\overline{\mathcal{F}}}}}\le \outexpc{\expinner{v_w,c}^2\innerexpc{\mathbf{1}_{\overline{\mathcal{F}}}}} 
\end{equation*}

We can split that expectation as 
\begin{equation}
\Exp_c \left[\expinner{v_w,c}^2 \mathbf{1}_{\langle v_w,c \rangle > 0}\ \innerexpc{\mathbf{1}_{\overline{\mathcal{F}}}} \right] + \Exp_c \left[ \expinner{v_w,c}^2 \mathbf{1}_{\langle v_w,c \rangle < 0} \innerexpc{\mathbf{1}_{\overline{\mathcal{F}}}}\right]\,.\label{eqn:eqn21}
\end{equation}
The second term of (\ref{eqn:eqn21}) is upper bounded by 
$$\Exp_{c,c'} [\mathbf{1}_{\overline{\mathcal{F}}}]\le \exp(-\Omega(\log^2 n))$$ 
We proceed to the first term of (\ref{eqn:eqn21}) and observe the following property of it:
$$ \Exp_c \left[\expinner{v_w,c}^2 \mathbf{1}_{\langle v_w,c \rangle > 0}\ \innerexpc{\mathbf{1}_{\overline{\mathcal{F}}}} \right] \leq \Exp_c \left[\expinner{\alpha v_w,c}^2 \mathbf{1}_{\langle v_w,c \rangle > 0}\ \innerexpc{\mathbf{1}_{\overline{\mathcal{F}}}} \right] \leq \Exp_c \left[\expinner{\alpha v_w,c}^2 \innerexpc{\mathbf{1}_{\overline{\mathcal{F}}}} \right]$$
where $\alpha > 1$. Therefore, it's sufficient to bound
$$\Exp_c \left[\expinner{v_w,c}^2 \innerexpc{\mathbf{1}_{\overline{\mathcal{F}}}} \right] $$
when $\|v_w\| = \Omega(\sqrt{d})$.   

Let's denote by $z$ the random variable $2\inner{v_w}{c}$. %Using the fact that $Z_c\ge 1$, then we have that 
%\begin{equation}
%%\littleexp{\frac{1}{Z_c^2}\expinner{v_w,c}^2\Exp[\mathbf{1}_{\overline{\mathcal{F}}}\mid c]}\le \Exp\left[\expinner{v_w,c}^2\Exp[\mathbf{1}_{\overline{\mathcal{F}}}\mid c]\right] = \Exp\left[\exp(z)\Exp[\mathbf{1}_{\overline{\mathcal{F}}}\mid z]\right] 
%\outexpc{\frac{1}{Z_c^2}\expinner{v_w,c}^2\innerexpc{\mathbf{1}_{\overline{\mathcal{F}}}}}\le \outexpc{\expinner{v_w,c}^2\innerexpc{\mathbf{1}_{\overline{\mathcal{F}}}}} = %\Exp\left[\exp(z)\Exp[\mathbf{1}_{\overline{\mathcal{F}}}\mid z]\right] 
%\Exp_c\left[\exp(z)\Exp_{c' \mid z} [\mathbf{1}_{\overline{\mathcal{F}}}\mid z]\right] 
%%= \Exp\left[\expinner{v_w,c}^2r(c)\right] 
%%\le \int_{-\infty}^{\infty} \exp(z) q(z)dz 
%\label{eqn:eqn11}
%\end{equation}
%where $z = 2\inner{v_w}{c}$. 
%%where $q(z) = \int_c p_1(c)\mathbf{1}_{2\inner{v_w}{c} = z}dc$. We have that $q(z)$ has the property that $q(z)\le $ $\int_{-\infty}^{\infty} q(z) \le \exp(-\Omega(\log^2n))$
%%%where we  and $q(z) \le p(z)$ where $p(z)$ is the density of $z$. 

Let's denote %$r(z) = \Exp[\mathbf{1}_{\overline{\mathcal{F}}}\mid z]$ 
$r(z) = \Exp_{c' \mid z} [\mathbf{1}_{\overline{\mathcal{F}}}]$ 
which is a function of $z$ between $[0,1]$. We wish to upper bound $\Exp_c \left[\exp(z)r(z)\right]$. 
%We can split that expectation as 
%\begin{equation}
%\Exp_c \left[\exp(z)r(z) \mathbf{1}_{z \geq 0}\right] + \Exp_c \left[\exp(z)r(z)\mathbf{1}_{z < 0}\right]\,.\label{eqn:eqn21}
%\end{equation}
%The second term is upperbounded by 
%$$\Exp_c \left[r(z)\right] = \Exp_{c,c'} [\mathbf{1}_{\overline{\mathcal{F}}}]\le \exp(-\Omega(\log^2 n))$$ 
%We proceed to the first term in~\eqref{eqn:eqn21}, and observe the following property of it:
%$$ \Exp_c \left[\exp(z)r(z) \mathbf{1}_{z \geq 0}\right] \leq \Exp_c \left[\exp(\alpha z)r(z) \mathbf{1}_{z \geq 0}\right] \leq \Exp_c \left[\exp(\alpha z)r(z)\right]$$
%where $\alpha > 1$. Therefore, it's sufficient to bound $\Exp_c \left[\exp(z)r(z)\right]$ when $\|v_w\| = \Omega(\sqrt{d})$.  
The worst-case $r(z)$ can be quantified using a continuous version of Abel's inequality as proven in Lemma~\ref{lem:abel}, which gives 
\begin{equation}
%\Exp\left[\exp(z)\Exp[\mathbf{1}_{\overline{\mathcal{F}}}\mid z]\right]  = \Exp[\exp(z)r(z)]\le \Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right]
\Exp_c[\exp(z)r(z)]\le \Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right]
\end{equation}
%\begin{equation}
%\int_{-\infty}^{\infty}  \exp(z) q(z)dz \le \int_{-\infty}^{\infty}  \exp(z)p(z)\indicator{[t,+\infty]}(z)dz \label{eqn:eqn10}
%\end{equation}
where $t$ satisfies that %$\Exp[\mathbf{1}_{[t,+\infty]}] = \Pr[z\ge t] = \Exp[r(z)]$.
$\Exp_c[\mathbf{1}_{[t,+\infty]}] = \Pr[z\ge t] = \Exp_c[r(z)] \leq \exp(-\Omega(\log^2 n))$. %Note that $\Exp[r(z)]= \Exp[\mathbf{1}_{\overline{\mathcal{F}}}]\le \exp(-\Omega(\log^2 n))$. Then, we claim $\Pr[z\ge t] \le \exp(-\Omega(\log^2 n))$ implies that $t \ge \Omega(\log^{.9} n)$.
%Note that $\Exp_c[r(z)]= \Exp_{c,c'} [\mathbf{1}_{\overline{\mathcal{F}}}]\le \exp(-\Omega(\log^2 n))$. 
Then, we claim $\Pr[z\ge t] \le \exp(-\Omega(\log^2 n))$ implies that $t \ge \Omega(\log^{.9} n)$.
%Indeed, to draw a unit vector $c$ from $\mathcal{C}^n$ one can draw $n$ i.i.d. samples $\tilde{c}_i$ from a univariate Gaussian with mean 0 and variance $\frac{1}{n}$, and output $c = (\frac{\tilde{c}_1}{\|\tilde{c}\|}, \frac{\tilde{c}_2}{\|\tilde{c}\|}, \dots, \frac{\tilde{c}_n}{\|\tilde{c}\|})$. It holds that 
%\begin{equation*} 
%\Pr[2 \langle v_w, c \rangle  \geq t] = \Pr[2 \langle v_w, \frac{\tilde{c}}{\| \tilde{c} \|} \rangle \geq t] \geq \Pr[2 \langle v_w, \frac{\tilde{c}}{\| \tilde{c} \|} \rangle \geq t | \|\tilde{c} \| \geq \frac{1}{10}] \Pr[\tilde{c} \geq \frac{1}{10}]
%\end{equation*}   
%However, $\Pr[\|\tilde{c}\| \geq \frac{1}{10}]$ is lower bounded by a constant by Markov's inequality. Hence, 
%\begin{equation*}
%\Pr[2 \langle v_w, \frac{\tilde{c}}{\| \tilde{c} \|} \rangle \geq t | \|\tilde{c} \| \geq \frac{1}{10}] \geq 
%\end{equation*} 
%\Anote{Perhaps there's a way to do the next paragraph more cleanly... This is the simplest thing I could think of.}
%\Anote{The below two claims/lemmas require a lower bound on $\|v_w\|$ on the order of $\sqrt{d}$. Maybe it can be removed... The prior proof also seemed to need it. } 

If $c$ were distributed as $\mathcal{N}(0, \frac{1}{d} I)$, this would be a simple tail bound. However, as $c$ is distributed uniformly on the sphere, this requires special care, and the claim follows by applying Lemma \ref{l:sphericalangle} instead. 
%\Tnote{Let's have a separate lemma for things below}
%Then, by Lemma .... we have 
%
%
% so $\Pr[\frac{\tilde{c}_1}{\|\tilde{c}\|} \geq t \mid \|\tilde{c}\| \leq 100] \geq \Pr[\frac{\tilde{c}_1}{100} \ge \frac{\Omega(e^{-t^2})}{t}]$.      
%\Anote{Hm.. the above ends up needing that $\|v_w\|$ has reasonable norm, which is true whp, but maybe it's possible to write it in a cleaner way that doesn't require it. }
%\Tnote{Need to verify the bound for $t$, since $z$ is not simply a Gaussian distribution with variance 4. Note that $c$ is uniform distribution over the shpere. }
%\Anote{Looks easy, lower priority for now.} 
%$\int_t^{+\infty}p(z) \le \exp(-\Omega(\log^2 n))$. Note that $z= 2\inner{v_w}{c}$ is a random variable with standard deviation 2, and therefore $p(z) = \frac{1}{\sqrt{8\pi}} \exp(-\frac{1}{8}z^2)$, and we have that $t \ge \Omega(\log^{.9} n)$. Therefore, 
Finally, applying Corollary \ref{c:abelspherical}, we have: 
\begin{equation}
\Exp[\exp(z)r(z)]\le \Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right] = \exp(-\Omega(\log^{1.8}n))
\end{equation}
%\Anote{The above claim is no longer true: we only get $\exp(-\Omega(\log^{1.8}n)) + \exp(-\Omega(d))$. The latter term is $o(\frac{1}{d})$, so if we propagate that error, it should still  
%only add an $o(\frac{1}{d})$ error.}
%\Tnote{Need to verify equation above again since $z$ has a distribution that is close to Gaussian but not really}

%we use the fact that $Z_c\ge n$, combining equation~\eqref{eqn:eqn10}, ~\eqref{eqn:eqn11},~\eqref{eqn:eqn12}, we obtain that 
%\begin{equation}
%\int_{c} \frac{1}{Z_c^2}\expinner{v_w,c}^2p_1(c)dc \le \frac{1}{n^2}\exp(-\Omega(\log^{1.8}n))
%\end{equation}
%and $\expinner{v_w,c} \le \exp( 2\kappa \sqrt{d})$ (by assumption $\nbr{v_w} \le \kappa \sqrt{d}$ and $\nbr{c} \le 2$), and conclude
%\begin{align}
%%	p(w,w') %&= \sum_{c,c'} \Pr[W_t = w,W_{t+1} = w', C_t = c, C_{t+1} = c']\nonumber\\
%	%&= \sum_{c,c'} \Pr[W_t = w\mid C_t  = c]\Pr[W_{t+1} = w' \mid C_{t+1} = c'] \Pr[C_t = c, C_{t+1} = c'] \nonumber\\
%	%&\le (1+\epsilon_z)^2 \frac{1}{Z^2} \int_{c,c'}\expinner{v_w,c}\expinner{v_{w'},c'} p(c)p(c'\vert c)\mathbf{1}_{\mathcal{F}}dcdc'	
%	& \int_{c,c'} \expinner{v_w,c}\expinner{v_{w'},c'} p(c)p(c'\vert c)\mathbf{1}_{\overline{\mathcal{F}}}dcdc'\nonumber
%	\\
%	&\le \Pr[\overline{\mathcal{F}}]\cdot 
%	\exp(4 \kappa \sqrt{d}) \le \exp(-d^{0.7})\label{eqn:inter2}
%	%& \le (1+\epsilon_z)^2 \frac{1}{Z^2} \int_{c,c'}\expinner{v_w,c}\expinner{v_{w'},c'} p(c)p(c'\vert c)\mathbf{1}_{\mathcal{F}}dcdc' + \Pr[\overline{\mathcal{F}}]\cdot 
%	%\frac{2 \exp(4 \kappa \sqrt{d} - 2 n^{0.4})}{n^2} 
%	%& \le (1+\epsilon_z)^2 \frac{1}{Z^2} \int_{c,c'}\expinner{v_w,c}\expinner{v_{w'},c'} p(c)p(c'\vert c)\mathbf{1}_{\mathcal{F}}dcdc' + \frac{2 \exp(4 \kappa \sqrt{d} - 2 n^{0.4})}{n^2} 
%	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
%	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
%\end{align}
We have the same bound for $c'$ as well.  
%Then using~\eqref{eqn:eqn9} we obtain, 
%
%\begin{align}
%& \Exp_{(c,c')\sim \mathcal{D}}\left[\frac{1}{Z_cZ_{c'}}\expinner{v_w,c}\expinner{v_{w'},c'} \mathbf{1}_{\mathcal{F}}\right]\nonumber \\
%& \le (1+\epsilon_z)^2 \frac{1}{Z^2} \superexp{\expinner{v_w,c}\expinner{v_{w'},c'} \mathbf{1}_{\mathcal{F}}}\label{eqn:inter1}
%\end{align}
Hence, for the second quantity of the right hand side of~\eqref{eqn:inter3}, we have
\begin{align}
&\superexp{\frac{1}{Z_cZ_{c'}}\expinner{v_w,c}\expinner{v_{w'},c'} \mathbf{1}_{\overline{\mathcal{F}}}}\nonumber\\
%& \le \left(\superexp{\frac{1}{Z_c^2}\expinner{v_w,c}^2\mathbf{1}_{\overline{\mathcal{F}}}}\right)\left(\superexp{\int_{c,c'} \frac{1}{Z_{c'}^2}\expinner{v_{w'},c'}^2\mathbf{1}_{\overline{\mathcal{F}}} }\right)\nonumber\\
%& \le \left(\littleexp{\frac{1}{Z_c^2}\expinner{v_w,c}^2\Exp[\mathbf{1}_{\overline{\mathcal{F}}}\mid c]}\right)^{1/2}\left(\Exp\left[{ \frac{1}{Z_{c'}^2}\expinner{v_{w'},c'}^2\Exp[\mathbf{1}_{\overline{\mathcal{F}}} \mid c']}\right]\right)^{1/2}\nonumber\\
&\le \left(\outexpc{\frac{1}{Z_c^2}\expinner{v_w,c}^2\innerexpc{\mathbf{1}_{\overline{\mathcal{F}}}}}\right)^{1/2} \left(\outexpcp{ \frac{1}{Z_{c'}^2}\expinner{v_{w'},c'}^2\innerexpcp{\mathbf{1}_{\overline{\mathcal{F}}}}}\right)^{1/2} \nonumber\\ 
& \le \exp(-\Omega(\log^{1.8}n))
%	& = \left(\int_{c} \frac{1}{Z_c^2}\expinner{v_w,c}^2p_1(c)dc\right)\left(\int_{c'} \frac{1}{Z_{c'}^2}\expinner{v_{w'},c'}^2p_2(c')dc'\right)
\label{eqn:rhsbound}
\end{align}
%
%For the last inequality we use $\Pr[\overline{\mathcal{F}}] \le 4\exp( - d^{0.2}). $ 
where the first inequality follows from Cauchy-Schwartz, and the second from the calculation above. 
Combining (\ref{eqn:inter3}), (\ref{eqn:inter1}) and (\ref{eqn:rhsbound}), we obtain
%\Anote{Should the last referenced equation be really \ref{eqn:eqn13}? Looks to me it should be just the bound above.}
%\Tnote{Yes, please do. A lot of edit of this type should be done as well. } 

\begin{align*}
	p(w,w')%&= \sum_{c,c'} \Pr[W_t = w,W_{t+1} = w', C_t = c, C_{t+1} = c']\nonumber\\
	%&= \sum_{c,c'} \Pr[W_t = w\mid C_t  = c]\Pr[W_{t+1} = w' \mid C_{t+1} = c'] \Pr[C_t = c, C_{t+1} = c'] \nonumber\\
	&\le (1+\epsilon_z)^2 \frac{1}{Z^2} \superexp{\expinner{v_w,c}\expinner{v_{w'},c'} \mathbf{1}_{\overline{\mathcal{F}}}}+ \frac{1}{n^2}\exp(-\Omega(\log^{1.8}n))\nonumber\\
	%&\le (1+\epsilon_z)^2 \frac{1}{Z^2} \int_{c,c'}\expinner{v_w,c}\expinner{v_{w'},c'} p(c)p(c'\vert c)\mathbf{1}_{\mathcal{F}}dcdc' + \frac{1}{n^2}\exp(-\Omega(\log^{1.8}n))\\
	&\le (1+\epsilon_z)^2 \frac{1}{Z^2} \superexp{\expinner{v_w,c}\expinner{v_{w'},c'}} + \delta_0\nonumber\\
	%& \le (1+\epsilon_z)^2 \frac{1}{Z^2} \left(\int_{c,c'}\expinner{v_w,c}\expinner{v_{w'},c'} p(c)p(c'\vert c)dcdc' + \delta_0\right)
	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
\end{align*}

%$$ p(w,w') \le (1+\epsilon_z)^2 \frac{1}{Z^2} \superexp{\expinner{v_w,c}\expinner{v_{w'},c'} \mathbf{1}_{\overline{\mathcal{F}}}}+ \frac{1}{n^2}\exp(-\Omega(\log^{1.8}n)) $$
%$$ \le (1+\epsilon_z)^2 \frac{1}{Z^2} \superexp{\expinner{v_w,c}\expinner{v_{w'},c'}} + \delta_0 $$

%\Anote{Not sure where the $\frac{1}{n^2}$ cropped up from. Seems to me it should only be $\exp(-\Omega(\log^{1.8}n))$.}
%\Anote{Tengyu, did you verify the above? $\frac{1}{n^2}$ still seems extra.} 
where $\delta_0 = \exp(-\Omega(\log^{1.8}n))Z^2 \le \exp(-\Omega(\log^{1.8}n))$ by the fact that $Z \le \exp(2\kappa)n = O(n)$. Note that $\kappa$ is treated as an absolute constant throughout the paper. %This is because $Z \le \exp(2\kappa) n$ and $d = \omega(\log^2 n)$, 
On the other hand, we can lowerbound similarly
\begin{align*}
	p(w,w') %&= \sum_{c,c'} \Pr[W_t = w,W_{t+1} = w', C_t = c, C_{t+1} = c']\nonumber\\
	%&= \sum_{c,c'} \Pr[W_t = w\mid C_t  = c]\Pr[W_{t+1} = w' \mid C_{t+1} = c'] \Pr[C_t = c, C_{t+1} = c'] \nonumber\\
	%&\ge (1-\epsilon_z)^2 \frac{1}{Z^2} \int_{c,c'}\expinner{v_w,c}\expinner{v_{w'},c'} p(c)p(c'\vert c)\mathbf{1}_{\mathcal{F}}dcdc' \\
	&\ge (1-\epsilon_z)^2 \frac{1}{Z^2} \superexp{\expinner{v_w,c}\expinner{v_{w'},c'} \mathbf{1}_{\overline{\mathcal{F}}}} \\
	%&\ge (1-\epsilon_z)^2 \frac{1}{Z^2} \left(\int_{c,c'}\expinner{v_w,c}\expinner{v_{w'},c'} p(c)p(c'\vert c)dcdc'  -  \frac{1}{n^2}\exp(-\Omega(\log^{1.8}n))\right)\\
	&\ge (1-\epsilon_z)^2 \frac{1}{Z^2} \superexp{\expinner{v_w,c}\expinner{v_{w'},c'}}  -  \frac{1}{n^2}\exp(-\Omega(\log^{1.8}n))\\
	%&\ge (1-\epsilon_z)^2 \frac{1}{Z^2} \left(\int_{c,c'}\expinner{v_w,c}\expinner{v_{w'},c'} p(c)p(c'\vert c)dcdc'  - \delta_0\right)
	&\ge (1-\epsilon_z)^2 \frac{1}{Z^2} \superexp{\expinner{v_w,c}\expinner{v_{w'},c'}}  - \delta_0
	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
\end{align*}
Taking logarithm, the multiplicative error translates to a additive error 
\begin{align*}
	\log p(w,w') %&= \sum_{c,c'} \Pr[W_t = w,W_{t+1} = w', C_t = c, C_{t+1} = c']\nonumber\\
	%&= \sum_{c,c'} \Pr[W_t = w\mid C_t  = c]\Pr[W_{t+1} = w' \mid C_{t+1} = c'] \Pr[C_t = c, C_{t+1} = c'] \nonumber\\
	%&= \log\left( \int_{c,c'}\expinner{v_w,c}\expinner{v_{w'},c'} p(c)p(c'\vert c)dcdc' \pm \delta_0\right) - 2\log Z + 2\log(1\pm \epsilon_z) \\
	&= \log\left(  \superexp{\expinner{v_w,c}\expinner{v_{w'},c'}}  \pm \delta_0\right) - 2\log Z + 2\log(1\pm \epsilon_z) \\
	%& + \log \left( 1 \pm 2 \exp\left(8 \kappa \sqrt{d} - 2 n^{0.4} \right) \right)
	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
\end{align*}
For the purpose of exploiting the fact that $c,c'$ should be close to each other, we further rewrite $\log p(w,w')$ by re-organizing the expectations above,
\begin{align}
	\log p(w,w') %&= \sum_{c,c'} \Pr[W_t = w,W_{t+1} = w', C_t = c, C_{t+1} = c']\nonumber\\
	%&= \sum_{c,c'} \Pr[W_t = w\mid C_t  = c]\Pr[W_{t+1} = w' \mid C_{t+1} = c'] \Pr[C_t = c, C_{t+1} = c'] \nonumber\\
	&= \log\left( \Exp_c\left[\expinner{v_w,c}\Exp_{c' \mid c}[\expinner{v_{w'},c'}]\right]\pm \delta_0\right) - 2\log Z + 2 \log(1\pm \epsilon_z)\nonumber\\
	& = \log\left( \Exp_c\left[\expinner{v_w,c} A(c)\right]\pm \delta_0\right) - 2\log Z + 2 \log(1\pm \epsilon_z)\label{eqn:ac}
	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
	%&= \log\left( \sum_{c}\expinner{v_w,\tilde{v}_c}p(c)\sum_{c'}\expinner{v_{w'},v_{c'}} p(c'\vert c)\right) - 2\log Z + \log(1\pm \epsilon_z)
\end{align}
where the inner integral which is denoted by $A(c)$, 
$$A(c) := \Exp_{c' \mid c}\left[\expinner{v_{w'},c'}\right]$$
%\Tnote{Need a small fix here}
%Note that by Lemma~\ref{lem:bound}, 
Since $\|v_w\| \le \kappa\sqrt{d}$.  %and any pairs of $c,c'$,
 Therefore we have that $\langle v_{w},c- c'\rangle \le \|v_w\|\|c-c'\|\le \kappa\sqrt{d}\|c-c'\|$. 
 %\le 4\|w\|\|\tilde{v}_{c} - \tilde{v}_{c'}\|\log n/\sqrt{d}\le4\kappa\|\tilde{v}_{c} - \tilde{v}_{c'}\|\log n $. 
	
Then we can bound $A(c)$ by 


\begin{align*}
%A(c) &= \Exp\left[\expinner{v_{w'},c'} \mid c\right]	 \\
A(c) &= \Exp_{c' \mid c} \left[\expinner{v_{w'},c'}\right]	 \\
%& = \expinner{v_{w'},c}\Exp\left[\expinner{v_{w'},c'-c} \mid c\right]\\
& = \expinner{v_{w'},c}\Exp_{c' \mid c}\left[\expinner{v_{w'},c'-c}\right]\\
%&=\expinner{v_{w'},c}\int_{c'}\expinner{v_{w'},c'-c} p(c'\vert c)dc' \\
%& \le \expinner{v_{w'},c}\int_{c'}\exp(4\kappa|c'-c|_1\log n) p(c'\vert c) \\
& \le \expinner{v_{w'},c}\Exp_{c'|c}[\exp(\kappa\sqrt{d}\|c-c'\|)]\\
&\le (1+\epsilon_2)\expinner{v_{w'},c}
\end{align*}
where the last inequality follows from our model assumptions. To derive a lower bound of $A(c)$, observe that 

%$$\Exp_{p(c'|c)}[\exp(4\kappa|c'-c|_1\log n)] + \Exp_{p(c'|c)}[\exp(-4\kappa|c'-c|_1\log n)]\ge 2$$
$$\Exp_{c'|c}[\exp(\kappa\sqrt{d}\|c-c'\|)] + \Exp_{c'|c}[\exp(-\kappa\sqrt{d}\|c-c'\|)]\ge 2$$

Therefore, our model assumptions imply that 

%$$ \Exp_{p(c'|c)}[\exp(-4\kappa|c'-c|_1\log n)]\ge 1-\epsilon_2$$
$$ \Exp_{c'|c}[\exp(-\kappa\sqrt{d}\|c-c'\|)]\ge 1-\epsilon_2$$

Hence,  
\begin{align*}
	A(c) %&= \sum_{c'}\expinner{v_{w'},\tilde{v}_{c'}} p(c'\vert c) 	 \\
	%&=\expinner{v_{w'},c}\int_{c'}\expinner{v_{w'},c'-c} p(c'\vert c)dc' \\
	&=\expinner{v_{w'},c}\Exp_{c' \mid c}\expinner{v_{w'},c'-c} \\
	%& \ge \expinner{v_{w'},c}\int_{c'}\exp(-4\kappa\|c'-c\|\log n) p(c'\vert c) dc'\\
	& \ge \expinner{v_{w'},c}\Exp_{c' \mid c}\exp(-\kappa\sqrt{d}\|c-c'\|)\\
	%& = \expinner{v_{w'},c}\Exp_{p(c'|c)}[\exp(-4\kappa\|c'-c\|\log n)]\\
	&\ge (1-\epsilon_2)\expinner{v_{w'},c}
\end{align*}

Therefore, we obtain that $A(c) = (1\pm \epsilon_2)\expinner{v_{w'},c}$. Plugging the just obtained estimate of $A(c)$ into the equation ~\eqref{eqn:ac}, we get that 

%\begin{align*}
%	\log p(w,w') %&= \sum_{c,c'} \Pr[W_t = w,W_{t+1} = w', C_t = c, C_{t+1} = c']\nonumber\\
%	%&= \sum_{c,c'} \Pr[W_t = w\mid C_t  = c]\Pr[W_{t+1} = w' \mid C_{t+1} = c'] \Pr[C_t = c, C_{t+1} = c'] \nonumber\\
%	&= \log\left( \int_{c}\expinner{v_w,c}p(c)A(c) dc\pm \delta_0\right) - 2\log Z + 2 \log(1\pm \epsilon_z)\\
%	& = \log\left(\int_{c}\expinner{v_w,c}p(c)(1\pm \epsilon_2)\expinner{v_{w'},c} dc \pm \delta_0\right) - 2\log Z + 2 \log(1\pm \epsilon_z)\\
%		& = \log\left( \int_{c}\expinner{v_w,c}p(c)\expinner{v_{w'},c} dc\pm \delta_0\right) - 2\log Z + 2\log(1\pm \epsilon_z) + \log(1\pm \epsilon_2)\\
%		& = \log\left( \int_{c}\expinner{v_w+v_{w'},c}p(c) dc\pm \delta_0\right) - 2\log Z + 2\log(1\pm \epsilon_z) + \log(1\pm \epsilon_2)\\
%		& = \log\left( \Exp_{c\sim \mathcal{C}}[\expinner{v_w+v_{w'},c}]\pm \delta_0\right) - 2\log Z +2 \log(1\pm \epsilon_z) + \log(1\pm \epsilon_2)\\
%	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
%	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
%	%&= \log\left( \sum_{c}\expinner{v_w,\tilde{v}_c}p(c)\sum_{c'}\expinner{v_{w'},v_{c'}} p(c'\vert c)\right) - 2\log Z + \log(1\pm \epsilon_z)
%\end{align*}

\begin{align}
	\log p(w,w') %&= \sum_{c,c'} \Pr[W_t = w,W_{t+1} = w', C_t = c, C_{t+1} = c']\nonumber\\
	%&= \sum_{c,c'} \Pr[W_t = w\mid C_t  = c]\Pr[W_{t+1} = w' \mid C_{t+1} = c'] \Pr[C_t = c, C_{t+1} = c'] \nonumber\\
	&= \log\left( \Exp_c\left[\expinner{v_w,c}A(c)\right] \pm \delta_0\right) - 2\log Z + 2 \log(1\pm \epsilon_z)\nonumber\\
	& = \log\left(\Exp_{c}\left[(1 \pm \epsilon_2) \expinner{v_w,c}\expinner{v_{w'},c}\right] \pm \delta_0\right) - 2\log Z + 2 \log(1\pm \epsilon_z)\nonumber\\
	%& = \log\left(\Exp_{c}\left[\expinner{v_w,c}\expinner{v_{w'}}\right] \pm \delta_0\right) - 2\log Z + 2\log(1\pm \epsilon_z) + \log(1\pm \epsilon_2)\\
	& = \log\left(\Exp_{c}\left[\expinner{v_w+v_{w'},c}\right]\pm \delta_0\right) - 2\log Z + 2\log(1\pm \epsilon_z) + \log(1\pm \epsilon_2)\label{eqn:eqn19}
	%& = \log\left(\Exp_{c\sim \mathcal{C}}[\expinner{v_w+v_{w'},c}]\pm \delta_0\right) - 2\log Z +2 \log(1\pm \epsilon_z) + \log(1\pm \epsilon_2)\\
	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
	%&= \log\left( \sum_{c}\expinner{v_w,\tilde{v}_c}p(c)\sum_{c'}\expinner{v_{w'},v_{c'}} p(c'\vert c)\right) - 2\log Z + \log(1\pm \epsilon_z)
\end{align}



Now it suffices to compute $ \Exp_{c}[\expinner{v_w+v_{w'},c}]$. Note that if $c$ had the distribution $\mathcal{N}(0,\frac{1}{d}I)$, which is very similar to uniform distribution over the sphere,  then we could get straightforwardly 
$ \Exp_{c}[\expinner{v_w+v_{w'},c}] = \exp(\|v_w+v_{w'}\|^2/(2d))$.  For $c$ having a uniform distribution over the sphere, by Lemma~\ref{lem:helper1}, the same equality holds approximately, 

\begin{equation}
\Exp_{c}[\expinner{v_w+v_{w'},c}] = (1\pm \epsilon_3)\exp(\|v_w+v_{w'}\|^2/(2d)) \label{eqn:eqn18}
\end{equation}
where $\epsilon_3  = \widetilde{O}(1/d)$. 
%Let $t = v_{w} + v_{w'}$.


%\Tnote{Below here the new proof will require calculating  $ \Exp_{c\sim \mathcal{C}}[\expinner{v_w+v_{w'},c}]$ with $c$ being uniform over the sphere. It's not exactly clear how to prove do it but at least we can show that  $ \Exp_{c\sim \mathcal{C}}[\expinner{v_w+v_{w'},c}]$ is $1\pm 1/\sqrt{d}$ close to the case when $c$ is Gaussian.}
%\Anote{Have not touched this yet. } 
%
%By our assumption, $\mathcal{C}$ is a product distribution across the coordinates. Therefore we can write 
%
%$$\Exp_{c\sim \mathcal{C}}[\expinner{v_w+v_{w'},c}] = \prod_{i=1}^d \Exp_{c_i}\exp(t_ic_i)$$
%
%Using lemma~\ref{lem:moment} for $t_i c_i \le 1$( we used the fact that $t_i \le 8\kappa\log n$  for all $t = v_w + v_{w'}$, $c_i \le \frac{2}{\sqrt{d}}$ (see Lemma~\ref{lem:bound});  In our setting $\kappa$ is a constant, $d = \omega((\log n)^2)$), we can estimate $\Exp_{c_i}\exp(t_ic_i)$ by 
%
%$$\Exp_{c_i}\exp(t_ic_i) =  1+ \frac{t_i^2}{2d} + O(t_i^4/d^2)$$
%
%Using the fact that $ x - \frac{x^2}{2}\le \ln(1 + x) \le x$. 
%
%\begin{eqnarray*}
%\log \Exp_{_c}[\expinner{v_w+v_{w'},c}] &&=  \sum_{i=1}^d \log\Exp_{c_i}\exp(t_ic_i) =  \sum_{i=1}^d \log\left(1+ \frac{t_i^2}{2d} + O(t_i^4/d^2)\right) \\
%&& %=  \sum_{i=1}^d \log\Exp_{(\tilde{v}_{c})_i}\exp(t_i(\tilde{v}_c)_i) 
%=  \sum_{i=1}^d \frac{t_i^2}{2d} + O(t_i^4/d^2) \\%O(\frac{t_i^4}{d^2}) \\
%&& = \|t\|^2/(2d) + O(\|t\|_4^4/d^2) %+ %o(\|t\|^2/d + \|t\|_4^4/d^2) \\
%\end{eqnarray*}




Plugging in equation~\eqref{eqn:eqn18} into equation~\eqref{eqn:eqn19}, we have that 
\begin{align*}
	\log p(w,w') %&= \sum_{c,c'} \Pr[W_t = w,W_{t+1} = w', C_t = c, C_{t+1} = c']\nonumber\\
	%&= \sum_{c,c'} \Pr[W_t = w\mid C_t  = c]\Pr[W_{t+1} = w' \mid C_{t+1} = c'] \Pr[C_t = c, C_{t+1} = c'] \nonumber\\
	%&= \log\left( \sum_{c}\expinner{v_w,\tilde{v}_c}p(c)A(c,c')\right) - 2\log Z + \log(1\pm \epsilon_z)\\
	%& = \log\left( \sum_{c}\expinner{v_w,\tilde{v}_c}p(c)(1\pm \epsilon_2)\expinner{v_{w'},\tilde{v}_{c}}\right) - 2\log Z + \log(1\pm \epsilon_z)\\
	%& = \log\left( \sum_{c}\expinner{v_w,\tilde{v}_c}p(c)\expinner{v_{w'},\tilde{v}_{c}}\right) - 2\log Z + \log(1\pm \epsilon_z) + \log(1\pm \epsilon_2)\\
	%& = \log\left( \sum_{c}\expinner{v_w+v_{w'},\tilde{v}_c}p(c)\right) - 2\log Z + \log(1\pm \epsilon_z) + \log(1\pm \epsilon_2)\\
	& = \log\left(  (1\pm \epsilon_3)\exp(\|v_w+v_{w'}\|^2/(2d)) \pm \delta_0 \right)- 2\log Z + 2\log(1\pm \epsilon_z) + \log(1\pm \epsilon_2)\\
	&  = \|v_w + v_{w'}\|^2/(2d) + O(\epsilon_3) + O(\delta_0') - 2\log Z \pm 2\epsilon_z\pm \epsilon_2\\
		%&  = (1+\delta)\|v_w + v_{w'}\|^2/(2d) - 2\log Z \pm 2\epsilon_z\pm \epsilon_2\\
	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
	%& =  \sum_{c,c'}\Pr[C_t = c]\Pr[C_{t+1} = c'|C_t = c] \frac{e^{\inner{v_{w}}{\tv_c}}}{Z_c}  \frac{e^{\inner{v_{w'}}{\tv_{c'}}}}{Z_{c'}}  \nonumber\\
	%&= \log\left( \sum_{c}\expinner{v_w,\tilde{v}_c}p(c)\sum_{c'}\expinner{v_{w'},v_{c'}} p(c'vert c)\right) - 2\log Z + \log(1\pm \epsilon_z)
\end{align*}

where $\delta_0' = \delta_0\cdot \left(\Exp_{c\sim \mathcal{C}}[\expinner{v_w+v_{w'},c}]\right)^{-1}= \exp(-\Omega(\log^{1.8} n))$. 
%\Anote{Should be $\exp(-\Omega(\log^{1.8}n))$ as things are set up right now.} 
Note that $\epsilon_3 = \widetilde{O}(1/d)$, $\epsilon_z = \widetilde{O}(1/\sqrt{n})$, and $\epsilon_2$ by assumption, therefore we obtain that%, where in the last step we used  Lemma \ref{lem:bound} that  $\|v_w + v_{w'}\|_4^4/d^2 < \|v_w + v_{w'}\|^2/d^{1.6}$. 

%Note that $\epsilon_z, \epsilon_2$ are on the order of $o(1)$, and $\delta(\|v_w + v_{w'}\|^2/(2d) ) = o(1)$ for all $w$ and $w'$ by Lemma~\ref{lem:bound}, we obtain the desired bound, 
\begin{equation*}
\log p(w,w')   = \frac{1}{2d}\|v_w + v_{w'}\|^2 - 2\log Z \pm O(\epsilon_z) + O(\epsilon_2)+ \widetilde{O}(1/d).
\end{equation*}
%\Anote{In the revision the theorem statement spells out the $o_n(1)$ so we should probably do that here too?}


%We have the following lemma: 


\ %Tnote{To be completed. Could somebody do it?}
%We use $X_i$ as a shorthand for the random variable $(\tilde{v}_{c})_i$. Note that by assumption ??, we have that $X_i$ is symmetric  and $\Exp[X_i^2] = \frac{1}{d}$ and $|X_i|\le 2/\sqrt{d}$ a.s. Therefore we have 
%
%$$\Exp_{X_i}\exp(t_iX_i) = \sum_{j=0}^{\infty} \frac{t_i^{2j}}{(2j)!}\Exp[X_i^{2j}]$$
%
%Therefore, 
%%$$\Exp_{X_i}\exp(t_iX_i) \ge 1 + t_i^2/$$





%By our assumption on the stationary distribution for the context vector, it is an expectation over picking a random vector with coordinates in $\pm \frac{1}{\sqrt{d}}, 0$ according to the distribution which sets a coordinate in $\tv_c$ independently to $0$ with probability $1-p$, with probability $\frac{p}{2}$  to $\frac{1}{\sqrt{d}}$, and with probability $\frac{p}{2}$ to $-\frac{1}{\sqrt{d}}$. Since we are picking the coordinates independently, and for independent random variables the expectation of a product is a product of expectations, we can rewrite this as:
%$$ \log \prod_{k=1}^d \sbr{\frac{p}{2} ( \exp(\frac{(v)_k}{\sqrt{d}})+ \exp(-\frac{(v)_k}{\sqrt{d}}) + (1-p))}$$ 
%
%Notice that since  $v_k \leq \epsilon_1$ by Assumption 1, $\frac{(v)_k}{\sqrt{d}} < 1$. [ANDREJ NOTES: This needs to be made explicit. $\epsilon_1$ is something concrete when we make a distributional assumption.]  
% 
%Let's denote $f(x) = \log(\frac{p}{2} ( e^{x} + e^{-x}) + (1-p)) $ and look at its Taylor expansion:
%\begin{itemize} 
%\item $f'(x) = \frac{1}{\frac{p}{2} (e^{x} + e^{-x}) + (1-p) } \frac{p}{2}(e^x - e^{-x})$ 
%\item $f''(x) = \frac{1}{\frac{p}{2} (e^{x} + e^{-x}) + (1-p) } \frac{p}{2} (e^{x} + e^{-x}) - \frac{1}{(\frac{p}{2} (e^{x} + e^{-x}) + (1-p))^2} (\frac{p}{2})^2 (e^{x} - e^{-x})^2 $
%\end{itemize} 

%Hence, we can conclude that 
%$$   \log \prod_{k=1}^d \sbr{\frac{p}{2} ( \exp(\frac{(v)_k}{\sqrt{d}})+ \exp(-\frac{(v)_k}{\sqrt{d}}) + (1-p))} = \frac{p}{2d} (v)^2_k + O(\frac{p}{d^2} (v)^4_k).$$ 
%
%Hence, $\log (\sum_{c} \Pr[C_t = c] \exp\rbr{\inner{v_{w}+v_{w'}}{\tv_c}}) \leq \frac{p}{2d} \nbr{v_{w}+v_{w'}}_2^2 + O(\frac{p}{d^2} \nbr{v_{w}+v_{w'}}_4^4)$ as we needed. 
%The lower bound is proven analogously. 
\end{proof}

%\begin{lem}\label{lem:bound}
%	With high probability over the choice of $v_w$'s, we have that for any $w\in W$ and any $i$, 
%	$(v_w)_i \le 4\kappa\log n$, and for  any pair of words $w, w'$, 
%	$$\|v_w + v_{w'}\|_4^4/d^2 < \|v_w + v_{w'}\|^2/d^{1.6}$$
%\end{lem}
%
%
%
%\begin{proof} Recall that we assume $v_w$ are generated independently as $v_w = s_w \cdot \hat{v}_w $ where $s_w \le \kappa \sqrt{d}$  for some constant $\kappa$ and $\hat{v}_w$ is from a spherical Gaussian distribution (each coordinate is i.i.d $N(0, 1/d)$). 
%
%Let's do each of the claims separately.
% 
%For a standard Gaussian distribution, we know that 
%$$\Pr \left[ |(\hat{v}_w)_i|  \ge 4 d^{-0.5}  \log n  \right] \le e^{-\frac{16}{2} \log^2 n} $$ 
%
%Since $s_w \le \kappa \sqrt{d}$, we know that 
%$$\Pr \left[ |(s_w \cdot \hat{v}_w)_i|  \ge 4 \kappa \log n \right] \le e^{-\frac{16}{2} \log^2 n}  $$ 
%
%Union bounding, we have that with probability $1-d n e^{-\frac{16}{2} \log^2 n} = 1 - o(1)$ (recall that $d < n^{0.5}$), for all words $w$, for every coordinate $i$, $(v_w)_i \le 4\kappa\log n$. 
%
%The second claim is not much more difficult. 
%For standard Gaussian distribution, we know that 
%$$\Pr \left[ |(\hat{v}_w)_i|  \ge d^{ - 0.3} / \kappa \right] \le e^{- \frac{d^{0.4} }{2 \kappa^2 }}$$
%Since $s_w \le \kappa \sqrt{d}$, we know that 
%$$\Pr \left[ |(s_w \cdot \hat{v}_w)_i|  \ge d^{0.2 } \right] \le e^{- \frac{d^{0.4} }{2 \kappa^2 }}$$
%
%Taking a union bound, we have: with probability $1 - d n e^{- \frac{d^{0.4} }{2 \kappa^2 }}$ (note in our setting $ d n e^{- \frac{d^{0.4} }{2 \kappa^2 }} = o(1)$ for large enough $d$), for all words $w$ and their coordinate $i$, $|(v_w)_i|  \le d^{0.2 }$. In this case we have: 
%$$(v_w + v_{w'})_i^4/d^2 \le  (v_w + v_{w'})_i^2/d^{1.6} $$
%which easily implies the claim we want. 
%
%%For standard Gaussian distribution, we know that 
%%$$\Pr \left[ |(\hat{v}_w)_i|  \ge d^{ - 0.1} / \kappa \right] \le e^{- \frac{d^{0.8} }{2 \kappa^2 }}$$
%
%%Since $s_w \le \kappa \sqrt{d}$, we know that 
%%$$\Pr \left[ |(s_w \cdot \hat{v}_w)_i|  \ge d^{0.4 } \right] \le e^{- \frac{d^{0.8} }{2 \kappa^2 }}$$
%
%%Taking union bound, we have: with probability $1 - d n e^{- \frac{d^{0.8} }{2 \kappa^2 }}$ (note in our setting $ d n e^{- \frac{d^{0.8} }{2 \kappa^2 }} = o(1)$ for large enough $d$), for all words $w$ and their coordinate $i$, $|(v_w)_i|  \le d^{0.4 }$. In this case we have: 
%%$$(v_w + v_{w'})_i^4 \le d^{0.8} (v_w + v_{w'})_i^2   = o(d (v_w + v_{w'})_i^2  )$$
%%$$\Pr \left[ |\langle \hat{v}_w , e_i \rangle|  \ge \frac{}\right]  $$
%
%\end{proof}

%
%\begin{lem}
%\label{l:slowcontext}
%Suppose that for all the partition constants, $Z_c \leq (1+\epsilon_z) Z$ and $Z_c \geq (1-\epsilon_z) Z$ holds; furthermore, suppose that assumptions \emph{1} and \emph{2} hold. 
%Then, 
%$$\log (\Pr[(W_t,W_{t+1}) = (w,w')]) \leq \log (\sum_{c} \Pr[C_t = c] \frac{1}{Z^2} e^{\inner{v_i+v_j}{\tv_c}}) - 2\log(Z) + 2\epsilon_z + 2\epsilon_2 + o(\epsilon^2_z) + o(\epsilon^2_2)$$ and 
%$$\log (\Pr[(W_t,W_{t+1}) = (i, j)]) \geq \log (\sum_{c} \Pr[C_t = c] \frac{1}{Z^2} e^{\inner{v_i+v_j}{\tv_c}}) - 2\log(Z) - 2\epsilon_z - 2\epsilon_2 - o(\epsilon^2_z) - o(\epsilon^2_2)$$ 
%
%\Tnote{Let use $w,w'$ and $c,c'$ for words and contexts.. }
%
%\Tnote{I suggest combing this lemma with the next lemma together.. people can't parse this lemma ..}
%
%\Tnote{Please taker care of the new scaling of $v_w$ and $\tilde{v}_c$.}
%\end{lem} 
%\begin{proof}
%By definition, 
%
%$$ \log (\Pr[(W_t,W_{t+1}) = (i, j)]) = \log (\sum_{c,c'} \Pr[C_t = c] \Pr[C_{t+1} = c' | C_t = c] \frac{1}{Z_c} e^{\inner{v_i}{\tv_c}} \frac{1}{Z_{c'}} e^{\inner{v_j}{\tv_{c'}}}) $$
%
%Let's partition the summation over $c'$ according to $\Delta(\tv_c,\tv_{c'})$: 
%
%$$ \log (\Pr[(W_t,W_{t+1}) = (i, j)]) = \log (\sum_{c} \Pr[C_t = c] \sum^{d}_{\delta = 0} \sum_{c': \Delta(\tv_c,\tv_{c'}) = \delta} \Pr[C_{t+1} = c' | C_t = c] \frac{1}{Z_c} e^{\inner{v_i}{\tv_c}} \frac{1}{Z_{c'}} e^{\inner{v_j}{\tv_{c'}}}) $$
%
%Since $Z_c' \leq (1+\epsilon_z) Z$, 
%
%$$ \log (\Pr[(W_t,W_{t+1}) = (i, j)]) \leq \log (\sum_{c} \Pr[C_t = c] \frac{(1+\epsilon_z)^2}{Z^2} \sum^{d}_{\delta = 0} \sum_{c': \Delta(c,c') = \delta} \Pr[C_{t+1} = c' | C_t = c]  e^{\inner{v_i}{\tv_c}} e^{\inner{v_j}{\tv_{c'}}}) $$
%
%Since $e^{\inner{v_i}{\tv_c}} e^{\inner{v_j}{\tv_{c'}}} = e^{\inner{v_i+v_j}{\tv_c}} e^{\inner{v_j}{\tv_{c'}-\tv_c}}$, and since we assumed  $\forall l, (v_{j})_l \leq \epsilon_1$,   it follows that $e^{\inner{v_j}{\tv_{c'}-\tv_c}} \leq e^{\delta \epsilon_1}$. 
%
%Hence, we have that 
%$$ \log (\Pr[(W_t,W_{t+1}) = (i, j)]) \leq $$ 
%$$ \log (\sum_{c} \Pr[C_t = c] \frac{(1+\epsilon_z)^2}{Z^2} e^{\inner{v_i+v_j}{\tv_c}} \sum^{d}_{\delta = 0} \Pr[\Delta(\tv_{C_{t+1}}, \tv_c) = \delta] e^{\delta \epsilon_1}) \leq  $$
%$$ \log(\sum_{c} \Pr[C_t = c] \frac{(1+\epsilon_z)^2}{Z^2} e^{\inner{v_i+v_j}{\tv_c}} (1+\epsilon_2)) = $$
%$$ \log(\sum_{c} \Pr[C_t = c] e^{\inner{v_i+v_j}{\tv_c}}) - 2 \log(Z) + 2 \log(1+\epsilon_z) + \log(1+\epsilon_2) $$
%
%By Taylor expanding , we can show that $\log(1+x) = 1 + x + o(x^2)$, so the upper bound on $\log (\Pr[(W_t,W_{t+1}) = (i, j)])$ follows. 
%
%\Tnote{ $\log(1+x) = 1 + x + o(x^2)$ .. this is not true. }
%
%The lower bound is analogous. 
%
%\end{proof}
%
%Now, under assumption \emph{3}, we'll show that the above expression for the co-occurence probability simplifies even more. 
%
%\begin{lem} 
%\label{l:pairs} 
%Suppose the HMM random walk has a stationary distribution satisfying \emph{3}. Suppose $\epsilon_2$ is as specified in ~\ref{l:slowcontext}. Then, 
%
 %$\log (\Pr[(W_t,W_{t+1}) = (i, j)]) \leq \frac{p}{2}||v_i + v_j||_2^2  - 2\log(Z) + O(p||v_i+v_j||_4^4) + 2\epsilon_z + 2\epsilon_2 + o(\epsilon^2_z) + o(\epsilon^2_2)$ and
 %$\log (\Pr[(W_t,W_{t+1}) = (i, j)]) \geq \frac{p}{2}||v_i + v_j||_2^2  - 2\log(Z) - O(p||v_i+v_j||_4^4) - 2\epsilon_z - 2\epsilon_2 - o(\epsilon^2_z) - o(\epsilon^2_2)$
 %
%\end{lem} 
%
%\begin{proof}
%
%By Lemma~\ref{l:slowcontext}, $\log (\Pr[(W_t,W_{t+1}) = (i, j)]) \leq \log (\sum_{c} \Pr[C_t = c]e^{\inner{v_i+v_j}{\tv_c}}) + \log(Z) + 2\epsilon_z + 2\epsilon_2 + o(\epsilon^2_z) + o(\epsilon^2_2)$, so need only show $\log (\sum_{c} \Pr[C_t = c] e^{\inner{v_i+v_j}{\tv_c}}) \leq \frac{p}{2}||v_i + v_j||_2^2 + O(p||v_i+v_j||_4^4$. 
%
%By our assumption on the stationary distribution for the context vector, $\sum_{c} \Pr[C_t = c] e^{\inner{v_i+v_j}{\tv_c}})$ 
%is an expectation over picking a random -1,0,1 vector according to the distribution which sets a coordinate in $\tv_c$ independently to 0 with probability $1-p$, with probability $\frac{p}{2}$  to 1, and with probability $\frac{p}{2}$ to -1. Since we are picking the coordinates independently, using the fact that the expectation of a product is a product of expectations, we can rewrite this as:
%
%$$ \log( \Pi_{k=1}^d (\frac{p}{2} ( e^{(v_{i} + v_{j})_k} + e^{-(v_{i} + v_{j})_k}) + (1-p))$$ 
%
%We'll look at the Taylor expansion of
  %
%$$\log(\frac{p}{2} ( e^{(v_{i} + v_{j})_k} + e^{-(v_{i} + v_{j})_k}) + (1-p)) $$ 
%
%Let's denote $f(x) = \log(\frac{p}{2} ( e^{x} + e^{-x}) + (1-p)) $. After a little calculation one can conclude that 
%
%\begin{itemize} 
%
%\item $f'(x) = \frac{1}{\frac{p}{2} (e^{x} + e^{-x}) + (1-p) } \frac{p}{2}(e^x - e^{-x})$ 
%\item $f''(x) = \frac{1}{\frac{p}{2} (e^{x} + e^{-x}) + (1-p) } \frac{p}{2} (e^{x} + e^{-x}) - \frac{1}{(\frac{p}{2} (e^{x} + e^{-x}) + (1-p))^2} (\frac{p}{2})^2 (e^{x} - e^{-x})^2 $
%
%\end{itemize} 
%
%Hence, we can conclude that 
%$$ \log(\frac{p}{2} ( e^{(v_{i} + v_{j})_k} + e^{-(v_{i} + v_{j})_k}) + (1-p)) = \frac{p}{2} (v_{i} + v_{j})^2_k + O(p (v_{i} + v_{j})^4_k) $$ 
%
%Hence, $\log (\sum_{c} \Pr[C_t = c] e^{\inner{v_i+v_j}{v_c}}) \leq \frac{p}{2}||v_i + v_j||_2^2 + O(p||v_i+v_j||_4^4)$ as we needed. 
%The lower bound is proven analogously. 
%\end{proof}

%Now, depending on the type of guarantee we want, there's a few ways to proceed: 
%\begin{itemize} 
%\item If we want an additive guarantee, we can assume $p||v_i + v_j||_4^4 = O(\epsilon)$. The constants in the big-oh notation can be made explicit by assuming an upper bound on the coordinates of the word/context vectors. 
%\item If we want a multiplicative guarantee, we can assume 
%$$\frac{p(v_{i} + v_{j})^4_k}{\frac{p}{2} (v_{i} + v_{j})^2_k} = \frac{(v_{i} + v_{j})^4_k}{(v_{i} + v_{j})^2_k} = O(\epsilon) $$ 
%One easy way to get this guarantee is to assume non-sparsity of the vectors $v_i$.
%\end{itemize}

%In a completely analogous way, one can prove the following lemma:
%\begin{lem}  
%\label{l:singletons} For any word $w$, 
%$$
%\log (\Pr[W_t = w]) = (1 \pm \delta)\nbr{v_{w}}_2^2/(2d)  - \log(Z) \pm \epsilon_z $$
%\end{lem}  

%Now we can finish the proof of the main theorem: 

%\begin{proof} [Proof of Theorem~\ref{t:main}]
%\Tnote{Needs to be done}
%By Lemma~\ref{l:pairs} and ~\ref{l:singletons} it immediately follows that 
%\begin{align*} \log \frac{P_{w, w'}}{P_w P_{w'}} &= \frac{1}{2d}\rbr{ \nbr{v_w + v_{w'}}_2^2 - \nbr{v_w}_2^2 - \nbr{v_{w'}}_2^2 } \pm \delta ( \nbr{v_w^2} / d  + \nbr{v_{w'}^2} / d)  \pm 4\epsilon_z \pm \epsilon_2
%\\
%&= \frac{1}{2d} \inner{v_w}{v_{w'}} + O(\delta + \epsilon_z + \epsilon_2) 
%\end{align*}
%for $\epsilon_z = o(1), \delta, \epsilon_2 = d^{- 0.6}$, which is exactly what we need.  
%\end{proof} 
%
%\subsection{Normalization constants are approximately the same} 
%
%In this section, we show that under the assumption that the context and word vectors are sparse, the normalization constants $Z_c$ are close to each other. More precisely, we prove: 
%
%\begin{thm} Let the word and context vectors be $k$-sparse, for $k = o(\sqrt{n})$, and such that their norms are bounded by a constant $D$. Furthermore, supppose that for each possible support of size $k$, there is exactly one word vector with that support. (In particular, this means the number of words $n$ is equal to the number of possible k-sparse supports.) Then, for all contexts $c$, $Z_c = n(1 \pm o(1))$. 
%\end{thm} 
%
%\begin{proof}
%Suppose that the context and word vectors both are $k$-sparse. Notice that if $v_i, v_c$ for word $i$ and context $c$ are such that their supports are disjoint, $e^{\inner{v_i}{v_c}} = 1$. On the other hand, since $\nbr{v_i}_2 = 1, \nbr{v_c}_2 = 1$, we have that $\frac{1}{e^D} \leq e^{\inner{v_i}{v_c}} \leq e^D$.  
%
%Furthermore, for any fixed $c$, since the for each possible $k$-sparse support there is one word vector, the fraction of words whose support intersects with the support of $c$ is at most $\frac{k^2}{n} = o(1)$. 
%
%Altogether, the above two observations prove $\forall c, (1-o(1))n \leq Z_c \leq (1-o(1))n + o(1)n e^D $, i.e. $\forall c, Z_c = n (1\pm o(1))$, as we needed. 
%\end{proof}
%
%A statement of the above kind is also true when the word vectors are "spread out" in a certain sense. More specifically, what we want is that for all context vectors, if we look at most of the word vectors, $<v_w, v_c>$ is small. Formally the following is true: 
%
%\begin{lem} If for any context vector $c$, for all but $o(1)$ fraction of the words, $|\inner{v_w}{v_c}| = o(1)$, and additionally both the word and context vectors have norm bounded by a constant, then for any context $c$, $Z_c = |W|(1 \pm o(1))$.  
%\end{lem} 
%\begin{proof}
%
%For the words $w$ s.t. $|\inner{v_w}{v_c}| = o(1)$, $e^{\inner{v_w}{v_c}} = 1 \pm o(1)$. This is easy to see from the Taylor expansion of $e^{x}$. 
%
%Hence, if $W_1$ is the set of words such that $|\inner{v_w}{v_c}| = o(1)$, $\sum_{w \in W_1} e^{\inner{v_w}{v_c}} = |W_1| (1 \pm o(1))$.  
%
%On the other hand, since the set $W_2$ of words such that $|\inner{v_w}{v_c}| = \Omega(1)$ is of size $o(1) |W|$ and the norms of the word and context vectors are bounded by a constant, $\sum_{w \in W_2} e^{\inner{v_w}{v_c}} = o(1) |W|$. 
%
%Hence, $Z_c \geq \sum_{w \in W_1}  e^{\inner{v_w}{v_c}} \geq |W|(1-o(1)$, and 
%$$Z_c \leq \sum_{w \in W_1}  e^{\inner{v_w}{v_c}} + \sum_{w \in W_2} e^{\inner{v_w}{v_c}} \leq |W|(1 + o(1))$$ 
%which proves the claim we wanted. 
%
%\end{proof} 

%One thing to notice in particular is that the above is satisfied, for example, when the word vectors are sampled from a unit spherical Gaussian centered at 0. In this case, the probability that $\inner{v_w}{v_c} = \Omega( \frac{1}{\sqrt{d}})$, where $d$ is the dimension of the word and context vectors, is exponentially small. So, as long as the number of valid contexts is polynomial in the dimension, a simple union bound will show that the conditions of the above lemma are satisfied with high probability. 
%
%\subsection{Other context distributions} 
%
%What can we say here? 
The following lemmas are helper lemmas that were used in the proof above. We use $\mathcal{C}^d$ to denote the uniform distribution over the unit sphere in $\R^d$. 


%\begin{lem}[Tail bound for spherical distribution] \label{l:sphericalangle} 
%If $a$ and $b$ are two vectors in $\Real^d$ where $\nbr{a} = 1$ and $b$ is uniformly distributed over the unit sphere $S^{d-1}$, then for any $ \omega(1) \le \alpha \le \sqrt{d}/2$, 
%$$
  %\Pr\sbr{ \abr{ \inner{a}{b} } \ge  \frac{\alpha}{\sqrt{d}} } \le e^{- \Omega(\alpha^2)}.
%$$
%\end{lem} 
%
%\begin{proof}
%By symmetry we can set $a = \rbr{1, \cdots, 0}$. Also, we can assume $b = \frac{\btil }{\nbr{\btil}}$ where $\btil  \sim  N(0, \frac{1}{d} I )$. Let $r = \sum_{i = 2}^d \btil^2_i$ (note that $r$ does not contain $\btil^2_1$). 
%So we have
%\begin{align*}
%\Pr[\abr{\inner{a}{b} }  \ge t]  
%& = \Pr\sbr{\abr{\btil_1} \ge t \nbr{\btil} } \\
%& = \Pr\sbr{ \abr{\btil_1} \ge t \nbr{\btil} \bigg| r \ge \frac{2}{5}}\Pr\sbr{r \ge \frac{2}{5}} + \Pr\sbr{ \abr{\btil_1} \ge t \nbr{\btil} \bigg| r \ge \frac{2}{5}}\Pr\sbr{r \le \frac{2}{5}} \\
%& \le \Pr\sbr{ \abr{\btil_1} \ge t \nbr{\btil} \bigg| r \ge \frac{2}{5}}  + \Pr\sbr{r \le \frac{2}{5}}.
%\end{align*}
%
%$\Pr\sbr{r \le \frac{2}{5}}$ can be upper bounded by Bernstein-type bounds for sub-exponential random variables. More precisely,
%by Remark 5.18 and Lemma 5.14 in~\cite{Vershynin10}, we know that 
%$\btil^2_i - 1/d$ is centered  sub-exponential random variable with sub-exponential norm $O(1/d)$. So by Proposition 5.16 in~\cite{Vershynin10}, 
%\begin{align*}
  %\Pr\sbr{r \le \frac{2}{5}} 
	%& \le \Pr\sbr{ \abr{\sum_{i=2}^d \btil_i^2 - \frac{1}{d} } \ge  \frac{1}{10} } \\
	%& \le 2 \exp\rbr{- \Omega\rbr{d}} \\
	%& \le \frac{1}{2} \exp\rbr{- \Omega(\alpha^2)}.
%\end{align*} 
%
%Next, we bound $\Pr\sbr{ \abr{\btil_1} \ge t \nbr{\btil} \bigg| r \ge \frac{2}{5}}$.
%
%
%\[
%\Pr\sbr{\abr{\btil_1} \ge t \nbr{\btil}  \bigg| r \ge \frac{2}{5}} \le \Pr\sbr{\btil_1 \ge \sqrt{\frac{t^2 r}{1  - t^2}} \bigg| r \ge \frac{2}{5}}
%\le \Pr\sbr{\btil_1 \ge \sqrt{\frac{2 t^2 }{5 (1 - t^2)}}}.
%\]
%
%Denote $\ttil =  \sqrt{\frac{2 t^2 d}{5 (1 - t^2)}}$. Since $\sqrt{d} \btil_1$ is a standard Gaussian, by a well known Gaussian tail bound, 
%\[
%\Pr\sbr{\btil_1 \ge \sqrt{\frac{2 t^2 }{5 (1 - t^2)}}} = \Pr\sbr{\sqrt{d} \btil_1 \ge \ttil} \le \frac{1}{\ttil}\exp\rbr{-\Omega(\ttil^2)}.
%\]
%By choosing $t = O(\alpha/\sqrt{d})$, this is bounded by $\frac{1}{2} \exp\rbr{- \Omega(\alpha^2)}$. The lemma then follows.
%\end{proof}


\begin{lem} [Tail bound for spherical distribution] If $c \sim \mathcal{C}^d$, $v \in \mathbb{R}^d$ is a vector with $\|v\| = \Omega(\sqrt{d})$ and $t = \omega(1)$, the random variable $z = \langle v, c \rangle$ satisfies $\Pr[z \geq t] = e^{-O(t^2)}$.  
\label{l:sphericalangle} 
\end{lem} 
\begin{proof} 
If $c=(c_1, c_2, \dots, c_d) \sim \mathcal{C}^d$, $c$ is in distribution equal to $\left( \frac{\tilde{c}_1}{\|\tilde{c}\|}, \frac{\tilde{c}_2}{\|\tilde{c}\|}, \dots, \frac{\tilde{c}_d}{\|\tilde{c}\|} \right)$ where the $\tilde{c}_i$ are i.i.d. samples from a univariate Gaussian with mean 0 and variance $\frac{1}{d}$. % and output $c = (\frac{\tilde{c}_1}{\|\tilde{c}\|}, \frac{\tilde{c}_2}{\|\tilde{c}\|}, \dots, \frac{\tilde{c}_d}{\|\tilde{c}\|})$. 
By spherical symmetry, we may assume that $v = (\|v\|, 0, \dots, 0)$. 
%so we just want to show $\Pr\left[\|v\| \frac{\tilde{c}_1}{\|\tilde{c}\|} \geq t\right] \geq \exp(-\Omega(\log^2 n))$ for $t \le \Omega(\log^{.9} n)$. 
Let's introduce the random variable $r = \sum_{i=2}^d \tilde{c}^2_i$. 
Since 
\begin{equation*}  
\Pr\left[\langle v,c \rangle \geq t\right] = \Pr\left[\|v| \frac{\tilde{c}_1}{\|\tilde{c}\|} \geq t\right] \le \Pr\left[\frac{\|v\|\tilde{c}_1}{\|\tilde{c}\|} \geq t \mid r \ge \frac{1}{2}\right] \Pr\left[r \ge \frac{1}{2}\right]  + \Pr\left[\frac{\|v\|\tilde{c}_1}{\|\tilde{c}\|} \geq t \mid r \ge \frac{1}{2}\right] \Pr\left[r \ge \frac{1}{2}\right] 
\end{equation*}   

it's sufficient to lower bound $\Pr\left[r \leq 100\right]$ and $\Pr\left[\|v\| \frac{\tilde{c}_1}{\|c\|} \geq t \mid r \leq 100\right]$. The former probability is easily seen to be lower bounded by a constant by a Chernoff bound. Consider the latter one next. It holds that
\begin{equation*}
\Pr\left[\|v\| \frac{\tilde{c}_1}{\|\tilde{c}\|} \geq t \mid r \leq 100\right] = \Pr\left[\tilde{c}_1 \geq \sqrt{\frac{t^2 \cdot r}{\|v\|^2-t^2}} \mid r \leq 100\right] \geq \Pr\left[\tilde{c}_1 \geq \sqrt{\frac{100 t^2}{\|v\|^2-t^2}}\right]
\end{equation*}
Denoting $\tilde{t} = \sqrt{\frac{100 t^2}{\|v\|^2-t^2}}$, by a well-known Gaussian tail bound it follows that
$$\Pr\left[\tilde{c}_1 \geq \tilde{t} \right] = e^{-O(d \tilde{t}^2)}\left(\frac{1}{\sqrt{d} \tilde{t}} - \left(\frac{1}{\sqrt{d} \tilde{t}}\right)^3\right) = e^{-O(t^2)} $$ 

where the last equality holds since $\|v\| = \Omega(\sqrt{d})$ and $t = \omega(1)$. 
\end{proof} 

\begin{lem} If $c \sim \mathcal{C}^d$, $v \in \mathbb{R}^d$ is a vector with $\|v\| = \Theta(\sqrt{d})$ and $t = \omega(1)$, the random variable $z = \langle v,c \rangle$ satisfies 
$$\Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right]  = \exp(-\Omega(t^2)) + \exp(-\Omega(d)) $$
\label{l:abelspherical} 
\end{lem} 
\begin{proof}
%We claim the proof is trivial if $d = o(\log^{4}n)$. Indeed, in this case, $\exp(\langle v,c\rangle) \le \exp(\|v\|) = \exp(O(\sqrt{d}))$. Hence, 
%$$\Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right]  = \exp(O(\sqrt{d})) \Exp[\indicator{[t,+\infty]}(z)] = \exp(O(\sqrt{d})) \Pr[z \geq t] = $$
%$$\exp(O(\sqrt{d}) - \Omega(\log^{2}n))  = \exp(-\Omega(\log^{1.8}n))$$ 
%as we wanted. 
%However, $\Pr[z \geq t] = \exp(\Omega(t^2))$. 
%$$\exp(-\Omega(t^2) + O(\sqrt{d}))$$ 
%where the last equality follows by Lemma \ref{l:sphericalangle}. Since $\sqrt{d} = o(t^2)$, the claim follows. 

%So, we may, without loss of generality assume that $d = \Omega(\log^{4}n)$.  
Similarly as in Lemma~\ref{l:sphericalangle}, if $c=(c_1, c_2, \dots, c_d) \sim \mathcal{C}^d$, $c$ is in distribution equal to $\left( \frac{\tilde{c}_1}{\|\tilde{c}\|}, \frac{\tilde{c}_2}{\|\tilde{c}\|}, \dots, \frac{\tilde{c}_d}{\|\tilde{c}\|} \right)$ where the $\tilde{c}_i$ are i.i.d. samples from a univariate Gaussian with mean 0 and variance $\frac{1}{d}$. Again, by spherical symmetry, we may assume $v = (\|v\|, 0, \dots, 0)$. Let's introduce the random variable $r = \sum_{i=2}^d \tilde{c}^2_i$. Then,
%$$\Pr\left[\langle v, c \rangle = u\right] = \Pr\left[\|v\| c_1 = u\right] = \Pr\left[\|v\| \frac{\tilde{c}_1}{\|\tilde{c}\|} = u\right] \leq $$ 
%$$ \Pr\left[\|v\| \frac{\tilde{c}_1}{\|\tilde{c}\|} = u \mid r \geq 10\right] \Pr\left[r \geq 10\right]$$
%By a simple Markov inequality, $\Pr[r \geq 10]$ is upper bounded by a constant. 
for an arbitrary $u > 1$, some algebraic manipulation shows 
$$ \Pr\left[ \exp\left(\langle v,c \rangle\right)\indicator{[t,+\infty]}(\langle v, c\rangle)\geq u\right] = \Pr\left[ \exp\left(\langle v,c \rangle\right) \geq u \wedge \langle v, c\rangle \geq t \right] = $$ 
\begin{equation} 
\Pr\left[\exp\left(\|v\| \frac{\tilde{c}_1}{\|\tilde{c}\|}\right) \geq u \wedge \|v\| \frac{\tilde{c}_1}{\|\tilde{c}\|} \geq u \right] =  \Pr\left[\tilde{c}_1 = \max\left(\sqrt{\frac{\tilde{u}^2 r}{\|v\|^2 - \tilde{u}^2}}, \sqrt{\frac{t^2 r}{\|v\|^2 - t^2}}\right) \right] 
\label{eq:abelexpr1}
\end{equation}  
where we denote $\tilde{u} = \log u$. Since $\tilde{c}_1$ is a mean 0 univariate Gaussian with variance $\frac{1}{d}$, and $\|v\| = \Omega(\sqrt{d})$ we have $\forall x \in \mathbb{R}$ 
$$\Pr\left[\tilde{c}_1 \geq \sqrt{\frac{x^2 r}{\|v\|^2 - u^2}} \right] = O\left(e^{-\Omega(x^2 r)}\right)$$ 
Next, we show that $r$ is lower bounded by a constant with probability $1-\exp(-\Omega(d))$. Indeed, $r$ is in distribution equal to $\frac{1}{d} \chi^2_{d-1}$, where $\chi^2_k$ is a Chi-squared distribution with $k$ degrees of freedom. Standard concentration bounds \cite{laurent2000adaptive} imply that $\forall \xi \geq 0, \Pr[r-1 \leq -2\sqrt{\frac{\xi}{d}}] \leq \exp(-\xi)$. Taking $\xi = \alpha d$ for $\alpha$ a constant implies that with probability $1-\exp(-\Omega(d))$,  $r \geq M$ for some constant $M$. 
%$$\Pr[\tilde{c}_i \geq \alpha \frac{1}{\sqrt{d}}] \geq \frac{1}{\sqrt{d} \alpha \frac{1}{\sqrt{d}}} e^{-d (\alpha \frac{1}{\sqrt{d}})^2} = \Omega(1)$$ 
%Since the $\tilde{c}_i$ are indepedendent, all $\tilde{c}_i$ are upper bounded by a constant with probability at most $\exp(-\Omega(n))$. Since $r = \sum_i \tilde{c}^2_i$, this implies that with probability $1-\exp(-\Omega(n))$, $r \geq M $ for some constant $M$. 
We can now rewrite
$$\Pr\left[\tilde{c}_1 \geq \sqrt{\frac{x^2 r}{\|v\|^2 - x^2}} \right] =  $$
$$ \Pr\left[\tilde{c}_1 \geq \sqrt{\frac{x^2 r}{\|v\|^2 - x^2}}  \mid r \geq M\right] \Pr[r \geq M] + \Pr\left[\tilde{c}_1 \geq \sqrt{\frac{x^2 r}{\|v\|^2 - x^2}} \mid r \leq M\right] \Pr[r \leq M]$$  
The first term is clearly bounded by $ e^{-\Omega(x^2)}$ and the second by $\exp(-\Omega(d))$. 
%But note that since $\|v\| = O(\sqrt{d})$ and $u \leq \|v\|$, $e^{-\Omega(u^2)} = e^{-\Omega(d)}$. 
Therefore, 
\begin{equation} 
\Pr\left[\tilde{c}_1 \geq \sqrt{\frac{x^2 r}{\|v\|^2 - x^2}} \right] = O\left(\max\left(\exp\left(-\Omega\left(x^2\right)\right), \exp\left(-\Omega\left(d\right)\right)\right)\right) 
\label{eq:abelexpr2}
\end{equation} 
%%\Anote{Here/next line is where $\|v\|$ requires a lower bound.} , 
Putting \ref{eq:abelexpr1} and \ref{eq:abelexpr2} together, we get that 
\begin{equation} 
\Pr\left[ \exp\left(\langle v,c \rangle\right)\indicator{[t,+\infty]}(\langle v, c\rangle)\geq u\right] = O\left(\max\left(\exp\left(-\Omega\left(\min\left(d, \left(\max\left(\tilde{u},t\right)\right)^2\right)\right)\right)\right)\right) 
\label{eq:abelexpr3}
\end{equation}
(where again, we denote $\tilde{u} = \log u$) 

For any random variable $X$ which has non-negative support, it's easy to check that 
$$\Exp[X] = \int_{0}^{\infty} \Pr[X \geq x] dx $$ 
Hence, 
%$$\Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right] = \int_{t}^{\|v\|} \Pr[\langle v,c \rangle = u] e^{u} du = \int_{t}^{\|v\|} O\left(\sqrt{d} e^{-\Omega(u^2)}\right) du = O(\sqrt{d} e^{-\Omega(t^2)})$$
$$\Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right] = \int_{0}^{\infty} \Pr\left[\exp(z)\indicator{[t,+\infty]}(z) \geq u \right] du = \int_{0}^{\exp(\|v\|)} \Pr\left[\exp(z)\indicator{[t,+\infty]}(z) \geq u \right] du $$
To bound this integral, we split into the following two cases: 
\begin{itemize} 
\item Case $t^2 \geq d$: $\max\left(\tilde{u},t\right) \geq t$, so $\min\left(d, \left(\max\left(\tilde{u},t\right)\right)^2\right) = d$. Hence, \ref{eq:abelexpr3} implies 
$$\Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right] = \exp(\|v\|)\exp(-\Omega(d)) = \exp(-\Omega(d))  $$
where the last inequality follows since $\|v\| = O(\sqrt{d})$. 
\item Case $t^2 < d$: In the second case, we will split the integral into two portions: 
$u \in [0, \exp(t)]$ and $u \in [\exp(t), \exp(\|v\|)]$. 

When $u \in [0, \exp(t)]$, $\max\left(\tilde{u},t\right)= t$, so $\min(d,\left(\max\left(\tilde{u},t\right)\right)^2) = t^2$. Hence, 
$$ \int_{0}^{\exp(t)} \Pr\left[\exp(z)\indicator{[t,+\infty]}(z) \geq u \right] du \leq \exp(t) \exp(-\Omega(t^2)) = -\exp(\Omega(t^2))$$ 

When $u \in [\exp(t), \exp(\|v\|)]$, $\max\left(\tilde{u},t\right)= \tilde{u}$. 
But $\tilde{u} \leq \log(\exp(\|v\|)) = O(\sqrt{d})$, so $\min(d,\left(\max\left(\tilde{u},t\right)\right)^2) = \tilde{u}$. Hence, 
$$ \int_{\exp(t)}^{\exp(\|v\|)} \Pr\left[\exp(z)\indicator{[t,+\infty]}(z) \geq u \right] du \leq \int_{\exp(t)}^{\exp(\|v\|)} \exp(-(\log(u))^2) du$$
Making the change of variable $\tilde{u} = \log(u)$, the we can rewrite the last integral as
$$ \int_{t}^{\|v\|} \exp(-\tilde{u}^2) \exp(\tilde{u}) d\tilde{u} = O(\exp(-t^2)) $$ 
where the last inequality is the usual Gaussian tail bound. 
%The first part is bounded by 
%$\exp(-t^2)\exp(t) = \exp(-t^2)$. The second part is  
%$$\int_{\exp(t)}^{\exp(\|v\|)} \exp(-(\log(u))^2) du = \int_{t}^{\|v\|} \exp(-\tilde{u}^2) e^{\tilde{u}} d\tilde{u} = O(\exp(-t^2))$$
%by the standard Gaussian tail bound.  
\end{itemize} 
In either case, we get that 
$$\int_{0}^{\exp(\|v\|)} \Pr\left[\exp(z)\indicator{[t,+\infty]}(z) \geq u \right] du =  \exp(-\Omega(t^2)) + \exp(-\Omega(d))) $$ 
which is what we want.
%where the last inequality holds because we assumed $d = \Omega(\log^{4}n)$ and $t^2 = \Omega(\log^{.9}n)$, so we get the claim we wanted.   
%$$ \int_{t}^{\infty} e^{-\Omega(u^2)} du = e^{-\Omega(t^2)}$$
%by a usual Gaussian tail bound, which gives the bound we want. 
\end{proof} 

As a corollary to the above lemma, we get the following: 

\begin{cor} If $c \sim \mathcal{C}^d$, $v \in \mathbb{R}^d$ is a vector with $\|v\| = \Theta(\sqrt{d})$ and %$t = \Omega(\log^{0.8}n)$
$t = \Omega(\log^{.9}n)$ then  
$$\Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right]  = \exp(-\Omega(\log^{1.8}n)) $$
\label{c:abelspherical} 
\end{cor} 
\begin{proof}
We claim the proof is trivial if $d = o(\log^{4}n)$. Indeed, in this case, $\exp(\langle v,c\rangle) \le \exp(\|v\|) = \exp(O(\sqrt{d}))$. Hence, 
$$\Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right]  = \exp(O(\sqrt{d})) \Exp[\indicator{[t,+\infty]}(z)] = \exp(O(\sqrt{d})) \Pr[z \geq t] $$
Since by Lemma~\ref{l:sphericalangle}, $\Pr[z \geq t] \le \exp(-\Omega(\log^2 n)$, we get
$$\Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right] = \exp(O(\sqrt{d}) - \Omega(\log^{2}n))  = \exp(-\Omega(\log^{1.8}n))$$ 
as we wanted. 
%However, $\Pr[z \geq t] = \exp(\Omega(t^2))$. 
%$$\exp(-\Omega(t^2) + O(\sqrt{d}))$$ 
%where the last equality follows by Lemma \ref{l:sphericalangle}. Since $\sqrt{d} = o(t^2)$, the claim follows. 

So, we may, without loss of generality assume that $d = \Omega(\log^{4}n)$. In this case, Lemma~\ref{l:abelspherical} implies  
$$\Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right]  = \exp(-\log^{1.8}n) + \exp(-\Omega(d)))  = \exp(-\log^{1.8}n)$$ 
where the last inequality holds because $d = \Omega(\log^{4}n)$ and $t^2 = \Omega(\log^{.9}n)$, so we get the claim we wanted.   

%Similarly as in Lemma~\ref{l:sphericalangle}, if $c=(c_1, c_2, \dots, c_d) \sim \mathcal{C}^d$, $c$ is in distribution equal to $\left( \frac{\tilde{c}_1}{\|\tilde{c}\|}, \frac{\tilde{c}_2}{\|\tilde{c}\|}, \dots, \frac{\tilde{c}_d}{\|\tilde{c}\|} \right)$ where the $\tilde{c}_i$ are i.i.d. samples from a univariate Gaussian with mean 0 and variance $\frac{1}{d}$. Again, by spherical symmetry, we may assume $v = (\|v\|, 0, \dots, 0)$. Let's introduce the random variable $r = \sum_{i=2}^d \tilde{c}^2_i$. Then,
%%$$\Pr\left[\langle v, c \rangle = u\right] = \Pr\left[\|v\| c_1 = u\right] = \Pr\left[\|v\| \frac{\tilde{c}_1}{\|\tilde{c}\|} = u\right] \leq $$ 
%%$$ \Pr\left[\|v\| \frac{\tilde{c}_1}{\|\tilde{c}\|} = u \mid r \geq 10\right] \Pr\left[r \geq 10\right]$$
%%By a simple Markov inequality, $\Pr[r \geq 10]$ is upper bounded by a constant. 
%for an arbitrary $u > 1$, some algebraic manipulation shows 
%$$ \Pr\left[ \exp\left(\langle v,c \rangle\right)\indicator{[t,+\infty]}(\langle v, c\rangle)\geq u\right] = \Pr\left[ \exp\left(\langle v,c \rangle\right) \geq u \wedge \langle v, c\rangle \geq t \right] = $$ 
%\begin{equation} 
%\Pr\left[\exp\left(\|v\| \frac{\tilde{c}_1}{\|\tilde{c}\|}\right) \geq u \wedge \|v\| \frac{\tilde{c}_1}{\|\tilde{c}\|} \geq u \right] =  \Pr\left[\tilde{c}_1 = \max\left(\sqrt{\frac{\tilde{u}^2 r}{\|v\|^2 - \tilde{u}^2}}, \sqrt{\frac{t^2 r}{\|v\|^2 - t^2}}\right) \right] 
%\label{eq:abelexpr1}
%\end{equation}  
%where we denote $\tilde{u} = \log u$. Since $\tilde{c}_1$ is a mean 0 univariate Gaussian with variance $\frac{1}{d}$, and $\|v\| = \Omega(\sqrt{d})$ we have $\forall x \in \mathbb{R}$ 
%$$\Pr\left[\tilde{c}_1 \geq \sqrt{\frac{x^2 r}{\|v\|^2 - u^2}} \right] = O\left(e^{-\Omega(x^2 r)}\right)$$ 
%Next, we show that $r$ is lower bounded by a constant with probability $1-\exp(-\Omega(d))$. Indeed, $r$ is in distribution equal to $\frac{1}{d} \chi^2_{d-1}$, where $\chi^2_k$ is a Chi-squared distribution with $k$ degrees of freedom. Standard concentration bounds \cite{laurent2000adaptive} imply that $\forall \xi \geq 0, \Pr[r-1 \leq -2\sqrt{\frac{\xi}{d}}] \leq \exp(-\xi)$. Taking $\xi = \alpha d$ for $\alpha$ a constant implies that with probability $1-\exp(-\Omega(d))$,  $r \geq M$ for some constant $M$. 
%%$$\Pr[\tilde{c}_i \geq \alpha \frac{1}{\sqrt{d}}] \geq \frac{1}{\sqrt{d} \alpha \frac{1}{\sqrt{d}}} e^{-d (\alpha \frac{1}{\sqrt{d}})^2} = \Omega(1)$$ 
%%Since the $\tilde{c}_i$ are indepedendent, all $\tilde{c}_i$ are upper bounded by a constant with probability at most $\exp(-\Omega(n))$. Since $r = \sum_i \tilde{c}^2_i$, this implies that with probability $1-\exp(-\Omega(n))$, $r \geq M $ for some constant $M$. 
%We can now rewrite
%$$\Pr\left[\tilde{c}_1 \geq \sqrt{\frac{x^2 r}{\|v\|^2 - x^2}} \right] =  $$
%$$ \Pr\left[\tilde{c}_1 \geq \sqrt{\frac{x^2 r}{\|v\|^2 - x^2}}  \mid r \geq M\right] \Pr[r \geq M] + \Pr\left[\tilde{c}_1 \geq \sqrt{\frac{x^2 r}{\|v\|^2 - x^2}} \mid r \leq M\right] \Pr[r \leq M]$$  
%The first term is clearly bounded by $ e^{-\Omega(x^2)}$ and the second by $\exp(-\Omega(d))$. 
%%But note that since $\|v\| = O(\sqrt{d})$ and $u \leq \|v\|$, $e^{-\Omega(u^2)} = e^{-\Omega(d)}$. 
%Therefore, 
%\begin{equation} 
%\Pr\left[\tilde{c}_1 \geq \sqrt{\frac{x^2 r}{\|v\|^2 - x^2}} \right] = O\left(\max\left(\exp\left(-\Omega\left(x^2\right)\right), \exp\left(-\Omega\left(d\right)\right)\right)\right) 
%\label{eq:abelexpr2}
%\end{equation} 
%%%\Anote{Here/next line is where $\|v\|$ requires a lower bound.} , 
%Putting \ref{eq:abelexpr1} and \ref{eq:abelexpr2} together, we get that 
%\begin{equation} 
%\Pr\left[ \exp\left(\langle v,c \rangle\right)\indicator{[t,+\infty]}(\langle v, c\rangle)\geq u\right] = O\left(\max\left(\exp\left(-\Omega\left(\min\left(d, \left(\max\left(\tilde{u},t\right)\right)^2\right)\right)\right)\right)\right) 
%\label{eq:abelexpr3}
%\end{equation}
%(where again, we denote $\tilde{u} = \log u$) 
%
%For any random variable $X$ which has non-negative support, it's easy to check that 
%$$\Exp[X] = \int_{0}^{\infty} \Pr[X \geq x] dx $$ 
%Hence, 
%%$$\Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right] = \int_{t}^{\|v\|} \Pr[\langle v,c \rangle = u] e^{u} du = \int_{t}^{\|v\|} O\left(\sqrt{d} e^{-\Omega(u^2)}\right) du = O(\sqrt{d} e^{-\Omega(t^2)})$$
%$$\Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right] = \int_{0}^{\infty} \Pr\left[\exp(z)\indicator{[t,+\infty]}(z) \geq u \right] du = \int_{0}^{\exp(\|v\|)} \Pr\left[\exp(z)\indicator{[t,+\infty]}(z) \geq u \right] du $$
%To bound this integral, we split into the following two cases: 
%\begin{itemize} 
%\item Case $t^2 \geq d$: $\max\left(\tilde{u},t\right) \geq t$, so $\min\left(d, \left(\max\left(\tilde{u},t\right)\right)^2\right) = d$. Hence, \ref{eq:abelexpr3} implies 
%$$\Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right] = \exp(\|v\|)\exp(-\Omega(d)) = \exp(-\Omega(d))  $$
%where the last inequality follows since $\|v\| = O(\sqrt{d})$. 
%\item Case $t^2 < d$: In the second case, we will split the integral into two portions: 
%$u \in [0, \exp(t)]$ and $u \in [\exp(t), \exp(\|v\|)]$. 
%
%When $u \in [0, \exp(t)]$, $\max\left(\tilde{u},t\right)= t$, so $\min(d,\left(\max\left(\tilde{u},t\right)\right)^2) = t^2$. Hence, 
%$$ \int_{0}^{\exp(t)} \Pr\left[\exp(z)\indicator{[t,+\infty]}(z) \geq u \right] du \leq \exp(t) \exp(-\Omega(t^2)) = -\exp(\Omega(t^2))$$ 
%
%When $u \in [\exp(t), \exp(\|v\|)]$, $\max\left(\tilde{u},t\right)= \tilde{u}$. 
%But $\tilde{u} \leq \log(\exp(\|v\|)) = O(\sqrt{d})$, so $\min(d,\left(\max\left(\tilde{u},t\right)\right)^2) = \tilde{u}$. Hence, 
%$$ \int_{\exp(t)}^{\exp(\|v\|)} \Pr\left[\exp(z)\indicator{[t,+\infty]}(z) \geq u \right] du \leq \int_{\exp(t)}^{\exp(\|v\|)} \exp(-(\log(u))^2) du$$
%Making the change of variable $\tilde{u} = \log(u)$, the we can rewrite the last integral as
%$$ \int_{t}^{\|v\|} \exp(-\tilde{u}^2) \exp(\tilde{u}) d\tilde{u} = O(\exp(-t^2)) $$ 
%where the last inequality is the usual Gaussian tail bound. 
%%The first part is bounded by 
%%$\exp(-t^2)\exp(t) = \exp(-t^2)$. The second part is  
%%$$\int_{\exp(t)}^{\exp(\|v\|)} \exp(-(\log(u))^2) du = \int_{t}^{\|v\|} \exp(-\tilde{u}^2) e^{\tilde{u}} d\tilde{u} = O(\exp(-t^2))$$
%%by the standard Gaussian tail bound.  
%\end{itemize} 
%In either case, we get that 
%$$\int_{0}^{\exp(\|v\|)} \Pr\left[\exp(z)\indicator{[t,+\infty]}(z) \geq u \right] du =  \exp(-\Omega(t^2)) + \exp(-\Omega(d)))  = \exp(-\log^{1.8}n)$$ 
%where the last inequality holds because we assumed $d = \Omega(\log^{4}n)$ and $t^2 = \Omega(\log^{.9}n)$, so we get the claim we wanted.   
%%$$ \int_{t}^{\infty} e^{-\Omega(u^2)} du = e^{-\Omega(t^2)}$$
%%by a usual Gaussian tail bound, which gives the bound we want. 
\end{proof} 
%
%\begin{lem}\label{lem:moment}
%	If a real random variable $X$ is symmetric and $\Exp[X^2] = 1/d$ and $|X|\le 2/\sqrt{d}$ a.s. Then for $t < \sqrt{d}/10$, we have
%		$$1+ \frac{t^2}{2d} \le \Exp_{X}\exp(tX) \le  1+ \frac{t^2}{2d} + \frac{4}{3}\left(\frac{t}{\sqrt{d}}\right)^{4}$$
%\end{lem}
%\begin{proof}
%	By the moment generating function of $X$, we have 
%	$$\Exp_{X}\exp(tX) = \sum_{j=0}^{\infty} \frac{t^{j}}{(j)!}\Exp[X^{j}]$$
%	
%	Therefore by the assumption that $X$ is symmetric and $\Exp[X^2] = \frac{1}{d}$, we have that 
%	
%	$$\Exp_{X}\exp(tX) \ge 1+ \frac{t^2}{2d}$$
%	
%	On the other hand, using the fact that $|X|< \frac{2}{\sqrt{d}}$ a.s.
%	$$\Exp_{X}\exp(tX) = \sum_{j=0}^{\infty} \frac{t^{2j}}{(2j)!}\Exp[X^{2j}] = 1+ \frac{t^2}{2d} + \sum_{j=2}^{\infty}\frac{1}{(2j)!}\left(\frac{2t}{\sqrt{d}}\right)^{2j}\le 1+ \frac{t^2}{2d} + \frac{4}{3}\left(\frac{t}{\sqrt{d}}\right)^{4}$$
%	where the last inequality is because we choose $t < \sqrt{d}/10$: $\frac{t}{\sqrt{d}} < 1/10$; hence 
%	$$\sum_{j=2}^{\infty}\frac{1}{(2j)!}\left(\frac{2t}{\sqrt{d}}\right)^{2j} \le \left( \frac{t}{\sqrt{d}}\right)^4 \sum_{j = 0}^{\infty}\left( \frac{1}{5} \right)^{2 j} \le \frac{4}{3}\left(\frac{t}{\sqrt{d}}\right)^{4} $$
%\end{proof}

%\begin{lem}\label{l:helperexp} If $c \sim \mathcal{C}^d, z = \langle v,c\rangle$ such that $v = O(\sqrt{d}$, and $0\le r(z)\le 1$ then 
%$$\Exp_c[u(z)r(z)] \le \Exp_c[r(z)] + \Exp_c[\exp(\alpha z) r(\alpha z) \indicator{[t,+\infty]}]$$ 
%\end{lem}
%\begin{proof}
%
%\end{proof} 

\begin{lem}[Continuous Abel's Inequality]\label{lem:abel}
	%Suppose $f(x)$ is density function and $F$ be the corresponding CDF , and $u(x)$ is an increasing function over the reals. 
	Let $0\le r(x)\le 1$ be a function such that such that $\Exp[r(x)] = \rho$. Moreover, suppose increasing function $u(x)$ satisfies that $\Exp[|u(x)|] < \infty$. Let $t$ be the real number  such that $\Exp[\indicator{[t,+\infty]}] = \rho$. 
	Then we have 
		\begin{equation}
		\Exp[u(x)r(x)]\le \Exp[u(x)\indicator{[t,+\infty]}]
		\end{equation}
\end{lem}

\begin{proof}
Let $G(z) = \int_{z}^{\infty} f(x)r(x) dx$, and $H(z) = \int_{z}^{\infty} f(x)\indicator{[t,+\infty]}(x)dx$. Then we have that $G(z)\le H(z)$ for all $z$. Indeed, for $z\ge t$, this is trivial since $r(z)\le 1$. For $z\le t$, we have  $H(z) = \Exp[\indicator{[t,+\infty]}] = \rho = \Exp[r(x)]\ge \int_{z}^{\infty} f(x)r(x) dx.$ Then by integration by parts we have, 
	\begin{align*}
				\int_{-\infty}^{\infty} u(x)f(x)r(x)dx& %= \int_{-\infty}^{\infty} u(x) f(x)\indicator{E} dx 
				=- \int_{-\infty}^{\infty} u(x) dG \\
&				= -u(x)G(x)\mid_{-\infty}^{\infty} + \int_{-\infty}^{+\infty} G(x)u'(x)dx \\
&				\le   \int_{-\infty}^{+\infty} H(x)u'(x)dx \\
& = \int_{-\infty}^{\infty} u(x)f(x)\indicator{[t,+\infty]}(x)dx, 
		\end{align*}
		where at the third line we use the fact that $u(x)G(x)\rightarrow 0$ as $x\rightarrow \infty$ and that $u'(x)\ge 0$, and at the last line we integrate by parts again. 
\end{proof}

\begin{lem}\label{lem:helper1}
	Let $v\in \R^d$ be a fixed vector with norm $\|v\| \le \kappa \sqrt{d}$ for absolute constant $\kappa$. Then for random variable $c$ with uniform distribution over the sphere, we have that 
	\begin{equation}
	\log \Exp[\exp(\inner{v}{d})] = \|v\|^2/{2d} \pm \epsilon
	\end{equation}
	where $\epsilon = \widetilde{O}(\frac{1}{d})$. 
\end{lem}

\begin{proof}
	Let $g\in \mathcal{N}(0,I)$, then $g/\|g\|$ has the same distribution as $c$. Let $r = \|v\|$. Since $c$ is spherically symmetric, we could, we can assume without loss of generality that $v = (r,0,\dots,0)$. Let $x= g_1$ and $y = \sqrt{g_2^2+\dots+g_d^2}$. Therefore $x\in \mathcal{N}(0,1)$ and $y^2$ has $\chi^2$ distribution with mean $d-1$ and variance $O(d)$.  
	
	Let $\mathcal{F}$ be the event that $x\le 20 \log d$ and $1.5\sqrt{d}\ge y\ge 0.5\sqrt{d}$. Note that the $\Pr[\mathcal F] \ge 1- \exp(-\Omega(\log^{1.8}(d))$. By Proposition~\ref{prop:helper4}, we have that 
	$ \Exp[\exp(\inner{v}{c})]  = \Exp[\exp(\inner{v}{c})\mid \mathcal{F}]\cdot (1\pm \Omega(-\log^{1.8}d))$. 
	%	\begin{equation}
	%	\Exp[\exp(\inner{v}{c})]  = \Exp[\exp(\inner{v}{c})\mid \mathcal{F}] \pm O(1/d^{10})
	%	\end{equation}
	
	Conditioned on event $\mathcal F$, we have 
	\begin{align}
		\Exp[\exp(\inner{v}{c})\mid \mathcal{F}] & = \Exp\left[\exp(\frac{rx}{\sqrt{x^2+y^2}})\mid \mathcal{F}\right]\nonumber\\
		& = \Exp\left[\exp(\frac{rx}{y} -\frac{rx^3}{y\sqrt{x^2+y^2}(y+\sqrt{x^2+y^2})} )\mid \mathcal{F}\right]\nonumber\\
		& = \Exp\left[\exp(\frac{rx}{y})\cdot \exp(\frac{rx^3}{y\sqrt{x^2+y^2}(y+\sqrt{x^2+y^2})} )\mid \mathcal{F}\right]\nonumber\\
		& = \Exp\left[\exp(\frac{rx}{y})\mid \mathcal F\right] \cdot (1\pm O(\frac{\log^{3} d}{d}) )\label{eqn:eqn17}
	\end{align}
	where we used the fact that $r\le \kappa \sqrt{d}$. Let $\mathcal{E}$ be the event that $1.5\sqrt{d}\ge y\ge 0.5\sqrt{d}$. By using Proposition~\ref{prop:helper3}, we have that 
	\begin{equation}
	\Exp[\exp(rx/y)\mid \mathcal F] =%= \Exp[\exp(rx/y)] \pm \exp(-\Omega(\log^2(d)) = 
	\Exp[\exp(rx/y)\mid \mathcal{E}] \pm \exp(-\Omega(\log^2(d))
	\end{equation} %and that conditioned on $\mathcal F$, it holds that $x\le 20\sqrt{\log d}$ and $y^2 \ge d/2$. 
	Then let $z = y^2/(d-1)$ and $w = z-1$. Therefore $z$ has $\chi^2$ distribution with mean 1 and variance $1/(d-1)$, and $w$ has mean 0 and variance $1/(d-1)$. 
	\newcommand{\calF}{\mathcal F}
	\begin{align*}
		%\Exp[\exp(\inner{v}{c})\mid \mathcal{F}] & = \Exp\left[\exp(\frac{rx}{\sqrt{x^2+y^2}})\mid \mathcal{F}\right]\\
		%& = \Exp\left[\exp(\frac{rx}{y} -\frac{rx^3}{y\sqrt{x^2+y^2}(y+\sqrt{x^2+y^2})} )\mid \mathcal{F}\right]\\
		%& = \Exp\left[\exp(\frac{rx}{y})\cdot \exp(\frac{rx^3}{y\sqrt{x^2+y^2}(y+\sqrt{x^2+y^2})} )\mid \mathcal{F}\right]\\
		\Exp\left[\exp(\frac{rx}{y})\mid \mathcal{E}\right] &= \Exp[\Exp[\exp(rx/y)\mid y]\mid \mathcal{E}]= \Exp[\exp(r^2/y^2)\mid \mathcal{E}] \\
		&  = \Exp[\exp(r^2/(d-1) \cdot 1/z^2 )\mid \mathcal{E}]\\ 
		& = \Exp[\exp(r^2/(d-1) \cdot (1+ \frac{2w+w^2}{(1+w)^2}))\mid \mathcal E]\\ 
		& = \exp(r^2/(d-1)) \Exp[\exp( 1+ \frac{2w+w^2}{(1+w)^2}))\mid \mathcal{E}]\\ 
		& = \exp(r^2/(d-1)) \Exp[ 1+ 2w \pm O(w^2)\mid \mathcal{E}]\\ 
		& = \exp(r^2/(d-1)^2) (1\pm 1/d)
	\end{align*}
	
	where the second-to-last line uses the fact that conditioned on $1/2\ge \mathcal E$, $w\ge -1/2$ and therefore the Taylor expansion approximates the exponential accurately,  and %therefore %$\frac{2w+w^2}{(1+w)^2} \le O(1)$
	the last line uses the fact that $|\Exp[w\mid \mathcal{E}]| = O(1/d)$ and $\Exp[w^2 \mid \mathcal E] \le O(1/d)$. Combining the series of approximations above completes the proof. 
	
\end{proof}

We finally provide the proofs for a few helper propositions on conditional probabilities for high probability events used in the lemma above.  

\begin{proposition}\label{prop:helper3}
	Suppose $x\sim \mathcal{N}(0,\sigma^2)$ with $\sigma = O(1)$. Then for any event $\mathcal E$ with $\Pr[\mathcal E] = 1-O(-\Omega(\log^2 d))$, we have that $\Exp[\exp(x)] = \Exp[\exp(x)\mid \mathcal{E}] \pm \exp(-\Omega(\log^2(d))$. 
\end{proposition}
\begin{proof}
Let's denote by $\bar{\mathcal{E}}$ the complement of the event $\mathcal{E}$. We will consider the upper and lower bound separately. 
Since 
$$\Exp[\exp(x)] = \Exp[\exp(x) \mid \mathcal{E}] \Pr[\mathcal{E}] + \Exp[\exp(x) \mid \bar{\mathcal{E}}] \Pr[\bar{\mathcal{E}}] $$
we have that 
\begin{equation} \Exp[\exp(x)] \le \Exp[\exp(x) \mid \mathcal{E}]  + \Exp[\exp(x) \mid \bar{\mathcal{E}}] \Pr[\bar{\mathcal{E}}] \label{eq:lbh3} \end{equation} 
and 
\begin{equation} \Exp[\exp(x)] \ge \Exp[\exp(x) \mid \mathcal{E}] (1-\exp(-\Omega(\log^2 d))) \ge \Exp[\exp(x) \mid \mathcal{E}] - \Exp[\exp(x) \mid \mathcal{E}] \exp(-\Omega(\log^2 d))) \label{eq:uph3} \end{equation}

Consider the upper bound \eqref{eq:lbh3} first. To show the statement of the lemma, it suffices to bound $\Exp[\exp(x) \mid \bar{\mathcal{E}}] \Pr[\bar{\mathcal{E}}]$.

Working towards that, notice that 
$$\Exp[\exp(x)\mid \bar{\mathcal{E}}]\Pr[\bar{\mathcal{E}}]= \Exp[\exp(x)\mathbf{1}_{\bar{\mathcal {E}}}] = \Exp[\exp(x)\Exp[\mathbf{1}_{\bar{\mathcal {E}}}\vert x]] =  \Exp[\exp(x)r(x)]$$
if we denote $r(x) = \Exp[\mathbf{1}_{\bar{\mathcal{E}}}\vert x]$. We wish to upper bound $\Exp[\exp(x) r(x)]$. By Lemma \ref{lem:abel}, we have 
$$ \Exp[\exp(x) r(x)] \le \Exp[\exp(x) \mathbf{1}_{[t, \infty]}]$$   
where $t$ is such that $\Exp[\mathbf{1}_{[t, \infty]}] = \Exp[r(x)]$. However, since $\Exp[r(x)] = \Pr[\bar{\mathcal{E}}] = \exp(-\Omega(\log^2 d))$, it must be the case that $t = \Omega(\log d)$ by the standard Gaussian tail bound, and the assumption that $\sigma = O(1)$. 
In turn, this means 
$$\Exp[\exp(x) \mathbf{1}_{[t, \infty]}] \le \frac{1}{\sigma \sqrt{2 \pi}}\int_{t}^{\infty} e^{x}e^{-\frac{x^2}{\sigma^2}} dx = 
\frac{1}{\sigma \sqrt{2 \pi}}\int_{t}^{\infty} e^{-(\frac{x}{\sigma} - \frac{\sigma}{2})^2 + \frac{\sigma^2}{4}} dx = 
e^{\frac{\sigma^2}{4}}  \frac{1}{\sqrt{2 \pi}}\int_{t/\sigma}^{+\infty} e^{-(x' - \frac{\sigma}{2})^2} dx' $$ 
where the last equality follows from the change of variables $x = \sigma x'$. However, 
$$ \frac{1}{\sqrt{2 \pi}}\int_{t/\sigma}^{+\infty} e^{-(x' - \frac{\sigma}{2})^2} dx' $$ 
 is nothing more than $\Pr[x' > \frac{t}{\sigma}]$, where $x'$ is distributed like a univariate gaussian with mean $\frac{\sigma}{2}$ and variance 1. Bearing in mind that $\sigma = O(1)$
$$ e^{\frac{\sigma^2}{4}}  \frac{1}{\sqrt{2 \pi}}\int_{t/\sigma}^{+\infty} e^{-(x' - \frac{\sigma}{2})^2} dx' = \exp(-\Omega(t^2)) = \exp(-\Omega(\log^2d))$$ 
by the usual Gaussian tail bounds, which proves the lower bound we need. 

We proceed to consider the lower bound \ref{eq:uph3}. To show the statement of the lemma, we will bound $\Exp[\exp(x) \mid \mathcal{E}]$. Notice trivially that since $\exp(x) \ge 0$, 
$$\Exp[\exp(x) \mid \mathcal{E}] \le \frac{\Exp[\exp(x)]}{\Pr[\mathcal{E}]}  $$ 
Since $\Pr[\mathcal{E}] \ge 1 - \exp(\Omega(\log^2 d))$, $\frac{1}{\Pr[\mathcal{E}]} \le 1 + \exp(O(\log^2))$. So, it suffices to bound $\Exp[\exp(x)]$. However, 
$$\Exp[\exp(x)] = \frac{1}{\sigma \sqrt{2 \pi}}\int_{t = -\infty}^{+\infty} e^{x} e^{-\frac{x^2}{\sigma^2}} dx = \frac{1}{\sigma \sqrt{2 \pi}}\int_{t = -\infty}^{+\infty} e^{-(\frac{x}{\sigma} - \frac{\sigma}{2})^2 + \frac{\sigma^2}{4}} dx = \frac{1}{\sqrt{2 \pi}} \int_{t = -\infty}^{+\infty} e^{-(x' - \frac{\sigma}{2})^2 + \frac{\sigma^2}{4}} dx'$$
where the last equality follows from the same change of variables $x = \sigma x'$ as before. Since 
$ \int_{t = -\infty}^{+\infty} e^{-(x' - \frac{\sigma}{2})^2} dx' = \sqrt{2 \pi} $, we get  
$$\frac{1}{\sqrt{2 \pi}} \int_{t = -\infty}^{+\infty} e^{-(x' - \frac{\sigma}{2})^2 + \frac{\sigma^2}{4}} dx' = e^{\frac{\sigma^2}{4}} = O(1) $$ 
Putting together with the estimate of $\frac{1}{\Pr[\mathcal{E}]}$, we get that $\Exp[\exp(x) \mid \mathcal{E}] = O(1)$. Plugging this back in \ref{eq:uph3}, we get the desired upper bound. 
\end{proof} 
%\Tnote{The proof of Prop 1 should be easier than the proof for the prop below. }
%\Anote{Changed the power of the log.}
\begin{proposition}\label{prop:helper4}
	Suppose  $c \sim \mathcal{C}$ and $v$ is an arbitrary vector with $\|v\| = O(\sqrt{d})$. Then for any event $\mathcal E$ with $\Pr[\mathcal E]\ge 1-\exp(-\Omega(\log^2 d))$, we have that $\Exp[\exp(\inner{v}{c})] = \Exp[\exp(\inner{v}{c})\mid \mathcal{E}] \pm \exp(-\log^{1.8} d)$. 
\end{proposition}

\begin{proof}[Proof of Proposition~\ref{prop:helper4}]
	Let $z = \inner{v}{c}$. We proceed similarly as in the proof of Proposition~\ref{prop:helper3}. We have
	$$ \Exp[\exp(z)] = \Exp[\exp(z)\mid \mathcal{E}]\Pr[\mathcal E] + \Exp[\exp(z)\mid \bar{\mathcal{E}}]\Pr[\bar{\mathcal E}]  $$ 
	and 
	\begin{equation} \Exp[\exp(z)] \le \Exp[\exp(z)\mid \mathcal{E}] + \Exp[\exp(z)\mid \bar{\mathcal{E}}]\Pr[\bar{\mathcal E}] \label{eq:uph4} \end{equation}
	and 
	\begin{equation} \Exp[\exp(z)] \ge \Exp[\exp(z)\mid \mathcal{E}]\Pr[\mathcal E] = \Exp[\exp(z)\mid \mathcal{E}] - \Exp[\exp(z)\mid \mathcal{E}] \exp(-\Omega(\log^2d))\label{eq:lwrh4} \end{equation}  
	We again proceed by separating the upper and lower bound. 
	%Notice that that $\Exp[\exp(z)\mid \mathcal{E}]\Pr[\mathcal E]= \Exp[\exp(z)\mathbf{1}_{\mathcal E}] = \Exp[\exp(z)\Exp[\mathbf{1}_{\mathcal E}\vert z]] =  \Exp[\exp(z)r(z)]$. %Using proposition~\ref{prop:helper5}, we obtain the desired result. \Tnote{Maybe a bit more detail}
%\end{proof}
%
%
%\begin{proposition}\label{prop:helper5}
%	Suppose $x\sim \mathcal{N}(0,\sigma^2)$ with $\sigma \le O(1)$, and $r(x)\in [0,1]$ satisfies that $\Exp[r(x)]  < \exp(\log^2 n)$, then 
%	\begin{equation}
%	\Exp[\exp(z)r(z)]\le = \exp(-\Omega(\log^{1.8}n))
%	\end{equation}
%	\end{proposition}
%	\begin{proof}
%		Let's denote %$r(z) = \Exp[\mathbf{1}_{\overline{\mathcal{F}}}\mid z]$ 
%		$r(z) = \Exp_{c' \mid z} [\mathbf{1}_{\overline{\mathcal{F}}}]$ 
%		which is a function of $z$ between $[0,1]$. 

We first consider the upper bound \ref{eq:uph4}. 

Notice that that 
$$\Exp[\exp(z)\mid \bar{\mathcal{E}}]\Pr[\bar{\mathcal E}]= \Exp[\exp(z)\mathbf{1}_{\bar{\mathcal E}}] $$

We can split the last expression as 
\begin{equation*}
\Exp \left[\expinner{v_w,c} \mathbf{1}_{\langle v_w,c \rangle > 0} \mathbf{1}_{\overline{\mathcal{E}}} \right] + \Exp \left[ \expinner{v_w,c} \mathbf{1}_{\langle v_w,c \rangle < 0} \mathbf{1}_{\overline{\mathcal{E}}} \right]\,.
\end{equation*}
The second term is upper bounded by 
$$\Exp [\mathbf{1}_{\overline{\mathcal{E}}}]\le \exp(-\Omega(\log^2 n))$$ 
We proceed to the first term of (\ref{eqn:eqn21}) and observe the following property of it:
$$ \Exp \left[\expinner{v_w,c} \mathbf{1}_{\langle v_w,c \rangle > 0} \mathbf{1}_{\overline{\mathcal{E}}}\right] \leq \Exp \left[\expinner{\alpha v_w,c} \mathbf{1}_{\langle v_w,c \rangle > 0}\ \mathbf{1}_{\overline{\mathcal{E}}} \right] \leq \Exp \left[\expinner{\alpha v_w,c} \mathbf{1}_{\overline{\mathcal{E}}} \right]$$
where $\alpha > 1$. Therefore, it's sufficient to bound
$$\Exp \left[ \exp(z) \mathbf{1}_{\overline{\mathcal{E}}} \right] $$
when $\|v_w\| = \Theta(\sqrt{d})$.   
Let's denote $r(z) = \Exp[\mathbf{1}_{\bar{\mathcal E}}\vert z]$. 

%Notice that that $\Exp[\exp(z)\mid \bar{\mathcal{E}}]\Pr[\bar{\mathcal E}]= \Exp[\exp(z)\mathbf{1}_{\bar{\mathcal E}}] = \Exp[\exp(z)\Exp[\mathbf{1}_{\bar{\mathcal E}}\vert z]] =  \Exp[\exp(z)r(z)]$, where we denote $r(z) = \Exp[\mathbf{1}_{\bar{\mathcal E}}\vert z]$. 
%
    %We can split that expectation as 
		%$$\Exp_c \left[\exp(z)r(z) \mathbf{1}_{z \geq 0}\right] + \Exp_c \left[\exp(z)r(z)\mathbf{1}_{z < 0}\right] $$ 
		%The second term is upper bounded by 
		%%$$\Exp_c \left[r(z)\right] = \Exp_{c,c'} [\mathbf{1}_{\overline{\mathcal{F}}}]\le \exp(-\Omega(\log^2 n))$$ 
		%$$\Exp_c \left[r(z)\right] = \Pr[\bar{\mathcal E}] = \exp(-\Omega(\log^2 d))$$ 
		%We proceed to the first term, and observe the following property of it:
		%$$ \Exp_c \left[\exp(z)r(z) \mathbf{1}_{z \geq 0}\right] \leq \Exp_c \left[\exp(\alpha z)r(z) \mathbf{1}_{z \geq 0}\right] \leq \Exp_c \left[\exp(\alpha z)r(z)\right]$$
		%where $\alpha > 1$. Therefore, it's sufficient to bound $\Exp_c \left[\exp(z)r(z)\right]$ when $\|v_w\| = \Theta(\sqrt{d})$.  
		Using Lemma~\ref{lem:abel}, we have that
		
		%Evidently, we want to upper bound $\Exp_c \left[\exp(z)r(z)\right]$. We can split that expectation as 
		%$$\Exp_c \left[\exp(z)r(z) \mathbf{1}_{z \geq 0}\right] + \Exp_c \left[\exp(z)r(z)\mathbf{1}_{z < 0}\right] $$ 
		%The second term is upper bounded by 
		%$$\Exp_c \left[r(z)\right] = \Exp_{c,c'} [\mathbf{1}_{\overline{\mathcal{F}}}]\le \exp(-\Omega(\log^2 n))$$ 
		%We proceed to the first term, and observe the following property of it:
		%$$ \Exp_c \left[\exp(z)r(z) \mathbf{1}_{z \geq 0}\right] \leq \Exp_c \left[\exp(\alpha z)r(z) \mathbf{1}_{z \geq 0}\right] \leq \Exp_c \left[\exp(\alpha z)r(z)\right]$$
		%where $\alpha > 1$. Therefore, it's sufficient to bound $\Exp_c \left[\exp(z)r(z)\right]$ when $\|v_w\| = \Omega(\sqrt{d})$.  
		%Using Lemma~\ref{lem:abel}, we have that 
		\begin{equation}
		%\Exp\left[\exp(z)\Exp[\mathbf{1}_{\overline{\mathcal{F}}}\mid z]\right]  = \Exp[\exp(z)r(z)]\le \Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right]
		%\Exp_c[\exp(z)r(z)]\le \Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right]
		\Exp_c[\exp(z)r(z)]\le \Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right]
		\end{equation}
		%\begin{equation}
		%\int_{-\infty}^{\infty}  \exp(z) q(z)dz \le \int_{-\infty}^{\infty}  \exp(z)p(z)\indicator{[t,+\infty]}(z)dz \label{eqn:eqn10}
		%\end{equation}
		where $t$ satisfies that %$\Exp[\mathbf{1}_{[t,+\infty]}] = \Pr[z\ge t] = \Exp[r(z)]$.
		%$\Exp_c[\mathbf{1}_{[t,+\infty]}] = \Pr[z\ge t] = \Exp_c[r(z)] \leq \exp(-\Omega(\log^2 n))$.
		$\Exp_c[\mathbf{1}_{[t,+\infty]}] = \Pr[z\ge t] = \Exp_c[r(z)] \leq \exp(-\Omega(\log^2 d))$.
		%Note that $\Exp[r(z)]= \Exp[\mathbf{1}_{\overline{\mathcal{F}}}]\le \exp(-\Omega(\log^2 n))$. Then, we claim $\Pr[z\ge t] \le \exp(-\Omega(\log^2 n))$ implies that $t \ge \Omega(\log^{.9} n)$.
		%Note that $\Exp_c[r(z)]= \Exp_{c,c'} [\mathbf{1}_{\overline{\mathcal{F}}}]\le \exp(-\Omega(\log^2 n))$. 
		Then, we claim $\Pr[z\ge t] \le \exp(-\Omega(\log^2 d))$ implies that $t \ge \Omega(\log^{.9} d)$.
		%Indeed, to draw a unit vector $c$ from $\mathcal{C}^n$ one can draw $n$ i.i.d. samples $\tilde{c}_i$ from a univariate Gaussian with mean 0 and variance $\frac{1}{n}$, and output $c = (\frac{\tilde{c}_1}{\|\tilde{c}\|}, \frac{\tilde{c}_2}{\|\tilde{c}\|}, \dots, \frac{\tilde{c}_n}{\|\tilde{c}\|})$. It holds that 
		%\begin{equation*} 
		%\Pr[2 \langle v_w, c \rangle  \geq t] = \Pr[2 \langle v_w, \frac{\tilde{c}}{\| \tilde{c} \|} \rangle \geq t] \geq \Pr[2 \langle v_w, \frac{\tilde{c}}{\| \tilde{c} \|} \rangle \geq t | \|\tilde{c} \| \geq \frac{1}{10}] \Pr[\tilde{c} \geq \frac{1}{10}]
		%\end{equation*}   
		%However, $\Pr[\|\tilde{c}\| \geq \frac{1}{10}]$ is lower bounded by a constant by Markov's inequality. Hence, 
		%\begin{equation*}
		%\Pr[2 \langle v_w, \frac{\tilde{c}}{\| \tilde{c} \|} \rangle \geq t | \|\tilde{c} \| \geq \frac{1}{10}] \geq 
		%\end{equation*} 
		%\Anote{Perhaps there's a way to do the next paragraph more cleanly... This is the simplest thing I could think of.}
		%\Anote{The below two claims/lemmas require a lower bound on $\|v_w\|$ on the order of $\sqrt{d}$. Maybe it can be removed... The prior proof also seemed to need it. } 
		
		Indeed, this follows by directly applying Lemma \ref{l:sphericalangle}. 
		%\Tnote{Let's have a separate lemma for things below}
		%Then, by Lemma .... we have 
		%
		%
		% so $\Pr[\frac{\tilde{c}_1}{\|\tilde{c}\|} \geq t \mid \|\tilde{c}\| \leq 100] \geq \Pr[\frac{\tilde{c}_1}{100} \ge \frac{\Omega(e^{-t^2})}{t}]$.      
		%\Anote{Hm.. the above ends up needing that $\|v_w\|$ has reasonable norm, which is true whp, but maybe it's possible to write it in a cleaner way that doesn't require it. }
		%\Tnote{Need to verify the bound for $t$, since $z$ is not simply a Gaussian distribution with variance 4. Note that $c$ is uniform distribution over the shpere. }
		%\Anote{Looks easy, lower priority for now.} 
		%$\int_t^{+\infty}p(z) \le \exp(-\Omega(\log^2 n))$. Note that $z= 2\inner{v_w}{c}$ is a random variable with standard deviation 2, and therefore $p(z) = \frac{1}{\sqrt{8\pi}} \exp(-\frac{1}{8}z^2)$, and we have that $t \ge \Omega(\log^{.9} n)$. Therefore, 
		Afterward, applying Lemma \ref{l:abelspherical}, we have: 
		\begin{equation}
		\Exp[\exp(z)r(z)]\le \Exp\left[ \exp(z)\indicator{[t,+\infty]}(z)\right] = \exp(-\Omega(\log^{1.8}d))
		\end{equation}
		%However, since $d \le n$, the result follows.  
which proves the upper bound we want. 
		
We now proceed to the lower bound \ref{eq:lwrh4}, which is again similar to the lower bound in the proof of Proposition~\ref{prop:helper3}: we just need to bound $\Exp[\exp(z)\mid \mathcal{E}]$. Same as in Proposition~\ref{prop:helper3}, since $\exp(x) \ge 0$, 
$$\Exp[\exp(z) \mid \mathcal{E}] \le \frac{\Exp[\exp(z)]}{\Pr[\mathcal{E}]}  $$ 
Consider the event $\mathcal{E}':z \leq t$, for $t = \Theta(\log^{.9}d)$, which by Lemma \ref{l:sphericalangle} satisfies $\Pr[\mathcal{E}'] \ge 1 - \exp(-\Omega(\log^2d))$. By the upper bound we just showed, 
$$\Exp[\exp(z)] \le \Exp[\exp(z) \mid \mathcal{E}'] + \exp(-\Omega(\log^2n)) = O(\exp(\log^{.9}d)) $$ 
where the last equality follows since conditioned on $\mathcal{E}'$, $z = O(\log^{.9}d)$. Finally, this implies  
$$\Exp[\exp(z) \mid \mathcal{E}] \le \frac{1}{\Pr[\mathcal{E}]}  O(\exp(\log^{.9}d)) = O(\exp(\log^{.9}d)) $$ 
where the last equality follows since $\Pr[\mathcal{E}] \ge 1 - \exp(-\Omega(\log^2n))$. Putting this together with \ref{eq:lwrh4}, we get	
$$ \Exp[\exp(z)] \ge \Exp[\exp(z)\mid \mathcal{E}]\Pr[\mathcal E] = \Exp[\exp(z)\mid \mathcal{E}] - \Exp[\exp(z)\mid \mathcal{E}] \exp(-\Omega(\log^2d)) \ge $$
$$ \Exp[\exp(z)\mid \mathcal{E}] - O(\exp(\log^{.9}d))\exp(-\Omega(\log^2d)) \ge \Exp[\exp(z)\mid \mathcal{E}]  - \exp(-\Omega(\log^2d))$$
which is what we needed.   	
	\end{proof}
%O(\
%\end{proof}\begin{lem}
%Let $v\in \R^d$ be a fixed vector with norm $\sqrt{d}/\kappa\le \|v\| \le \kappa \sqrt{d}$ for constant $\kappa$. Then for random variable $c$ with uniform distribution over the sphere, we have that 
%\begin{equation}
%\log \Exp[\exp(\inner{v}{d})] = \|v\|^2/{2d} \pm \epsilon
%\end{equation}
%where $\epsilon = O(\frac{\log d}{d})$. 
%\end{lem}



==> arxivjul22 copy/experiment.tex <==
%!TEX root = semantic_vector_main.tex
\section{Experimental verification}\label{sec:experiment} 

In this section, we provide experiments empirically supporting our generative model. 

\paragraph{Corpus.}
All word embedding vectors are trained on the English Wikipedia (March 2015 dump). It is pre-processed by standard approach (removing non-textual elements, sentence splitting, and tokenization), leaving about $3$ billion tokens. 
Words that appeared less than $1000$ times in the corpus are ignored, resulting in a vocabulary of $68,430$.
The co-occurrence is then computed using windows of 10 tokens to each side of the focus word. 


\paragraph{Training method.}
Our embedding vectors are trained by optimizing  the \textbf{SN} objective %(\ref{eqn:SNobj}) 
using AdaGrad~\cite{duchi2011adaptive} with initial learning rate of $0.05$ and 100 iterations.  The \textbf{PMI} objective derived from (\ref{eqn:PMI}) was also used. \textbf{SN} has average (weighted) term-wise error of $5$\%, and \textbf{PMI} has $17$\%.  We observed that \textbf{SN} vectors typically fit the model better and have better performance, which can be explained by larger errors in PMI, as implied by Theorem~\ref{thm:main}.  So, we only report the results for \textbf{SN}. 

For comparison, GloVe and two variants of word2vec (skip-gram and CBOW) vectors are trained. 
GloVe's vectors are trained on the same co-occurrence as \textbf{SN} with the default parameter values.\footnote{\url{http://nlp.stanford.edu/projects/glove/}} word2vec vectors are trained using a window size of 10, with other parameters set to default values.\footnote{\url{https://code.google.com/p/word2vec/}}


% figure scale and margin
\newcommand{\scalefac}{0.18}
\newcommand{\hmargin}{-.1in}
\newcommand{\vmargin}{-.0in}

\begin{figure*}
%\captionsetup{font=small}
	\centering
	\hspace{\hmargin}
	\subfigure[\textbf{SN}]{		\includegraphics[height=\scalefac\textwidth]{figure/zc_sq-eps-converted-to}}
	\hspace{\hmargin}
	\subfigure[GloVe]{		\includegraphics[height=\scalefac\textwidth]{figure/zc-eps-converted-to}}
	\hspace{\hmargin}
	\subfigure[CBOW]{	\includegraphics[height=\scalefac\textwidth]{figure/zc_cbow-eps-converted-to}}
	\hspace{\hmargin}
	\subfigure[skip-gram]{		\includegraphics[height=\scalefac\textwidth]{figure/zc_skip-eps-converted-to}}
	\caption{The partition function $Z_c$. The figure shows the histogram of $Z_c$ for $1000$ random vectors $c$ of appropriate norm, as defined in the text. The $x$-axis is normalized by the mean of the values. The values $Z_c$ for different $c$ concentrate around the mean, mostly in $[0.9, 1.1]$. This concentration phenomenon is predicted by our analysis.
	\label{fig:zc}}
	\vspace{-.1in}
\end{figure*} 

\subsection{Model verification}
\label{subs: mverif} 
Experiments were run to test our modeling assumptions. First, we tested two counter-intuitive properties: the concentration of the partition function $Z_c$ for different discourse vectors $c$ (see Theorem~\ref{thm:Z_c}), and the random-like behavior of the matrix of word embeddings in terms of its singular values   (see Theorem~\ref{thm:noise-reduction}).
 For comparison we also 
 %Since these only depend on the inner products between the embedding vectors, the 
 tested these properties for word2vec and GloVe vectors, though they are trained by different objectives. %Therefore, we also tested the two on word2vec and GloVe vectors. 
 Finally, we tested the linear relation between the squared norms of our word vectors and the logarithm of the word frequencies, as implied by Theorem~\ref{thm:main}.

\begin{figure}[!t]
%\captionsetup{font=small}
	\centering
	\includegraphics[height=0.3\columnwidth]{figure/nf_sq-eps-converted-to}
	\caption{The linear relationship between the squared norms of our word vectors and the logarithms of the word frequencies.
		Each dot in the plot corresponds to a word, where $x$-axis is the natural logarithm of the word frequency, and $y$-axis is the squared norm of the word vector. The Pearson correlation coefficient between the two is 0.75, indicating a significant linear relationship, which strongly supports our mathematical prediction, that is, equation~\eqref{eqn:singleword} of Theorem~\ref{thm:main}. %which is implied by our model.
	\label{fig:normVSfreq}
	}
	\vspace{-2mm}
\end{figure} 



\paragraph{Partition function.} Our theory predicts the counter-intuitive concentration of the partition function  $Z_{c} = \sum_{w'} \exp(c^\top v_{w'})$ for a random discourse vector $c$ (see Lemma~\ref{thm:Z_c}). This is verified empirically by picking a uniformly random direction, of norm $\|c\|  = 4/\mu_w$, where $\mu_w$ is the average norm of the word vectors.\footnote{Note that our model uses the inner products between the discourse vectors and word vectors, so it is invariant  if the discourse vectors are scaled by $s$ while the word vectors are scaled by $1/s$ for any $s>0$. Therefore, one needs to choose the norm of $c$ properly. We assume $\|c\| \mu_w = \sqrt{d}/\kappa \approx 4$ for a constant $\kappa = 5$ so that it gives a reasonable fit to the predicted dynamic range of word frequencies according to our theory; see model details in Section~\ref{sec:model}.}
 Figure~\ref{fig:zc}(a) shows the histogram of $Z_c$ for $1000$ such randomly chosen $c$'s for our vectors. The values are concentrated, mostly in the range $[0.9,1.1]$ times the mean.  Concentration is also observed for other types of vectors, especially for GloVe and CBOW.

\paragraph{Isotropy with respect to singular values.} Our theoretical explanation of {\sc relations=lines} assumes that the matrix of word vectors behaves like a random matrix with respect to the properties of singular values.  In our embeddings, the quadratic mean of the singular values is 34.3, while the minimum non-zero singular value of our word vectors is 11. Therefore, the ratio between them is a small constant, consistent with our model. 
The ratios for GloVe, CBOW, and skip-gram are 1.4, 10.1, and 3.1, respectively, which are also small constants.

\paragraph{Squared norms v.s. word frequencies.}  
Figure~\ref{fig:normVSfreq} shows a scatter plot for the squared norms of our vectors and the logarithms of the word frequencies. A linear relationship is observed (Pearson correlation 0.75), thus supporting Theorem~\ref{thm:main}. The correlation is stronger  for high frequency words, possibly because the corresponding terms have higher weights in the training objective.
% have smaller weights and allow larger range of vector norms. Overall, the , indicating a significant linear relationship, thus 
% This aligns with our conclusion, and thus provides positive support for our analysis.

This correlation  %in Figure~\ref{fig:normVSfreq}
 is much weaker for other types of word embeddings. This is possibly because they have more free parameters (\textquotedblleft knobs to turn\textquotedblright), which imbue the embeddings with other properties.
 % For example, GloVe has a similar objective as \textbf{SN}, but the additional bias parameters can affect the word vector norms significantly. 
 This can also cause the difference in the concentration of the partition function for the two methods.


\subsection{Performance on analogy tasks} 
We compare the performance of our word vectors on analogy tasks, specifically the 
two  testbeds GOOGLE and MSR~\cite{mikolov2013efficient,mikolov2013linguistic}.
The former contains $7874$ semantic questions such as ``\emph{man}:\emph{woman}::\emph{king}:??", and $10167$ syntactic ones such as ``\emph{run}:\emph{runs}::\emph{walk}:??."  The latter has $8000$ syntactic questions for adjectives, nouns, and verbs. 
%The algorithm 
%For evaluation, the algorithm should return a ranlist of candidates, and is judged if the
% These questions are answered correctly only if the correct missing term is ranked top $1$.
%We also set up our own testbed \ourtestbed with more difficult questions
%%\footnote{The testbed is available at \\ \url{http://semvec.cs.princeton.edu/PRINCETON.zip}.}. 
%\footnote{The testbed will be made public online.}. 
%It includes $5425$ semantic questions collected from English courses, such as ``\emph{cat}:\emph{kitten}::\emph{river}:??."      
%%Our vocabulary covers about $92\%$ of the GOOGLE questions, $63\%$ of MSR, and $92\%$ of our testbed.
 %These questions  are answered correctly if the missing term is among the top $10$. 

To solve these tasks, we use linear algebraic queries.\footnote{One can instead use the 3COSMUL in~\cite{levy2014linguistic}, which increases the accuracy by about $3\%$. But it is not linear while our focus here is the linear algebraic structure.}
That is, first normalize the vectors to unit norm and then solve ``\emph{a}:\emph{b}::\emph{c}:??''  by 
\vspace{-.1in}
\begin{align}\label{eqn:exp_linearquery}
\argmin_{d} \nbr{v_a - v_b - v_c + v_d}_2^2.%\argmax_{d} \nbr{v_a}_2\inner{v_d}{v_c + v_b -v_a}.
\vspace{-.2in}
\end{align}
The algorithm succeeds if the best $d$ happens to be correct.
\begin{table}
%\captionsetup{font=small}
	\centering
	%{\scriptsize
		\begin{tabular}{c | l | c c c c c c }
		  \hline
			& Relations                             & \textbf{SN}  & GloVe  & CBOW  & skip-gram   \\
			\hline\hline
			\multirow{3}{*}{G}%{\begin{sideways} GOOGLE \end{sideways} }
			& semantic                             &       0.84   &  0.85    &  0.79     & 0.73           \\
			& syntactic                              &       0.61   &    0.65    &  0.71    & 0.68            \\
			& total                                     &        0.71     &    0.73   & 0.74   & 0.70        \\
			\hline\hline
			\multirow{4}{*}{M}%{\begin{sideways} MSR \end{sideways} }
			&    adjective        &     0.50 &  0.56  & 0.58 &    0.58     \\
			& noun                  &      0.69 &  0.70 &  0.56 & 0.58      \\
			& verb                   &      0.48   &    0.53 &   0.64    &0.56 \\
			&  total                    & 0.53   &  0.57       &    0.62    & 0.57   \\
			\hline
			%\begin{sideways} 
			%\ourtestbed  
			%\end{sideways} 
			%S
			%&   total           &      0.57&   0.57 &     0.57    &  0.56               \\
			%\hline\hline
		\end{tabular}
	%}
	\caption{The accuracy on two word analogy task testbeds: G (the GOOGLE testbed); M (the MSR testbed). Performance is close to the state of the art despite using a generative model with provable properties. \vspace{-.15in} } 
	\label{tab:acc}	
\end{table}

The performance of different methods is presented in Table~\ref{tab:acc}.  Our vectors achieve performance comparable to the state of art on semantic analogies (similar accuracy as GloVe, better than word2vec).  On syntactic tasks, they achieve accuracy $0.04$ lower than GloVe and skip-gram, while CBOW typically outperforms the others.\footnote{It was earlier reported that skip-gram outperforms CBOW~\cite{mikolov2013efficient,pennington2014glove}. This may be due to the different training data sets and hyperparameters used.}
%This is not surprising 
%This leads us to believe that our model is better suited for semantics, and lacks specific features 
The reason is probably that our model ignores local word order, whereas the other models capture it to some extent. For example, a word ``\emph{she}'' can affect the context by a lot and determine if the next word is ``\emph{thinks}'' rather than ``\emph{think}''. 
Incorporating  such linguistic features in the model is left for future work.

%Perhaps the main mystery we mention in Section~\ref{sec:interpretability} in the main body stems from the two seemingly contradictory facts that there is high entry-wise error in the optimization, and that the best score only have a small margin over the second best. The first can be observed in the training error: our {\bf SN} objective has average (weighted) termwise error of $5$\%.
%For the second fact, we present in Figure~\ref{fig:gap} a scatter plot of the best and second best scores for the questions in GOOGLE when solved by our method \textbf{SN}. It can be seen that for a significant portion of the questions, the two scores are close to each other. 
%
%\begin{figure}
%\centering
%\includegraphics[width=0.45\columnwidth,natwidth=610,natheight=642]{gap.pdf}	
	%\caption{The scatter plot showing the small gap between the best score and the second best score for all questions in the testbed GOOGLE. The $x$-axis is the best score, the $y$-axis is the second best score, and a ``+'' mark in the plot corresponds to the scores of the answer for an analogy question. The red line is $x=y$. \label{fig:gap} 
	%}
%\end{figure}
 
%\vspace{-4mm}
\subsection{Verifying {\sc relations=lines}}
The theory in Section~\ref{sec:interpretability} predicts the existence of a direction for a relation, whereas  earlier~\citet{levy2014linguistic} had questioned if this phenomenon is real.  The experiment uses the analogy testbed, where each relation is tested using $20$ or more analogies. For each relation, we take the set of vectors $v_{ab} = v_a -v_b$ where the word pair $(a, b)$ satisfies the relation. Then calculate the top singular vectors of the matrix formed by these $v_{ab}$'s, and compute the cosine similarity (i.e., normalized inner product) of individual $v_{ab}$ to  the singular vectors. 
We observed that most $(v_a -v_b)$'s are correlated with the first singular vector, but have inner products around 0 with the second singular vector.  Over all relations, the average projection on the first singular vector is 0.51  (semantic: 0.58; syntactic: 0.46), and the average on the second singular vector is 0.035.
For example, Table~\ref{tab:verifyrd} shows the mean similarities and standard deviations on the first and second singular vectors for 4 relations. 
%Thus most $(v_a -v_b)$'s are correlated with the first singular vector, which can be taken as the direction associated with this relation. The inner products with the second singular vector are centered around 0 with larger deviations, suggesting those components are like random noise, in line with our model. 
%These are also observed for all the other 10 relations in the testbed: the average inner products on the first singular vector are in the range $[0.35, 0.65]$, while those on the second are in the range $[0,0.09]$. 
Similar results are also obtained for word embedings by GloVe and word2vec.
Therefore, the first singular vector can be taken as the direction associated with this relation, while the other components are like random noise, in line with our model. 
%{\sc report the avg correlation of say $20$ relations; that that the phenomenon holds for other relations.}



%Finally, we took a random pair from other relations and computed its similarity to the 1st singular vector. The results are shown in the last row of the table. There are clear gaps between them and those for pairs from the same relation, so it is possible to distinguish between the two.

%\begin{table*}
%\centering
%{\scriptsize
%\begin{tabular}{c|ccccccc}
%\hline 
%relation & 1 & 2 & 3 & 4 & 5 & 6 & 7 \\
%\hline\hline
%on 1st singular vector & 0.65 $\pm$ 0.07 & 0.61 $\pm$ 0.09 & 0.52 $\pm$ 0.08 & 0.54 $\pm$ 0.18 & 0.60 $\pm$ 0.21 & 0.35 $\pm$ 0.17 & 0.42 $\pm$ 0.16 \\
%on 2nd singular vector  & 0.02 $\pm$ 0.28 & 0.00 $\pm$ 0.23 & 0.05 $\pm$ 0.30 & 0.06 $\pm$ 0.27 & 0.01 $\pm$ 0.24 & 0.07 $\pm$ 0.24 & 0.01 $\pm$ 0.25 \\
%\hline
%\end{tabular}
%\begin{tabular}{c|ccccccc}
%\hline
%relation & 8 & 9 & 10 & 11 & 12 & 13 & 14 \\
%\hline\hline
%on 1st singular vector& 0.56 $\pm$ 0.09 & 0.53 $\pm$ 0.08 & 0.37 $\pm$ 0.11 & 0.72 $\pm$ 0.10 & 0.37 $\pm$ 0.14 & 0.40 $\pm$ 0.19 & 0.43 $\pm$ 0.14 \\
%on 2nd singular vector & 0.00 $\pm$ 0.22 & 0.01 $\pm$ 0.26 & 0.02 $\pm$ 0.20 & 0.01 $\pm$ 0.24 & 0.07 $\pm$ 0.26 & 0.07 $\pm$ 0.23 & 0.09 $\pm$ 0.23 \\ 
%\hline
%\end{tabular}
%}
%\caption{The verification of relation directions on 2 semantic relations and 2 syntactic relations in the GOOGLE testbed. For each relation, take $v_{ab} = v_a -v_b$ for word pairs $(a, b)$ in the relation, calculate the top singular vectors of the matrix formed by these $v_{ab}$'s, and compute the cosine similarity of individual $v_{ab}$ to  the singular vectors. The table shows the mean similarity and the standard deviation on the first and second singular vectors. }
%\label{tab:verifyrd}
%\end{table*} 

\begin{table*}
\vspace{5mm}
%\captionsetup{font=small}
\centering
{%\scriptsize
\begin{tabular}{c|ccccccc}
\hline 
relation & 1 & 2 & 3 & 4 & 5 & 6 & 7 \\
\hline\hline
1st & 0.65 $\pm$ 0.07 & 0.61 $\pm$ 0.09 & 0.52 $\pm$ 0.08 & 0.54 $\pm$ 0.18 & 0.60 $\pm$ 0.21 & 0.35 $\pm$ 0.17 & 0.42 $\pm$ 0.16 \\
2nd & 0.02 $\pm$ 0.28 & 0.00 $\pm$ 0.23 & 0.05 $\pm$ 0.30 & 0.06 $\pm$ 0.27 & 0.01 $\pm$ 0.24 & 0.07 $\pm$ 0.24 & 0.01 $\pm$ 0.25 \\
\hline
\end{tabular}
\begin{tabular}{c|ccccccc}
\hline
relation & 8 & 9 & 10 & 11 & 12 & 13 & 14 \\
\hline\hline
1st & 0.56 $\pm$ 0.09 & 0.53 $\pm$ 0.08 & 0.37 $\pm$ 0.11 & 0.72 $\pm$ 0.10 & 0.37 $\pm$ 0.14 & 0.40 $\pm$ 0.19 & 0.43 $\pm$ 0.14 \\
2nd & 0.00 $\pm$ 0.22 & 0.01 $\pm$ 0.26 & 0.02 $\pm$ 0.20 & 0.01 $\pm$ 0.24 & 0.07 $\pm$ 0.26 & 0.07 $\pm$ 0.23 & 0.09 $\pm$ 0.23 \\ 
\hline
\end{tabular}
}
\caption{The verification of relation directions on 2 semantic and 2 syntactic relations in the GOOGLE testbed. Relations include cap-com: capital-common-countries; cap-wor: capital-world; adj-adv: gram1-adjective-to-adverb; opp: gram2-opposite. For each relation, take $v_{ab} = v_a -v_b$ for pairs $(a, b)$ in the relation, and then calculate the top singular vectors of the matrix formed by these $v_{ab}$'s.  The row with label ``1st''/``2nd'' shows the cosine similarities of individual $v_{ab}$ to  the 1st/2nd singular vector (the mean and standard deviation). 
%The row ``cross'' shows the cosine similarities of random pairs from different relations to the 1st singular vector.
}
\label{tab:verifyrd}
\end{table*} 

%\begin{figure}[!t]
%\centering
  %\includegraphics[width=0.7\columnwidth]{inner.pdf}
  %\caption{Relation direction. The $y$ axis indicates the percentage of points with a given inner product--$x$-axis.} \label{fig:relation}
%\end{figure}

%\begin{figure}[!t]
%\centering
  %\includegraphics[width=0.7\columnwidth]{relation_total.pdf}
	%\caption{Accuracy (percentage) of the relation direction method on the GOOGLE testbed, using different number of word pairs for estimation.}\label{fig:relation_analogy}
%\end{figure}


%\begin{table}
%\captionsetup{font=small}
%\centering
%{\scriptsize
%\begin{tabular}{c|c|ccc}
%\hline 
%&  & k=3 & k = 5 & k = 10 \\
%\hline\hline
%\multirow{3}{*}{\textbf{SN}}
 %& semantic & 0.83$\pm$ 0.03  & 0.87$\pm$ 0.04  & 0.90 $\pm$ 0.02 \\
 %& syntactic & 0.58$\pm$ 0.05  & 0.67$\pm$ 0.03  & 0.74$\pm$ 0.01  \\
 %& total & 0.70 $\pm$ 0.04  & 0.76$\pm$ 0.04 & 0.84$\pm$ 0.01 \\
%\hline
%GloVe & total & 0.77$\pm$ 0.02 & 0.82$\pm$ 0.03 & 0.86$\pm$ 0.01 \\
%CBOW & total & 0.79$\pm$ 0.03 & 0.82$\pm$ 0.03  & 0.86$\pm$ 0.01 \\
%skip-gram & total & 0.74$\pm$ 0.02  & 0.77$\pm$ 0.02 & 0.83$\pm$ 0.01\\
%\hline
%\end{tabular}
%}
%\caption{The accuracy of the relation direction method on the GOOGLE testbed. For each relation, take $v_{ab} = v_a -v_b$ for $k$ word pairs $(a, b)$ in the relation, substitute the top singular vector of these $v_{ab}$'s for $v_a -v_b$ in \eqref{eqn:exp_linearquery} when solving the analogy. The table shows the mean accuracy and the standard deviation over 10 runs when using different $k$ and different types of vectors. }
%\label{tab:rdperf}
%\end{table}

%% results using RD methods on GOOGLE
%k & 3 & 4 & 5 & 6 & 7 & 8 \\
%SN & 0.70\pm 0.04  & 0.72\pm 0.04  & 0.76\pm 0.04  & 0.78\pm 0.03  & 0.80\pm 0.02  & 0.82\pm 0.02  & 0.81\pm 0.02  & 0.84\pm 0.01 \\
%GloVe & 0.77\pm 0.02  & 0.78\pm 0.02  & 0.82\pm 0.03  & 0.83\pm 0.02  & 0.84\pm 0.02  & 0.85\pm 0.01  & 0.85\pm 0.02  & 0.86\pm 0.01 \\
%CBOW & 0.79\pm 0.03  & 0.81\pm 0.01  & 0.82\pm 0.03  & 0.83\pm 0.02  & 0.84\pm 0.01  & 0.86\pm 0.02  & 0.86\pm 0.01  & 0.86\pm 0.01 \\
%Skip-gram & 0.74\pm 0.02  & 0.74\pm 0.03  & 0.77\pm 0.02  & 0.78\pm 0.02  & 0.80\pm 0.02  & 0.81\pm 0.02  & 0.81\pm 0.01  & 0.83\pm 0.01


%This then suggests a better (but cheating) way to solve the analogy task with a {\em batched} algorithm. The testbed has many questions for the same relation. Instead of solving them one by one, one can take $v_{ab} = v_a -v_b$ for $k$ pairs $(a,b)$ in the same relation, use the first singular vectors of these $v_{ab}$'s as an estimation of the relation direction, and substitute that for $v_a -v_b$ in \eqref{eqn:exp_linearquery}. We call it the relation direction method.
%Table~\ref{tab:rdperf} shows that its performance on GOOGLE when different number of pairs $k$ and different vectors are used.  For each value of $k$ and  each type of vectors, we randomly sampled $k$ pairs from the same relation, removed the questions that contain any sampled pair, and then computed the accuracy on the left questions. Using our vectors and $k=5$ pairs already leads to $0.87$ accuracy on semantic tasks, $0.67$ on syntactic ones, and $0.76$ overall, with reasonable standard deviation. Comparing with the performance using \eqref{eqn:exp_linearquery} in Table~\ref{tab:acc}, the relation direction method has a clear advantage, especially when $k=10$. 
%It can also be applied with other types of vectors. As shown in Table~\ref{tab:rdperf}, this can achieve similar or better performance. These results support the existence of relation directions, as well as a useful method for solving analogies when a small number of word pairs in the relation are known.

%\begin{table}
%\captionsetup{font=small}
%\centering
%{\scriptsize
%\begin{tabular}{c|c|ccc}
%\hline 
%&  & $k$ = 20 & $k$ = 30 & $k$ = 40 \\
%\hline\hline
%\multirow{1}{*}{\textbf{SN} + \textbf{RD}}
 %& semantic & 0.88 & 0.89 & 0.87 \\
 %& syntactic & 0.64 & 0.72 & 0.68 \\
 %& total & 0.74  & 0.79 & 0.76 \\
%\hline
%GloVe + \textbf{RD}& total & 0.77 & 0.80 & 0.80 \\
%CBOW + \textbf{RD}& total & 0.79 & 0.82 & 0.80\\
%skip-gram + \textbf{RD}& total & 0.75 & 0.80 & 0.77 \\
%\hline
%\end{tabular}
%}
%\caption{The accuracy of \textbf{RD} method on the GOOGLE testbed. Take $v_{ab} = v_a -v_b$ for all word pairs $(a, b)$ and do $k$-means clustering on them. For each $(a,b)$, estimate the relation direction by taking the first singular vector of its cluster, and substitute that for $v_a -v_b$ in \eqref{eqn:exp_linearquery} when solving the analogy.}
%\label{tab:rdperf}
%\end{table}

\begin{table}
%\captionsetup{font=small}
\centering
%{\scriptsize
%\begin{tabular}{c|c|ccc}
%\hline
%\multirow{2}{*}{} & \multirow{2}{*}{w/o \textbf{RD} } & \multicolumn{3}{c}{\textbf{RD}}\\
%\cline{3-5} 
%&  & $k$ = 20 & $k$ = 30 & $k$ = 40 \\
%\hline\hline
%\textbf{SN} & 0.71 & 0.74  & 0.79 & 0.76 \\
%GloVe & 0.73 & 0.77 & 0.80 & 0.80 \\
%CBOW & 0.74 & 0.79 & 0.82 & 0.80\\
%skip-gram & 0.70 & 0.75 & 0.80 & 0.77 \\
%\hline
%\end{tabular}
\begin{tabular}{c|cccc}
\hline 
& \textbf{SN} & GloVe & CBOW & skip-gram \\
\hline\hline
w/o \textbf{RD} & 0.71 & 0.73 & 0.74 & 0.70\\
\hline
\textbf{RD}($k$ = 20) & 0.74 & 0.77 & 0.79 & 0.75 \\
\textbf{RD}($k$ = 30) & 0.79 & 0.80 & 0.82 & 0.80 \\
\textbf{RD}($k$ = 40) & 0.76 & 0.80 & 0.80 & 0.77 \\
\hline
\end{tabular}
%}
\caption{The accuracy of the \textbf{RD} algorithm (i.e., the cheater method) on the GOOGLE testbed. 
The \textbf{RD} algorithm is described in the text.
%\textbf{RD} method: Take $v_{ab} = v_a -v_b$ for all word pairs $(a, b)$ and do $k$-means clustering on them; for each $(a,b)$, estimate the relation direction by taking the first singular vector of its cluster, and substitute that for $v_a -v_b$ in \eqref{eqn:exp_linearquery} when solving the analogy. 
For comparison, the row ``w/o \textbf{RD}'' shows the accuracy of the old method without using \textbf{RD}.}
\label{tab:rdperf}
\end{table}

\paragraph{Cheating solver for analogy testbeds.} The above linear structure suggests a better (but cheating) way to solve the analogy task. This uses the fact that the same semantic relationship (e.g., masculine-feminine,
singular-plural) is tested many times in the testbed. If a relation $R$ is represented by a direction $\mu_R$ then
the cheating algorithm can learn this direction (via rank 1 SVD) after seeing a few examples of the relationship. Then use the following method of solving ``\emph{a}:\emph{b}::\emph{c}:??'': look for a word $d$ such that $v_c -v_d$ has the largest projection on $\mu_R$, the relation direction for $(a,b)$. This can boost success rates by about $10\%$. 

The testbed can try to combat such cheating by giving analogy questions in a random order. But the cheating  algorithm can just {\em cluster}
the presented analogies to learn which of them are in the same relation. 
Thus the final algorithm, named analogy solver with relation direction ($\textbf{RD}$), is: 
take all vectors  $v_a - v_b$ for all the word pairs $(a,b)$ presented among the analogy questions and do $k$-means clustering on them; for each $(a,b)$, estimate the relation direction by taking the first singular vector of its cluster, and substitute that for $v_a -v_b$ in \eqref{eqn:exp_linearquery} when solving the analogy. 
%do $k$-means clustering on all vectors  $v_a - v_b$ for all the word pairs $(a,b)$ presented among the analogy questions, and then learn the direction.  
Table~\ref{tab:rdperf} shows the performance on GOOGLE with different values of $k$; e.g.
using our \textbf{SN} vectors and $k=30$ leads to $0.79$ accuracy.
Thus future designers of analogy testbeds should remember not to test the same relationship too many times!
This still leaves other ways to cheat, such as learning the directions for  interesting semantic relations
from other collections of analogies. 
\iffalse Comparing with the performance using \eqref{eqn:exp_linearquery} in Table~\ref{tab:acc}, the relation direction method has a clear advantage.
It can also be applied with other types of vectors and achieve similar or better performance. These results support the existence of relation directions, as well as a useful method for solving analogies when a batch of analogies need to be solved.
\fi  
 %Leveraging such linear algebraic insights from our model may reduce the data requirement for NLP tasks. This also has implications for future design of testbeds and algorithms: if more than 5 questions for the same analogy relation is given, then it can be solved much better by the relation direction method.
 
\paragraph{Non-cheating solver for analogy testbeds.} Now we show that even if a relationship
is tested only once in the testbed, there is a  way to use the above structure. 
 Given ``\emph{a}:\emph{b}::\emph{c}:??,'' the solver first finds the top $300$ nearest neighbors of $a$ and those of $b$, and then finds among these neighbors the top $k$ pairs $(a',b')$ so that the cosine similarities between $v_{a'} - v_{b'}$ and $v_a - v_b$ are largest. Finally, the solver uses these pairs to estimate the relation direction (via rank 1 SVD), and substitute this (corrected)
 estimate for $v_a -v_b$ in \eqref{eqn:exp_linearquery} when solving the analogy. 
This algorithm is named analogy solver with relation direction by nearest neighbors ($\textbf{RD-nn}$). 
%It is not cheating since it does not use any information beyond word vectors. In particular, it does not require the same relationship is tested many times in the testbed as $\textbf{RD}$.  
Table~\ref{tab:rdnnperf} shows its performance, which consistently improves over the old method by about $3\%$.

\begin{table}
%\captionsetup{font=small}
\centering
%{\scriptsize
\begin{tabular}{c|cccc}
\hline 
& \textbf{SN} & GloVe & CBOW & skip-gram \\
\hline\hline
               w/o \textbf{RD-nn} & 0.71 & 0.73 & 0.74 & 0.70\\
\hline
\textbf{RD-nn} ($k$ = 10) & 0.71 & 0.74 & 0.77 & 0.73 \\
\textbf{RD-nn} ($k$ = 20) & 0.72 & 0.75 & 0.77 & 0.74 \\
\textbf{RD-nn} ($k$ = 30) & 0.73 & 0.76 & 0.78 & 0.74 \\
\hline
\end{tabular}
%}
\caption{The accuracy of the \textbf{RD-nn} algorithm on the GOOGLE testbed. 
The algorithm is described in the text.
For comparison, the row ``w/o \textbf{RD-nn}'' shows the accuracy of the old method without using \textbf{RD-nn}.}
\label{tab:rdnnperf}
\end{table}

==> arxivjul22 copy/generative_model.tex <==
%!TEX root = semantic_vector_main.tex
\section{Generative model and its properties}\label{sec:model}

\newtheorem{model}{Model}
\newcommand{\tv}{\tilde{v}}
\newcommand{\consWordVector}{\Gamma}

The model treats corpus generation as a dynamic process, where the $t$-th word is produced at step $t$. The process is driven by the random walk of a discourse vector $c_t \in \Re^d$. Its coordinates represent what is being talked about.\footnote{This is a different interpretation of the term \textquotedblleft discourse\textquotedblright\ compared to some other settings in computational linguistics.} Each word has a  (time-invariant) latent vector $v_w \in \Re^d$ that captures its correlations with the discourse vector.
% a coordinate could correspond to {\em gender}, with the sign indicating  {\em male/female}. This coordinate %could be positive in $v_{king}$ and negative in $v_{queen}$.
%When the discourse vector has a positive value of the gender coordinate, it should be more likely to produce %words like ``{\em king, man},'' and when it has negative value, favor words like ``{\em queen, woman}.'' 
We model this bias with a log-linear word production model: %(equivalently, product-of-experts): 
\begin{equation} 
\displaystyle 
 \Pr[w~\mbox{emitted at time $t$}~|~c_t] \propto \expinner{c_t,v_w}. \label{eqn:themodel}
\end{equation}

The discourse vector $c_t$ does a slow random walk  (meaning that $c_{t+1}$ is obtained from $c_t$ by adding a small random displacement vector), so that nearby words are generated under similar discourses.
We are interested in the probabilities that word pairs co-occur near each other, so occasional big jumps in the random walk are allowed because they have negligible effect on these  probabilities.
 
A similar log-linear model appears in~\citet{mnih2007three} but without the random walk. 
The linear chain CRF of~\citet{lafferty2001conditional} is more general.
The dynamic topic model of~\citet{blei2006dynamic} utilizes topic dynamics, but with a linear word production model. \citet{belanger2015linear} have proposed a dynamic model for text using Kalman Filters, where the sequence of words is generated from  Gaussian linear dynamical systems, rather than the log-linear model in our case.

The novelty here over such past works is a theoretical analysis  in the method-of-moments tradition~\cite{hsu2012spectral,cohen2012spectral}. 
Assuming a prior on the random walk we analytically integrate out the hidden random variables and compute a simple closed form expression that approximately connects the model parameters to the observable joint probabilities (see Theorem~\ref{thm:main}). This is reminiscent of analysis of similar random walk models in finance~\cite{black1973pricing}.


\paragraph{Model details.}  
Let $n$ denote the number of words and $d$ denote the dimension of the discourse space, where $1\le d\le n$.  %, where $c_1 \log^2 n \le d \le c_2\sqrt{n}$ for some constants $c_1, c_2 > 0$.
Inspecting (\ref{eqn:themodel}) suggests word vectors need to have  varying lengths, to fit the empirical finding that word probabilities satisfy a power law. Furthermore, we will assume that 
in the bulk, the word vectors are distributed uniformly in space, earlier referred to as isotropy. 
This can be quantified as a prior in the Bayesian tradition. More precisely, the ensemble of word vectors consists of i.i.d draws generated by $v =  s \cdot \hat{v}$, where $\hat{v}$ is from the spherical Gaussian distribution, and $s$ is a scalar random variable.
We assume $s$ is a random scalar with expectation $\tau = \Theta(1)$ and 
 $s$ is always upper bounded by $\kappa $, which is another constant. Here $\tau$ governs the expected magnitude of $\inner{v}{c_t}$, %(linearly up to a constant factor $\sqrt{2/\pi}$), 
 and it is particularly important to choose it to be $\Theta(1)$ so that the distribution $\Pr[w\vert c_t] \propto \exp(\inner{v_w}{c_t})$ is interesting.\footnote{A larger $\tau$ will make $\Pr[w\vert c_t]$ too peaked and a smaller one will make it too uniform.} Moreover, the dynamic range of word probabilities will roughly equal $\exp(\kappa^2)$, so one should think of $\kappa$ as an absolute constant like $5$. These details about $s$ are important for realistic modeling but not too important in our analysis. (Furthermore, readers uncomfortable with this simplistic Bayesian prior should look at Section~\ref{sec:weakassumption} below.)

Finally, we clarify the nature of the random walk. We assume that the stationary distribution of the random walk is uniform over the unit sphere, denoted by $\mathcal C$. 
The transition kernel of the random walk can be in any form so long as %the stationary distribution $\mathcal{C}$ of the random walk is uniform on  $[-\frac{1}{\sqrt{d}}, \frac{1}{\sqrt{d}}]^d$, and
at each step the movement of the discourse vector is at most $\epsilon_2/\sqrt{d}$
%$O(1/\log^2 n)$
in $\ell_2$ norm.\footnote{ 
	More precisely, the proof extends to any symmetric product stationary distribution $\mathcal C$ with sub-Gaussian coordinate satisfying $\Exp_{c}\left[\|c\|^2\right] = 1$, and the steps are such that for all $c_t$, $\Exp_{p(c_{t+1}|c_t)}[\exp(\kappa\sqrt{d}\|c_{t+1}-c_t\|)]\le 1+\epsilon_2$ for some small $\epsilon_2$.
}
%\Tnote{Need to check this condition one more time}
This is still fast enough to let the walk mix quickly in the space.  

The following lemma (whose proof appears in the appendix) is central to the analysis. It says that under the Bayesian prior, 
the partition function $Z_c = \sum_{w} \exp(\inner{v_w}{c})$, which is the implied normalization in equation~\eqref{eqn:themodel}, is close to some constant $Z$ for most of the discourses $c$.    
This can be seen as a plausible theoretical explanation of a phenomenon called {\em self-normalization} in log-linear models:  ignoring the partition function or treating it as a constant (which greatly simplifies training) is known to often give good results.  This has also been studied in~\cite{andreas2014when}.

\begin{lem}[Concentration of partition functions]\label{thm:Z_c}
	If the word vectors satisfy the Bayesian prior described in the model details, then 
	\begin{equation}
		\Pr_{c\sim \mathcal{C}}\left[(1-\epsilon_z)Z\le Z_c\le (1+\epsilon_z) Z\right]\ge 1-\delta \label{eqn:lem_zc},
	\end{equation}
	%for any fixed unit vector $c\in \R^d$,  with probability $1-\exp(-\Omega(\log^2 n))$ over the choices of $v_w$'s, we have
	%Let $Z = \Exp[\exp(\inner{v_w,c})\mid |\inner{v_w}{c}| < \frac{1}{2}\log n] $
	%	
	%	
	%	Suppose $\sqrt{n} > d > n^{.01}$, there exists $Z$ such that for any context $c$ with $|\|c\| - 1| \le d^{-0.4}$ , with probability $1-\exp(-\Omega(\log^2 n))$ over the choice of $v_w$'s, 
%	\begin{eqnarray}
%	(1-\epsilon_z)Z\le Z_c\le (1+\epsilon_z) Z\label{eqn:lem_zc}, 
%	\end{eqnarray}
	for $\epsilon_z = \widetilde{O}(1/\sqrt{n})$, and $\delta = \exp(-\Omega(\log^2 n)) $.
\end{lem}
%\begin{equation}
%Z_c = \sum_{w} \exp(\inner{v_w}{c}).
%\end{equation} %Partition function is often difficult to deal with. 
\iffalse Though partition functions are normally difficult to deal with,  in our case we can prove that the values of the partition functions $Z_c$'s typically don't vary much. 
Such concentration of partition function holds empirically, as verified in 

\fi 



%We assume that each coordinate of the hidden discourse vectors $\{c_t\}$ lies in $[-\frac{1}{\sqrt{d}}, \frac{1}{\sqrt{d}}]$.

 %It leads to a training method for the model, and makes it nicely {\em interpretable}.
The concentration of the partition functions then leads to our main theorem (the proof is in the appendix).
The theorem gives simple closed form approximations for $p(w)$, the  probability of word $w$ in the corpus, and $p(w,w')$, the probability that two words $w,w'$ occur next to each other. The theorem states the result for  the window size $q = 2$,  but the same analysis works for pairs that appear in a small window, say of size $10$, as stated in Corollary~\ref{cor:qsize}. 
Recall that $\mbox{PMI}(w, w') = \log [p(w,w')/(p(w)p(w'))]$. 
% and $q$ is the window size within which we count co-occurrences. 
  
  \begin{thm}\label{thm:main}
  	\label{l:pairs} 
  	%There is a constant $Z>0$, and some $\epsilon =\epsilon(n, d)$ that goes to $0$ as $d \rightarrow \infty$  such that with high probability over the choice of word vectors, for any two different words $w$ and $w'$
  	Suppose the word vectors satisfy the inequality~\eqref{eqn:lem_zc}, and window size $q = 2$. Then, 
%  \begin{eqnarray}
%  \log p(w,w')   & = & \frac{\|v_w + v_{w'}\|_2^2 }{2d}- 2\log Z  \nonumber \\
%	&& + \log \left(\frac{q(q-1)}{2}\right) \pm \epsilon,  \label{eqn:twowords_cooc} \\
%  	\log p(w) & = & \frac{\nbr{v_{w}}_2^2}{2d}  - \log Z \pm \epsilon. \label{eqn:singleword}
%  \end{eqnarray}
\begin{align}
	\log p(w,w')   & =  \frac{\|v_w + v_{w'}\|_2^2 }{2d}- 2\log Z  \pm \epsilon,  \label{eqn:twowords_cooc} \\
	\log p(w) & =  \frac{\nbr{v_{w}}_2^2}{2d}  - \log Z \pm \epsilon. \label{eqn:singleword}
\end{align}
for $\epsilon = O(\epsilon_z) +\widetilde{O}(1/d) + O(\epsilon_2)$. %+\exp(-\Omega(\log^{1.8} n))$. 
  Jointly these imply: 
%  \begin{equation}
%   \mbox{PMI}~(w, w') = \frac{\langle v_w, v_{w'}\rangle}{d}  + \log \left(\frac{q(q-1)}{2}\right) \pm O(\epsilon). \label{eqn:PMI}
%   \end{equation}
\begin{equation}
	\mbox{PMI}~(w, w') = \frac{\langle v_w, v_{w'}\rangle}{d}  \pm O(\epsilon). \label{eqn:PMI}
\end{equation}
  \end{thm}

\vspace{2mm}
\noindent
{\bf Remarks 1.} Since the word vectors have $\ell_2$ norm of the order of $\sqrt{d}$,  for two typical word vectors $v_w,v_{w'}$, $\|v_{w}+ v_{w'}\|_2^2$ is of the order of $\Theta(d)$. Therefore the noise level $\epsilon$ is very small compared to the leading term $\frac{1}{2d}\|v_w + v_{w'}\|_2^2$. For PMI however, the noise level $O(\epsilon)$ could be comparable to the leading term, and empirically we also find higher error here.

\vspace{2mm}
\noindent
{\bf Remarks 2.} 
Variants of the expression for joint probability in  (\ref{eqn:twowords_cooc}) had been hypothesized based upon empirical evidence in~\newcite{mikolov2013distributed} and also~~\newcite{globerson2007euclidean}, and~\newcite{DBLP:conf/nips/MaronLB10} . 

\vspace{2mm}
\noindent
{\bf Remarks 3.}
Theorem~\ref{thm:main} directly leads to the extension to a general window size $q$ as follows: %in the remarks that follow. 
\begin{cor}\label{cor:qsize}
	%For window size $q > 2$, equations in Theorem~\ref{thm:main} need to be corrected with constant shift $\gamma = \log \left(\frac{q(q-1)}{2}\right)$:
	Let $p_q(w,w')$ be the co-occurrence probability in windows of size $q$, and $\mbox{PMI}_q(w,w')$ be the corresponding PMI value. Then 
	\begin{align}
	\log p_q(w,w')   & =  \frac{\|v_w + v_{w'}\|_2^2 }{2d}- 2\log Z  + \gamma \pm \epsilon,  \nonumber\\
\mbox{PMI}_{q}~(w, w') &= \frac{\langle v_w, v_{w'}\rangle}{d}  + \gamma \pm O(\epsilon). \nonumber
	\end{align}
	where $\gamma = \log \left(\frac{q(q-1)}{2}\right)$. 
\end{cor}
%\Anote{We should exchange $\exp(-\Omega(\log^2n))$ by $\exp(-\Omega(\log^{1.8}n))$. The proofs in the arxiv version are a bit more conservative. (Though I guess we can get any
%$\exp(-\Omega(\log^{2-\epsilon}n))$ but we should be consistent.
%Additionally, if $\epsilon_z$ is really $\frac{1}{\sqrt{n}}$, $\exp(-\Omega(\log^2n))$ is swallowed by it. Tengyu, did you want to keep this there so we can say if we happen to have better concentration of $Z$, we could get a better bound? In which case, we should say this explicitly.  } 


%(2) When window size $q > 2$, both equation~\eqref{eqn:twowords_cooc} and~\eqref{eqn:PMI} need to be corrected with adding constant $\log \left(\frac{q(q-1)}{2}\right)$ on the right hand sides. 

It is quite easy to see that Theorem~\ref{thm:main} implies the Corollary~\ref{cor:qsize}, as when the window size is $q$ the pair $w,w'$ could appear in any of ${q \choose 2}$ positions within the window, and the joint probability of $w,w'$ is roughly the same for any positions because the discourse vector changes slowly. (Of course, the error term gets worse as we consider larger window sizes, although for any constant size, the statement of the theorem is correct.) This is also consistent with the shift $\beta$ for fitting PMI in~\cite{levy2014neural}, which showed that  
%(2)~\citet{levy2014neural} showed that 
without dimension constraints, the solution to skip-gram with negative sampling satisfies $\mbox{PMI}~(w, w') - \beta =  \langle v_w, v_{w'}\rangle$ for a constant $\beta$ that is related to the negative sampling in the optimization. Our result justifies via a generative model why this should be satisfied even for low dimensional word vectors. 



% We later explain why this error doesn't cause problems in analogy solving in Section~\ref{sec:interpretability}.  


%\iffalse
%\vspace{2mm}
%\noindent
%\Tnote{Should we connect (2.2) and (2.3) to GloVe and Levy-Goldberg and say that we gave a theoretical explanation why their fitting objective makes sense? }
%\Tnote{Commented out the istropic paragraph}
%{\sc to be placed elsewhere}
%{\bf Isotropy and its consequences.} 
%The set of word vectors is said to be {\em isotropic} if the matrix $\Sigma = \sum_{w} v_w v_w^T$ is (close to) a scaling of the identity matrix $I$.  
%Our model's prior implies that the set of word vectors is isotropic, which is useful for our theory that explains the error-resilience phenomenon of the dimension-reduced word vectors  in Section~\ref{sec:interpretability}. We actually require milder isotropic condition (see the first condition of Theorem~\ref{thm:noise-reduction}) and 
%in Section~\ref{sec:experiment} we report that the empirical word vectors discovered using our model are indeed mildly isotropic.
%{\sc up to here}
  %meaning the values $u^\top \Sigma u$ are within a small interval for most vectors $u$.
%\fi

\input{proofsketch}


\subsection{Weakening the model assumptions}  \label{sec:weakassumption}
For readers uncomfortable with Bayesian priors,  we can 
replace our assumptions with  concrete properties of  word vectors that are empirically 
verifiable (Section~\ref{subs: mverif}) for our final word vectors, and in fact also for word vectors computed using other recent methods.
%Readers uncomfortable with Bayesian modeling can take the following alternative view. 

The word meanings are assumed to be represented by some \textquotedblleft ground truth\textquotedblright\ vectors, which the experimenter is trying to recover. These ground truth vectors are assumed to be spatially isotropic in the bulk, in the following two specific ways:
(i) For almost all unit vectors $c$ the sum $\sum_{w} \expinner{v_w,c}$ is close to a constant $Z$; (ii) Singular values of the matrix of word vectors satisfy properties similar to those of random matrices, as formalized in the paragraph before Theorem~\ref{thm:noise-reduction}.
Our Bayesian prior on the word vectors happens to imply that these two conditions hold with high probability. But the conditions may hold even if the prior doesn't hold. Furthermore, they 
are compatible with all sorts of local structure among word vectors such as existence of clusterings, which would be absent in  truly random vectors drawn from our prior.

%These bulk properties have the side benefit of 
%Furthermore, these two deterministic properties are verified empirically in 

%\Tnote{It might be useful to flesh out this point: if the word vector norm has a gaussian distribution or sub-Gaussian tail, then the word frequency has power law} 




==> arxivjul22 copy/inmain-noise.tex <==
%\section{Dimension reduction and error-resilience} \label{sec:noise}

%In this section, we present a formal statement and proof of the meta claim 2 in Section 4. Recall that we have words $a, b$ in a relation $R$. Given a word $\chi$ we define $\zeta_{a,b,R}(\chi)$ as the noise between the log of the co-occurrence ratio and the log of relation functions: $\log\left(\frac{p(\chi\mid a)}{p(\chi \mid b)}\right) = \log(\nu_R(\chi) )+ \zeta_{a,b,R}(\chi)$. Let $\epsilon_{a,b}(\chi) = \log\left(\frac{p(\chi\mid a)}{p(\chi \mid b)}\right) - \frac{1}{d}\inner{v_{\chi}}{v_a-v_b} $ be the fitting error of the word vectors. We also define $\zeta'_{a,b,R} = d(\zeta_{a,b,R} - \epsilon_{a,b,R})$ as the total noise, $\bar{\zeta}_{a,b,R} =(v_a - v_b ) - \mu_R$ as the noise between $(v_a - v_b )$ and the relation vector $ \mu_R $. We have the following theorem:


\begin{thm}[Noise reduction]
\label{thm:noise-reduction}
\iffalse Let $V = P \Sigma Q^T$ be the singular value decomposition of $V$, where $P = [P_1,\dots,P_d]$ are the left singular vectors of $V$ and $(\sigma_1, \sigma_2, \dots, \sigma_d)$ are the non-zero singular values of $V$. We assume that $V$ satisfies: 
\begin{itemize} 
\item $V$ is mildly isotropic: the smallest non-zero singular values of $V$ is larger than constant $c_1$ times the quadratic mean of the singular values, that is, $\|V\|_F/\sqrt{d}$.  
\item The noise vector $\zeta'_{a,b,R}$ is uncorrelated with the left singular vectors --- $\forall i\in [d], |\inner{P_i}{\zeta'_{a,b,R}}|\leq c_2 \frac{\|\zeta'_{a,b,R}\|}{\sqrt{n}}$ for a constant $c_2$. 
\end{itemize} 
Moreover, we assume that the rows of the $V$ (the word vectors) have norm at most $O(\sqrt{d})$. 
Then the
%
\fi
Under the conditions of the previous paragraph, the noise in the dimension-reduced semantic vector space satisfies 
\begin{equation*}
\|\bar{\zeta}_{a,b,R}\|_2 \lesssim \|\zeta'_{a,b,R}\|_2\frac{\sqrt{d}}{n}.
\end{equation*} 
As a corollary, the relative error in the dimension-reduced space is a factor of $\sqrt{d/n}$ smaller. 
%	Let $P = [P_1,\dots,P_d]$ be the left singular vectors of matrix $V$ whose rows are word vectors $\{v_{\chi}\}$. If the word vectors are isotropic and the noise vector $\zeta'_{a,b,R}$ is uncorrelated with the left singular vectors ---$\forall i\in [d], |\inner{P_i}{\zeta'_{a,b,R}}|\lesssim \frac{C\|\zeta'_{a,b,R}\|}{\sqrt{n}}$ for some constant $C$, then the noise in the dimension-reduced semantic vector space satisfies $\|\bar{\zeta}_{a,b,R}\| \lesssim \|\zeta'_{a,b,R}\|\frac{Cd}{n}$.
\end{thm}


 

%\end{document}

==> arxivjul22 copy/interpretability.tex <==
%!TEX root = semantic_vector_main.tex

\section{Explaining {\sc relations=lines}} 
%, analogies and error-resilience}
\label{sec:interpretability}

As mentioned, word analogies like \textquotedblleft $a$:$b$::$c$:??\textquotedblright\ can be  
solved via a linear algebraic expression:
%to solve \textquotedblleft \textquotedblright~recent methods use 
\begin{equation} 
\argmin_{d} \nbr{v_a - v_b - v_c + v_d}_2^2, \label{eqn:query}
\end{equation}
where vectors have been normalized such that $\nbr{v_d}_2=1$. 
This suggests that the semantic relationships being tested in the analogy are characterized by a straight line,\footnote{Note that this interpretation has been disputed; e.g., it is argued in~\newcite{levy2014linguistic} that (\ref{eqn:query}) can be understood using only the classical
connection between inner product and word similarity, using which the objective (\ref{eqn:query}) is slightly improved to a different objective called 3COSMUL. However, this \textquotedblleft explanation\textquotedblright\ is still dogged by the issue of large termwise error pinpointed here, since inner product is only a rough approximation to word similarity. Furthermore, the experiments in Section~\ref{sec:experiment} clearly support the {\sc relations=lines} interpretation.}  referred to earlier as {\sc relations=lines}. 



Using our model we will show the following for low-dimensional embeddings: for each such relation $R$ there is a direction $\mu_R$ in space such that for any word pair $a, b$ satisfying the relation,  $v_a -v_b$  is like $\mu_R$ plus some noise vector. This happens for relations satisfying a certain condition described below.  Empirical results supporting this theory appear in Section~\ref{sec:experiment}, where this linear structure is further leveraged to slightly improve analogy solving. 

A side product of our argument will be a mathematical explanation of the empirically well-established superiority of 
low-dimensional word embeddings over high-dimensional ones in this setting~\cite{levy2014linguistic}. 
As mentioned earlier, the usual explanation that smaller models generalize better is fallacious.
\iffalse But that is fallacious since analogy solving plays no role in the training objective.
Generalization theory does not apply easily to such unsupervised settings,  
and there is no {\em a priori} guarantee that a more succinct solution  will do better at analogy solving
---just as there is no guarantee it will do better at another task like predicting the weather.
\fi

We first sketch what was missing in prior attempts to prove versions of {\sc relations=lines} from first principles.  
The basic issue is approximation error: the difference between the best 
solution and the 2nd best solution to (\ref{eqn:query}) is typically small, 
whereas the approximation error in the objective in the low-dimensional solutions
is larger. For instance, if one uses our {\bf PMI} objective, then the weighted average of the termwise error in~(\ref{eqn:PMI}) is $17\%$, and the expression in (\ref{eqn:query}) above contains six inner products. Thus in principle the approximation error could lead to a failure of the method and the emergence of linear relationship, but it does not.

\paragraph{Prior explanations.}
%We now summarize prior explanations of this phenomenon. 
\citet{pennington2014glove} try to propose a model 
where such linear relationships should occur {\em by design}. 
% to have the property that the embeddings obtained from it solve analogies 
%via the above query~(\ref{eqn:query}). 
They posit that {\em queen} is a solution to the analogy
\textquotedblleft {\em man}:{\em woman}::{\em king}:??\textquotedblright\ because 
\begin{equation} \label{eqn:analogy}
\frac{p(\chi\mid king)}{p(\chi \mid queen)} \approx \frac{p(\chi\mid man)}{p(\chi \mid woman)},
\end{equation}
where $p(\chi\mid king)$ denotes the conditional probability of seeing word $\chi$ in a small window
of text around ${king}$. Relationship (\ref{eqn:analogy}) is intuitive since  both sides  will be $\approx 1$ for gender-neutral $\chi$ like ``{\em walks}'' or ``{\em food}'',  will be $>1$ when $\chi$ is like ``{\em he, Henry}'' and will be $<1$ when $\chi$ is like ``{\em dress, she, Elizabeth}.'' This was also observed by~\citet{levy2014linguistic}.
 Given (\ref{eqn:analogy}), they then posit that the correct model describing word embeddings in terms of word occurrences must be a {\em homomorphism} from $({\Re^d, +})$ to $(\Re^+, \times)$,
 so vector differences map to ratios of probabilities.  This leads to the expression
$$ p_{w,w'} = \inner{v_{w}}{v_{w'}} + b_w + b_{w'},$$
and their method is a (weighted) least squares fit for this expression. 
One shortcoming of this argument is that the homomorphism assumption  {\em assumes} the linear relationships instead of explaining them from a more basic principle. More importantly, 
the empirical fit to the homomorphism has nontrivial approximation error, high enough that  it does not % homomorphism,
%so the two sides of the expression are actually fairly different for most word pairs. 
%Such error is high enough that it is no longer 
%and thus does not 
imply the desired strong linear relationships.
%guaranteed that the desired linear relations in the vectors will appear and be strong enough to 
%needed to explain the success of  (\ref{eqn:query}). 


\citet{levy2014neural} show that empirically, skip-gram vectors satisfy 
\begin{equation}  \inner{v_{w}}{ v_{w'} }\approx \mbox{PMI}(w, w') \label{eqn:pmi2}
\end{equation}
up to some shift.
They also give an argument suggesting this relationship must be present  if the solution is  allowed to be very high-dimensional. Unfortunately, that  argument does not 
extend to low-dimensional embeddings. 
%This relationship is very suggestive of the \textquotedblleft homomorphism\textquotedblright
%property hypothesized by Pennington et al.. 
Even if it did, the issue of termwise approximation error remains.
%
%and so this also does not imply the approximate linear relationships seen in analogy solving.

\paragraph{Our explanation.}
The current paper has introduced a generative model to theoretically explain  the emergence of relationship (\ref{eqn:pmi2}). However, as noted after Theorem~\ref{thm:main}, the issue of high approximation error does not go away either in theory or in the empirical fit.
%empirically nor in theory).  
We now  show that the isotropy of word vectors  (assumed in the theoretical model and verified empirically) implies
that even a weak version of~(\ref{eqn:pmi2}) is enough to imply the emergence of the observed linear relationships in low-dimensional embeddings. 


%This is easily checked by thinking of analogies like ) 
%to assume that low-dimensional vectors will automatically be \textquotedblleft better\textquotedblright than high-dimensional vectors.)

This argument will assume the analogy in question involves a relation that obeys Pennington et al.'s suggestion in (\ref{eqn:analogy}).
%as a working definition of
%a {\em strict semantic relation} between word pairs. (The word \textquotedblleft strict\textquotedblright is supposed to clarify that not all conceivable   semantic relations satisfy this definition, only some, such as the masculine-feminine relation above.) 
%That is, a pair of words are said to have a {\em relation} $R$, which in the above case is {\em %masculine-feminine. }
%In other words, start by positing/observing that a relation $R$ of interest is one where
%for a word pair $a, b$ satisfying it, 
 % their co-occurrences with most other words $\chi$ fit such pattern:
 Namely, for such a relation $R$ there exists  function
$\nu_R(\cdot)$ depending only upon $R$ such that for any $a, b$ satisfying $R$ there is a {\em noise function} $\xi_{a,b,R}(\cdot )$  for which:
	\begin{equation}
	\frac{p(\chi\mid a)}{p(\chi \mid b)} = \nu_R(\chi)\cdot \xi_{a,b,R}(\chi) \label{eqn:relation-mutliplicative}
	\end{equation}
%where $\xi_{a,b,R} > 0$ is a multiplicative noise. 
For different words $\chi$ there is huge variation in (\ref{eqn:relation-mutliplicative}), so the multiplicative noise may be large.

Our goal is to show that the low-dimensional word embeddings have the property that there is a vector $\mu_R$ such that for every pair of words $a, b$ in that relation, $v_{a} - v_{b} = \mu_R + \mbox{noise vector}$, where the noise vector is small.
%({\em This is the mathematical result missing from the earlier papers.})


Taking logarithms of~\eqref{eqn:relation-mutliplicative} results in:
\begin{equation}
	\log\left(\frac{p(\chi\mid a)}{p(\chi \mid b)}\right) = \log(\nu_R(\chi) )+ \zeta_{a,b,R}(\chi)\label{eqn:relationship-log}
\end{equation}
	

Theorem~\ref{thm:main} implies that the left-hand side simplifies to $\log\left(\frac{p(\chi\mid a)}{p(\chi \mid b)}\right) = \frac{1}{d}\inner{v_{\chi}}{v_a-v_b} +\epsilon_{a,b}(\chi)$ where  $\epsilon$ captures the small approximation errors induced by the inexactness of Theorem~\ref{thm:main}. This adds yet more noise! Denoting by $V$ the $n\times d$  matrix whose rows are the $v_{\chi}$ vectors, we rewrite~\eqref{eqn:relationship-log} as:
\begin{equation}
V(v_a-v_b) = d\log(\nu_R) + \zeta'_{a,b,R}\label{eqn:linear-regression}
\end{equation}
where $\log(\nu_R)$ in the element-wise log of vector $\nu_R$ and $\zeta'_{a,b,R} = d(\zeta_{a,b,R} - \epsilon_{a,b,R})$ is the noise. 

In essence,~\eqref{eqn:linear-regression} shows that $v_a -v_b$ is a solution to a linear regression in $d$ variables and $m$ constraints, with $\zeta'_{a, b, R}$ being the \textquotedblleft noise.\textquotedblright\  
\iffalse We can think of $\zeta'_{a,b,R}$ as noise-like and fixed, whereas 
\fi
 The \emph{design matrix} in the regression is $V$, the matrix of all word vectors, which in our model
(as well as empirically) satisfies an isotropy condition. This  makes
it random-like, and thus solving the regression by left-multiplying by $V^{\dagger}$, the pseudo-inverse of $V$,   %(Essentially a random matrix.) 
%Such a regression should be expected 
ought to \textquotedblleft denoise\textquotedblright\
effectively. We now show that it does. 

%Now we use the assumption that word vectors are isotropic, which 
Our model assumed the set of all word vectors satisfies bulk properties similar to a 
set of Gaussian vectors.  
The next theorem will only need the following weaker properties. %implies not only that
%We assume $V$ has %Note that matrix $V$ can be assumed to have 
%full column rank but also that its rows are like random vectors.
%Specifically, we asume the following properties of $V$:
(1) The smallest non-zero singular value of $V$ is larger than some constant $c_1$ times the quadratic mean of the singular values, namely,  $\|V\|_F/\sqrt{d}$. %$V$ is mildly isotropic: the non-zero singular values of $V$ are within a constant $c_1$ from each other. 
Empirically we find $c_1 \approx 1/3$ holds; see Section~\ref{sec:experiment}.
(2) The left singular vectors behave like random vectors with respect to $\zeta'_{a,b,R}$, namely, have inner product at most $c_2 \|\zeta'_{a,b,R}\|/\sqrt{n}$ with  $\zeta'_{a,b,R}$, for some constant $c_2$. 
(3) The max norm of a row in $V$ is $O(\sqrt{d})$.
The proof is included in the appendix. 
 

==> arxivjul22 copy/intro.tex <==
%!TEX root = semantic_vector_main.tex

\begin{abstract}
Semantic word embeddings represent  the meaning of a word via a vector, and are created by diverse methods. Many use nonlinear operations on co-occurrence statistics, and have hand-tuned hyperparameters and reweighting methods.

This paper proposes a new generative model, a dynamic version of the log-linear topic model of~\citet{mnih2007three}.  The methodological novelty is to use the prior to  compute  closed form expressions for word statistics. This provides a theoretical justification for nonlinear models like PMI, word2vec, and GloVe, as well as some hyperparameter choices. It also helps explain why low-dimensional semantic embeddings contain linear algebraic structure that allows solution of word analogies, as shown by~\citet{mikolov2013efficient} and many subsequent papers.
 
Experimental support is provided for the generative model assumptions, the most important of which is  that latent word vectors are fairly uniformly dispersed in space. 
 
\end{abstract}


%\begin{abstract}
%Semantic word embeddings represent  the meaning of a word via a vector, and are created by
%diverse methods such as Latent Semantic Analysis (LSA),  generative text models
%such as topic models, matrix factorization,   neural nets, and energy-based models.  Many methods
%use nonlinear operations ---such as Pairwise Mutual Information (PMI)--- on co-occurrence statistics, and have hand-tuned hyperparameters and reweightings. 
%
%Often a generative model can help provide theoretical insight into such modeling choices,
%but there appears to be no such model to \textquotedblleft explain\textquotedblright\ the above nonlinear models. For example, we know of no generative model for which the correct solution is 
%the usual (dimension-restricted) PMI model.
%
%This paper gives a new generative model, a dynamic version of the loglinear topic model of
%\citet{mnih2007three}. 
 %The methodological novelty is to use the prior to  compute  closed form
 %expressions for word statistics. These provide an explanation for nonlinear models like PMI, word2vec, and GloVe, as well as some hyperparameter choices. 
 %
 %Experimental support is provided for the generative model assumptions, the most important of which is  that latent word vectors are fairly uniformly dispersed (\textquotedblleft isotropic\textquotedblright) in space. 
 %
 %The model also helps explain why low-dimensional semantic embeddings contain linear algebraic structure that allows 
 %solution of word analogies, as shown by~\citet{mikolov2013efficient} and many subsequent papers.
%\end{abstract}


\section{Introduction} \label{sec:intro}
Vector representations of words (word embeddings) try to capture relationships between words as distance or angle, and have many applications in computational linguistics and machine learning. 
They are constructed by various models whose unifying  philosophy is that the meaning of a word is defined by  \textquotedblleft the company it keeps\textquotedblright~\cite{firth1957a}, namely, co-occurrence statistics. The simplest methods use word vectors that explicitly represent co-occurrence statistics.
Reweighting heuristics are known to improve these methods, as is dimension reduction~\cite{deerwester1990indexing}.  Some reweighting methods are nonlinear, which include taking the square root of co-occurrence counts~\cite{rohde2006}, or the logarithm, or 
the related Pointwise Mutual Information (PMI)~\cite{church1990word}.
These are collectively referred to as Vector Space Models, surveyed in~\cite{turney2010frequency}.
%All have the property that similarity of words is captured by the cosine of the angle
%between their embeddings.
% before applying dimension reduction (eg using SVD).

Neural network language models~\cite{hinton1984distributed,rumelhart1988learning,bengio2006neural,collobert2008unified} propose another way to construct embeddings: the word vector is simply the neural network's internal representation for the word. This method is nonlinear and nonconvex. It was popularized via
word2vec, a family of energy-based models in~\cite{mikolov2013distributed,mikolov2013linguistic}, followed by a matrix factorization approach called GloVe~\cite{pennington2014glove}.
The first paper also showed how to solve analogies using linear algebra on word embeddings.
Experiments and theory were used to suggest that these newer methods
are related to the older PMI-based models, but with new hyperparameters and/or
term reweighting methods~\cite{levy2014neural}. 

But note that even the old PMI method is a bit mysterious. The simplest version considers a symmetric matrix with each row/column indexed by a word. The entry for $(w, w')$ 
is $\mbox{PMI}(w, w') =\log \frac{p(w, w')}{p(w)p(w')}$, where 
$p(w, w')$ is the empirical
probability  of words $w, w'$ appearing within a window of
certain size in the corpus,  and $p(w)$ is the marginal probability of $w$. (More complicated models could use 
asymmetric matrices with columns corresponding to context words or phrases, and also involve tensorization.)
Then word vectors are obtained by low-rank SVD on this matrix, or a related matrix with term reweightings.   
In particular, the PMI matrix is found to be closely approximated by a low rank matrix:
there exist word vectors in say $300$ dimensions, which is much smaller than the number of words in the dictionary, such that
\begin{align} \label{eqn:whypmi}
\inner{v_w}{v_{w'}} \approx \mbox{PMI}(w, w')
\end{align}
where $\approx$ should be interpreted loosely.

There appears to be no theoretical explanation for this empirical
finding about the approximate low rank of the PMI matrix. The current paper addresses this.
Specifically, we propose a probabilistic model of text generation that augments the log-linear topic model of~\citet{mnih2007three} with dynamics, in the form of
a random walk over a latent discourse space.  
The chief methodological contribution is using the model priors to analytically derive a closed-form expression that directly explains~(\ref{eqn:whypmi}); see Theorem~\ref{thm:main} in Section~\ref{sec:model}. 
Section~\ref{sec:unification} builds on this insight to give a rigorous justification for
models such as word2vec and GloVe, including the hyperparameter choices for the latter.  
The insight also leads to a mathematical explanation for why these word embeddings allow analogies to be solved using linear algebra; see Section~\ref{sec:interpretability}.
Section~\ref{sec:experiment} shows good empirical fit to this model's assumtions and predictions, including the surprising one that word vectors are pretty uniformly distributed (isotropic) in space.

\subsection{Related work}

Latent variable probabilistic models of language have been used for word embeddings before, including
Latent Dirichlet Allocation (LDA) and its more complicated variants (see the survey~\cite{blei2012probabilistic}), and some neurally inspired nonlinear models~\cite{mnih2007three,DBLP:conf/acl/MaasDPHNP11}. In fact, LDA evolved
out of efforts in the 1990s to provide a generative model that \textquotedblleft explains\textquotedblright\ 
the success of older vector space methods like Latent Semantic Indexing~\cite{Papadimitriouetal98,hofmann1999probabilistic}. However, none of these earlier generative models
has been linked to PMI models.

\citet{levy2014neural} tried to relate word2vec to PMI models. They showed that if there were no dimension constraint in word2vec, specifically, the \textquotedblleft skip-gram with negative sampling (SGNS)\textquotedblright\ version of the model, then its solutions would
satisfy (\ref{eqn:whypmi}), provided 
%if the dimension $d$ were {\em unconstrained} and 
the right hand side
were replaced by $\mbox{PMI}(w, w') -\beta$ for some scalar $\beta$.
%\footnote{To check: Is this 
%trivially true, i.e. is there always a $\beta$ for which this is  positive semidefinite???}. 
However, skip-gram is a discriminative model (due to the use of negative sampling), not generative. Furthermore,  their argument only applies to very high-dimensional word embeddings, and thus does not address low-dimensional embeddings, which have superior quality in applications.
% better than high-dimensional ones in applications.
% and where the {\sc relations=lines} phenomenon is most apparent. 
%is strongly restricted (say, $d =300$). 


%analogy solving and the key role of low dimensionality.  
\citet{hashimoto2016word} focuses on issues similar to our paper. They model text generation as a random walk on words, which are assumed to be embedded as vectors in a geometric space. Given that the last word produced was $w$, the probability that the next word is $w'$ is assumed to be given by
$h(|v_w -v_{w'}|^2)$ for a suitable function $h$,  and this model leads to an explanation of 
(\ref{eqn:whypmi}). 
% somewhat related framed word embedding as metric recovery of a semantic space. They proposed a Markov process model for generating the text where the transition probabilities are determined by the Euclidean distances between the words and showed that in the limit the log co-occurrences of words are consistent with the distances. In contrast,
 By  contrast our random walk involves a latent discourse vector, which has a clearer semantic interpretation and has proven useful in subsequent work, e.g. understanding structure of word embeddings for polysemous words~\newcite{arora2016linear}. Also our work clarifies 
 some weighting and bias terms in the training objectives of previous methods (Section~\ref{sec:unification})
%  better NLP interpretation for the weighting and the bias terms in the training objective. Our %work furthermore provides 
and also the phenomenon discussed in the next paragraph. 
%(Section~\ref{sec:interpretability}), as
%well as the key role played by the number of dimensions being small.

Researchers have tried to understand why vectors obtained from the highly nonlinear word2vec models exhibit linear structures~\cite{levy2014linguistic,pennington2014glove}. Specifically, for analogies like ``\emph{man}:\emph{woman}::\emph{king}:{??},"  \emph{queen} happens to be the word whose vector  $v_{queen}$  is the most similar to the vector $v_{king} -v_{man} + v_{woman}$. This suggests that simple semantic relationships, such as
{\em masculine} vs  {\em feminine} tested in the above example, correspond approximately to a single direction in space, a phenomenon we will henceforth refer to as {\sc relations=lines}.

Section~\ref{sec:interpretability} surveys earlier attempts to explain this phenomenon and their shortcoming, namely, that they ignore the large approximation error in relationships like (\ref{eqn:whypmi}). This error appears larger than the  
difference between the best solution and the second best (incorrect) solution in analogy solving, so that
this error could in principle lead to a complete failure in analogy solving. In our explanation, the low dimensionality 
of the word vectors plays a key role. 
This can also be seen as a theoretical 
explanation of the old observation
that dimension reduction improves the quality of word embeddings for various tasks.
The intuitive explanation often given ---that smaller models generalize better---turns out to be fallacious, since the training method for creating embeddings makes no reference to analogy solving.
Thus there is no a priori reason why low-dimensional model parameters (i.e., lower model capacity) should lead to better performance in analogy solving, just as there is no reason they are better at some other unrelated task like predicting the weather.




%Section~\ref{subsec:genbenefit} will explain the benefits of our generative model approach.
\subsection{Benefits of generative approaches}
\label{subsec:genbenefit}
In addition to giving some form of \textquotedblleft unification\textquotedblright\ of existing methods, our generative model also brings more intepretability to word embeddings beyond traditional cosine similarity and even analogy solving.  For example, it led to an understanding of how
the different senses of a polysemous word  (e.g., {\em bank}) reside in linear superposition within the word embedding~\cite{arora2016linear}.  Such insight into embeddings may prove useful in the numerous settings in NLP and neuroscience where they are used.
%the underlying text. 

Another new explanatory feature of our model is that low dimensionality of word embeddings plays a key theoretical role ---unlike in previous papers where the model is agnostic about the dimension of the embeddings, and the superiority of low-dimensional embeddings is an empirical finding
(starting with~\newcite{deerwester1990indexing}). Specifically, our theoretical analysis makes the key assumption that the set of all word vectors
(which are latent variables of the generative model) are spatially isotropic, which means that
they have no preferred direction in space.  Having $n$ vectors be isotropic in $d$ dimensions 
requires $d \ll n$.
This isotropy is needed in the calculations (i.e., multidimensional integral) that yield~(\ref{eqn:whypmi}). It also holds empirically for our word vectors, as shown in 
Section~\ref{sec:experiment}.  
%(Note that isotropy is a bulk property of the set of all word vectors, and does not 
%preclude clustering or other structure among small subsets of vectors.)  

The isotropy of low-dimensional word vectors also plays a key role in our explanation of the {\sc relations=lines} phenomenon~(Section~\ref{sec:interpretability}). The  isotropy  has  a \textquotedblleft purification\textquotedblright\ effect that  mitigates the effect 
of the (rather large) approximation error in the PMI models.


 %We also need small dimension to explain the emergence of the {\sc relations = lines} phenomenon. 

% (Note that the two vectors may only make an angle of, say, 45 degrees, but that is still a significant overlap in $300$-dimensional space.)  


%This method, in usual topic model tradition, is somewhat insensitive to local word order in a sentence, and therefore does better at capturing semantic relations than syntactic ones (see Section~\ref{sec:experiment}).


==> arxivjul22 copy/proofsketch.tex <==
%!TEX root = semantic_vector_main.tex
\subsection{Proof sketches}
Here we provide the proof sketches, while the complete proof can be found in the appendix. 

\paragraph{Proof sketch of Theorem~\ref{thm:main}}
%For simplicity, we focus on analyzing co-occurrences of words $w,w'$ in a window of size 2. 
%The proof easily extends to larger window sizes. 
Let $w$ and $w'$ be two arbitrary words. Let $c$ and $c'$ denote two consecutive context vectors, where $c\sim \mathcal{C}$ and $c'\vert c$ is defined by the Markov kernel $p(c'\mid c)$.  

We start by using the law of total expectation, integrating out the hidden variables $c$ and $c'$:
\begin{align}
 p(w,w')  & =  \Exp_{c,c'}\left[\Pr[w,w'\vert c,c']\right] \nonumber\\
 & = \Exp_{c,c'}[p(w\vert c)p(w'\vert c')] \nonumber\\
 & = \Exp_{c,c'}\left[  \frac{\expinner{v_w,c}}{Z_c}\frac{\expinner{v_{w'},c'}}{Z_{c'}} \right] \label{eqn:int}
%	\int_{c,c'} p(c,c')\sbr{p(w\vert c)p(w'\vert c')} dcdc'\nonumber \\
	%& =  \int_{c,c'} p(c,c')\frac{\expinner{v_w,c}}{Z_c}\frac{\expinner{v_{w'},c'}}{Z_{c'}} dcdc'  
\end{align}
%\begin{eqnarray*}
% p(w,w') & = & \EE_{c,c'} \sbr{p(w\vert c)p(w'\vert c')} \nonumber \\
%& = & \EE_{c,c'} \sbr{\frac{\expinner{v_w,c}}{Z_c}\frac{\expinner{v_{w'},c'}}{Z_{c'}} }
%\end{eqnarray*}
%where $c$ and $c'$ are the hidden discourse variables that control the emission of two words $w,w'$, and $Z_c = \sum_{w} \expinner{v_w,c}$ is the {\em partition function} that is the implied normalization in equation~\eqref{eqn:themodel}. 

An expectation like~\eqref{eqn:int} would normally be difficult to analyze because of the partition functions. However, we can assume the inequality~\eqref{eqn:lem_zc}, that is, the partition function typically does not vary much for most of context vectors $c$. Let $F$ be the event that both $c$ and $c'$ are within $(1\pm \epsilon_z)Z$. Then by~\eqref{eqn:lem_zc} and the union bound, event $F$ happens with probability at least $1-2\exp(-\Omega(\log^2 n))$. We will split the right-hand side (RHS) of~\eqref{eqn:int} into the parts according to whether $F$ happens or not.  
%(Equation~\eqref{eqn:lem_zc} is in turn established in Lemma~\ref{thm:Z_c}.) 
%showed that 
%in our case we can prove that the values of the partition functions $Z_c$'s typically don't vary much. 
%
%\begin{lemma}\label{thm:Z_c}
%	There exists $Z$ such that with high probability $(1-4\exp(-d^{0.2}))$ over the choice of $v_w$'s and $c$, 
%	\begin{equation}
%	(1-o(1))Z\le Z_c\le (1+o(1)) Z \label{eqn:zc-constant}
%	\end{equation}
%\end{lemma}
%Using this lemma, we get that the right-hand side of~\eqref{eqn:int} equals 
\begin{align}
\textup{RHS of}~\eqref{eqn:int} &= \underbrace{\Exp_{c,c'}\left[  \frac{\expinner{v_w,c}}{Z_c}\frac{\expinner{v_{w'},c'}}{Z_{c'}}\mathbf{1}_{F} \right]}_{T_1}\nonumber\\
&+ \underbrace{\Exp_{c,c'}\left[  \frac{\expinner{v_w,c}}{Z_c}\frac{\expinner{v_{w'},c'}}{Z_{c'}} \mathbf{1}_{\bar{F}}\right]}_{T_2}\label{eqn:eqn1}
\end{align}
where $\bar{F}$ denotes the complement of event $F$ and $\mathbf{1}_{F}$ and $\mathbf{1}_{\bar{F}}$ denote indicator functions for $F$ and $\bar{F}$, respectively. When $F$ happens, we can replace $Z_c$ by $Z$ with a $1\pm \epsilon_z$ factor loss: The first term of the RHS of~\eqref{eqn:eqn1} equals to
\begin{align}
 T_1 = \frac{1\pm O(\epsilon_z)}{Z^2}\Exp_{c,c'}\left[ \expinner{v_w,c}\expinner{v_{w'},c'}\mathbf{1}_{F} \right] \label{eqn:eqn2}
%\frac{1 \pm o(1)}{Z^2} \int_{c,c'} p(c,c')\expinner{v_w,c}\expinner{v_{w'},c'} dcdc' \label{eqn:intz}
%\frac{1 \pm o(1)}{Z^2}\Exp_{c\sim \mathcal{C}}\left[\expinner{v_w+v_{w'},c}\right] .
\end{align}

On the other hand, we can use $\Exp[\mathbf{1}_{\bar{F}}] = \Pr[\bar{F}] \le \exp(-\Omega(\log^2 n))$ to show that the second term of RHS of~\eqref{eqn:eqn1} is negligible,  
\begin{equation}
|T_2| = \exp(-\Omega(\log^{1.8} n))\,. \label{eqn:eqn5}
\end{equation}
%\Tnote{Need to check the exact bound}
This claim must be handled somewhat carefully since the RHS does not depend on $d$ at all. 
%\Tnote{required a bit simplicifation}
Briefly, the reason this holds is as follows: in the regime when $d$ is small ($\sqrt{d} = o(\log^2 n)$), any word vector $v_w$ and discourse $c$ satisfies that $\exp(\langle v_w, c\rangle) \leq \exp(\|v_w\|) = \exp(O(\sqrt{d}))$, and since $\Exp[\mathbf{1}_{\bar{F}}] = \exp(-\Omega(\log^2 n)) $, the claim follows directly; In the regime when $d$ is large ($\sqrt{d} = \Omega(\log^2 n)$), we can use concentration inequalities to show that except with a small probability $\exp(-\Omega(d))= \exp(-\Omega(\log^2 n))$, a uniform sample from the sphere behaves equivalently to sampling all of the coordinates from a standard Gaussian distribution with mean 0 and variance $\frac{1}{d}$, in which case the claim is not too difficult to show using Gaussian tail bounds. 
   
Therefore it suffices to only consider~\eqref{eqn:eqn2}. Our model assumptions state that $c$ and $c'$ cannot be too different. We leverage that by rewriting~\eqref{eqn:eqn2} a little, and get that
it equals
\begin{align}
T_1&= \frac{1 \pm O(\epsilon_z)}{Z^2} \Exp_c\left[\expinner{v_w,c}\Exp_{c'\mid c}\left[\expinner{v_{w'},c'} \right]\right] \nonumber \\
& = \frac{1 \pm O(\epsilon_z)}{Z^2} \Exp_c\left[\expinner{v_w,c}A(c)\right] \label{eqn:eqn3}
\end{align}
where $\displaystyle A(c) :=\Exp_{c'\mid c}\left[\expinner{v_{w'},c'} \right]$. We claim that $\displaystyle A(c) = (1 \pm O(\epsilon_2)) \expinner{v_{w'},c}$.
Doing some algebraic manipulations,  
\begin{align*}
A(c) %&= \Exp_{c'\mid c}\left[\expinner{v_{w'},c'} \right] \\
&=\expinner{v_{w'},c}\Exp_{c'\mid c}\left[\expinner{v_{w'},c'-c} \right].
\end{align*}
%By the fact that the directions of the vectors $v_w$ are Gaussian distributed, one can show that the maximum absolute value of any coordinate 
%of $v_w$ is $\|v_w\|_{\infty} = O(\kappa\log n)$. 
Furthermore,  by our model assumptions, $\|c-c'\| \le \epsilon_2/\sqrt{d}$.  So 
$$ \langle v_{w},c- c'\rangle \le \|v_w\| \|c-c'\| = O(\epsilon_2)$$ 
and thus $\displaystyle A(c) = (1 \pm O(\epsilon_2)) \expinner{v_{w'},c}$. 
%Also note that for any $c_0$, the expectation of $|c' - c|_1$ under the distribution of $c'$ conditioned on $c=c_0$ is small, so that $\EE_{c'|c=c_0}\expinner{v_{w'},c'-c} = 1 \pm o(1)$. 
%This, together
%From our model assumptions the discourses $c,c'$ cannot be very different. 
Plugging the simplification of $A(c)$ to~\eqref{eqn:eqn3}, %combining with decomposition~\eqref{eqn:eqn1}, and ignoring the term 
%\Tnote{Stopped editing here}
\begin{eqnarray}
T_1 = \frac{1 \pm O(\epsilon_z)}{Z^2}\Exp[\expinner{v_w+v_{w'},c}]. \label{eqn:eqn4}
%\frac{1 \pm o(1)}{Z^2}\Exp_{c\sim \mathcal{C}}\left[\expinner{v_w+v_{w'},c}\right] .
\end{eqnarray}
%Since $\mathcal{C}$ is a product distribution, 
Since $c$ has uniform distribution over the sphere, the random variable $\inner{v_w+v_{w'}}{c}$ has distribution pretty similar to Gaussian distribution $\mathcal{N}(0,\|v_w+v_{w'}\|^2/d)$, especially when $d$ is relatively large. Observe that $\Exp[\exp(X)]$ has a closed form for Gaussian random variable $X\sim \mathcal{N}(0,\sigma^2)$, 
\begin{align}
\Exp[\exp(X)] &= \int_x \frac{1}{\sigma\sqrt{2\pi}} \exp(-\frac{x^2}{2\sigma^2}) \exp(x)dx \nonumber\\
%&=\int_x \frac{1}{\sigma\sqrt{2\pi}} \exp(-\frac{(x-\sigma^2)^2}{2\sigma^2} + \sigma^2/2)dx \nonumber\\
&= \exp(\sigma^2/2) \,.\label{eqn:gaussian}
\end{align}

Bounding the difference between $\inner{v_w+v_{w'}}{c}$ from Gaussian random variable, 
%But again, the approximation error must be handled carefully (especially in the low $d$ case), and 
we can show that for $\epsilon = \widetilde{O}(1/d)$, %which is accounted for 
\begin{align}
\Exp[\expinner{v_w+v_{w'},c}] = (1\pm \epsilon ) \exp\left(\frac{\|v_w+v_{w'}\|^2}{2d}\right)\,.
%\pm \epsilon\,. 
\label{eqn:eqn6}
\end{align}

%\Anote{Tengyu, should we add a bit more details on the proof of this claim? This part is not so easy. } 
%a product distribution, by Taylor expanding $\expinner{v,c}$ (considering the coordinates of $v$ as variables) and bounding the terms with order higher than 2, 
%we can show that 
%\begin{align*}
%	p(w,w') & =  \frac{(1 \pm o(1))}{Z^2} \exp(\|v_w + v_{w'}\|_2^2/2d)
%	%\frac{1 \pm o(1)}{Z^2}\Exp_{c\sim \mathcal{C}}\left[\expinner{v_w+v_{w'},c}\right] .
%\end{align*}
%for $v = v_w+v_{w'}$,
%$$\Exp_{c\sim \mathcal{C}}\left[\expinner{v,c}\right] = (1 \pm o(1)) \exp(\|v\|_2^2/2d)$$

Therefore, the series of simplification/approximation above (concretely, combining equations~\eqref{eqn:int},~\eqref{eqn:eqn1},~\eqref{eqn:eqn5},~\eqref{eqn:eqn4}, and~\eqref{eqn:eqn6})  
lead to the desired bound on $\log p(w,w')$ for the case when the window size $q = 2$.
The bound on $\log p(w)$ can be shown similarly.

%What remains is to prove Lemma~\ref{thm:Z_c}. 

\paragraph{Proof sketch of Lemma~\ref{thm:Z_c}}
%Here the crucial fact that we are using that 
Note that for fixed $c$, when word vectors have Gaussian priors assumed as in our model, $Z_c = \sum_{w} \expinner{v_w,c}$ is a sum of independent random variables. 

We first claim that using proper concentration of measure tools, it can be shown that the variance of $Z_c$ are relatively small compared to its mean $\Exp_{v_w}[Z_c]$, and thus $Z_c$ concentrates around its mean. Note this is quite non-trivial: the random variable $\expinner{v_w,c}$ is neither bounded nor subgaussian/sub-exponential, since the tail is approximately inverse poly-logarithmic instead of inverse exponential.  %since the scaling of $w$ and $c$ is such that $\langle v_w,c\rangle$ is $\Theta(1)$,  and therefore $\expinner{v_w,c}$ can be in the non-linear regime reasonably often. 
In fact, the same concentration phenomenon does not happen for $w$. The occurrence probability of word $w$ is not necessarily concentrated because the $\ell_2$ norm of $v_w$ can vary a lot in our model, which allows the frequency of the words to have a large dynamic range. 
%\Tnote{maybe we should remove this: --- In fact, the same concentration phenomenon does not happen for $w$. The occurrence probability of word $w$ is not necessarily concentrated because the $\ell_2$ norm of $v_w$ can vary a lot in our model, which allows the words to have a large dynamic range.}
%\Anote{Alternatively, we can say that the same concentration phenomenon does not happen for $w$, and this is an intended feature of the model. (In fact, at some point we did have something like this, in one of the older versions.)} 

%Briefly, we prove the concentration by carefully truncating the random variable $\inner{v_w}{c}$ at some threshold, and arguing that the probability mass beyond it is irrelevant for our purpose. (Note that our result only works for certain choice of $\delta$, which is more than enough for us. However, the bound of $\delta$ won't get significantly better as typically does for sub-Gaussian or sub-exponential tail. This is exactly the reason why typical concentration inequality doesn't apply.)
 
%It's also necessary to ignore the far tail and only pay attention to the type of concentration that we need, since the whole tail of $Z_c$ is also not sub-exponential %) %%(It's essentially necessary to ignore the very far tail  it will be relevant when a sub-Gaussian or sub-exponential bound for the tail of $Z_c$ is pursued. )
So now it suffices to show that $\E_{v_w}[Z_c]$ for different $c$ are close to each other.
%First, we show that the values $\E_{v_w}[Z_c]$ are close to each other because they are not sensitive to the exact position of $v_w$'s, and in turn are mostly governed by the norms of the $c$'s (which are fairly concentrated around 1). 
Using the fact that the word vector directions have a Gaussian distribution, %and a calculation similar to equation~\eqref{eqn:gaussian}, 
$\Exp_{v_w}[Z_c]$ turns out to only depend on the norm of $c$ (which is equal to 1). %(which are fairly concentrated around 1). 
More precisely, 
\begin{equation}
\Exp_{v_w}[Z_c]  = f(\|c\|_2^2) = f(1)
\end{equation}
where $f$ is defined as $f(\alpha) = n \Exp_{s}[\exp({s}^2\alpha/2)]$ and $s$ has the same distribution as the norms of the word vectors. We sketch the proof of this. 
In our model, $v_w = s_w \cdot \hat{v}_w$, where $\hat{v}_w$ is a Gaussian vector with identity covariance $I$. %, and $s_w$ is the norm of $v_w$. 
Then
\begin{align*}
  \Exp_{v_w}[Z_c] &= n\Exp_{v_w}[\exp(\langle v_w, c\rangle)] \\
	&=n \Exp_{s_w}\left[\Exp_{v_w|s_w}\left[\exp(\langle v_w, c\rangle)\mid s_w\right]\right]
\end{align*}
where the second line is just an application of the law of total expectation, if we pick the norm of the (random) vector $v_w$ first, followed by its direction.  
Conditioned on $s_w$,  $\langle v_w,c \rangle$ is a Gaussian random variable with variance $\|c\|_2^2 s_w^2$, and therefore using similar calculation as in~\eqref{eqn:gaussian}, we have
$$\Exp_{v_w|s_w}\left[\exp(\langle v_w, c\rangle)\mid s_w\right] = \exp({s}^2\|c\|_2^2/2)\,.$$ Hence, 
$\Exp_{v_w}[Z_c] = n \Exp_{s}[\exp({s}^2\|c\|_2^2/2)]$ as needed. 
%\Tnote{Removed the remark that we crucially need $d < \sqrt{n}$. }
%Using more concentration inequalities, we have that the typical $c$ has $\|c\|_2 = 1 \pm o(1)$ and therefore it can be shown that $f(\|c'\|_2^2) \approx f(\|c\|_2^2)$. In summary, we connected $Z_c$ with $Z_{c'}$ by  
%\begin{equation*}
%Z_c \approx \Exp_{v_w}[Z_c]  = f(\|c\|_2^2) \approx  f(\|c'\|_2^2) = \Exp_{v_w}[Z_{c'}]  \approx Z_{c'}
%\end{equation*}

%Bounding the amount of approximation in each step carefully will lead to the desired result as in Lemma~\ref{thm:Z_c}. 
%As assumed in the model, $v_w = s_w \cdot \hat{v}_w$, where $\hat{v}_w$ is a unit Gaussian vector, and $s_w$ is the norm of $v_w$. Then
%\begin{align*}
%  \E_{v_w}[Z_c] &= n\Exp_{v_w}[\exp(\langle v_w, c\rangle)] \\
%	&=n \Exp_{s_w}\left[\Exp_{v_w|s_w}\left[\exp(\langle v_w, c\rangle)\mid s_w\right]\right]
%\end{align*}
%Conditioned on $s_w$, we have that $\langle v_w,c\rangle$ is a Gaussian random variable with variance $\sigma^2 = \|c\|_2^2 s_w^2/d$. Hence, 
%$\Exp_w[Z_c] = n \Exp_{s_w}[\exp(s^2\|c\|_2^2/2)]$. Furthermore, a small calculation shows that with high probability, $\|c\|_2 = 1 \pm o(d^{-0.4})$, which then leads to $\Exp_w[Z_c] =  (1 \pm o(1))n \Exp_{s_w}[\exp(s_w^2/2)]$ as desired.
%
%Then, we use the fact that word vectors have evenly spread directions, being scaled Gaussian vectors, to show that $Z_c$ is close to its mean.  Note this is quite non-trivial: the random variable $\expinner{v_w,c}$ is not subgaussian nor bounded, since the scaling of $w$ and $c$ is such that $\langle v_w,c\rangle$ is $\Theta(1)$,  and therefore $\expinner{v_w,c}$ is in the non-linear regime. 
%% with potentially some non-trivial fluctuations. 
%In fact, the same concentration phenomenon does not happen for $w$. The occurrence probability of word $w$ is not necessarily concentrated because the $\ell_2$ norm of $v_w$ can vary a lot in our model, which allows the words to have a large dynamic range. 
%Finally we note that the concentration bounds crucially use the fact that $d$ is sufficiently small ($O(\sqrt{n})$), so the low-dimensionality is necessary for our main result. 

\iffalse
\vspace{2mm}
\noindent
{\bf Proof Sketch of Main Theorem} \label{sec:theory}
We briefly sketch the proof of Theorem~\ref{thm:main}, and defer the full proof to Section~\ref{sec:proofmain} in the supplementary material.

To derive the expression (\ref{eqn:twowords_cooc}) for $p(w,w')$, we start by marginalizing out the contexts $c,c'$: 
\begin{eqnarray*}
 p(w,w') & = & \EE_{c,c'} \sbr{p(w\vert c)p(w'\vert c')} \nonumber \\
& = & \EE_{c,c'} \sbr{\frac{\expinner{v_w,c}}{Z_c}\frac{\expinner{v_{w'},c'}}{Z_{c'}} }
\end{eqnarray*}
Where $Z_c = \sum_{w} \expinner{v_w,c}$ is the {\em partition function}.
This integral would normally be difficult, because of the appearance of the partition functions. However, we can prove: 
\begin{lemma}\label{thm:Z_c}
	There exists $Z$ such that with high probability $(1-4\exp(-d^{0.2}))$ over the choice of $v_w$'s and $c$, 
	\begin{equation}
	(1-o(1))Z\le Z_c\le (1+o(1)) Z \label{eqn:zc-constant}
	\end{equation}
\end{lemma}
So roughly we have $Z_c \approx Z_{c'}$.
This is only a proof sketch, so suppose the context drifts extremely slowly: with probability extremely close to 1, context $c'$ is equal to $c$. Then, we simplify $p(w,w')$ by just setting $c = c'$: 
\begin{eqnarray*}
p(w,w') & \approx &\frac{1}{Z^2}\Exp_{c\sim \mathcal{C}}\left[\expinner{v_w+v_{w'},c}\right] 
\end{eqnarray*}
(Note that the above can and is made completely formal in Section~\ref{sec:proofmain} of the supplementary material.)
Since we assume $\mathcal{C}$ is a product distribution under which $c$ has expected norm 1, by Taylor expanding we can show 
$\Exp_{c}\left[\expinner{v_w+v_{w'},c}\right] \approx \exp(\|v_w+v_{w'}\|^2/(2d))$, 
which gives us the result we want. 
In an analogous way, we can prove that log occurrence probability of word $w$ is proportional to $\|w\|^2$ up to an $o(1)$ shift. 

Finally, we sketch the proof of Theorem~\ref{thm:Z_c}. We use the fact that word vectors have evenly spread directions, being scaled Gaussian vectors, to show that $Z_c$ is close to its mean. The means of the $Z_c$'s are also close to each other because they mainly depend on the norms of $c$'s, which are fairly concentrated around 1. Note this is all non-trivial: the random variable $\expinner{v_w,c}$ is not subgaussian nor bounded, since the scaling of $w$ and $c$ is such that $\langle v_w,c\rangle$ is $\Theta(1)$,  and therefore $\expinner{v_w,c}$ is in the non-linear regime. 
% with potentially some non-trivial fluctuations. 
In fact, the same concentration phenomenon doesn't happen for $w$. The occurrence probability of word $w$ is not necessarily concentrated because the $\ell_2$ norm of $v_w$ can vary a lot in our model. (This allows the words to have a large dynamic range.) 
We note finally that the concentration bounds crucially use the fact that $d$ is suffuciently small (O($\sqrt{n})$), so the low-dimensionality assumption is necessary for our main result. 
%We also note that since the $\ell_2$ norm of $v_w$ varies a lot, the occurrence probability for $w$, which can be thought as counterpart of partition function for $w$, is %certainly not concentrated. 

%Equipped with Theorem~\ref{thm:Z_c}, we give in the rest of the section a non-rigorous sketch of the proof of  (\ref{eqn:twowords}) in Theorem~\ref{thm:main}. 
\fi



\paragraph{Proof of Theorem~\ref{thm:noise-reduction}}
%The proof is very similar to the analysis of linear regression. We omit the subscript in $\bar{\zeta}$ and $\zeta$ since they are not relevant for this proof. Let $P\Sigma Q^T$ be the SVD of $V$. Since word vectors $\{ v_{\chi} \}$ are isotropic, with our scaling of word vectors we have $V^{\top}V = \frac{n}{d}I$, which implies that $\Sigma =  \sqrt{\frac{n}{d}} I$. Now we have that $\bar{\zeta} = V^{\dagger}\zeta'= Q \Sigma^{-1}P^T\zeta'$. By the first assumption we have $|P^T\zeta'|_{\infty}\le \frac{C}{\sqrt{n}}\|\zeta'\|$ and therefore $\|P^T\zeta'\|^2 \le \frac{C^2d}{n}\cdot \|\zeta'\|^2$. It follows that $\|\bar{\zeta}\|\le \| \Sigma^{-1}P^T\zeta'\| \le \sqrt{\frac{d}{n}} \sqrt{\frac{C^2d}{n}\|\zeta'\|^2} = \frac{Cd}{n}\|\zeta'\|$ as desired. 
The proof uses the standard analysis of linear regression. Let $V = P \Sigma Q^T$
be the SVD of $V$ and let $\sigma_1, \ldots, \sigma_d$
be the left singular values of $V$ (the diagonal entries of $\Sigma$). For notational ease we omit the subscripts in $\bar{\zeta}$ and $\zeta'$ since they are not relevant for this proof. Since $V^{\dagger} = Q\Sigma^{-1}P^T$ and thus $\bar{\zeta} = V^{\dagger}\zeta'= Q\Sigma^{-1}P^T \zeta'$, we have 
\begin{align}
\|\bar{\zeta}\|_2 \le \sigma_d^{-1}\|P^T\zeta'\|_2. \label{eqn:bzeta}
\end{align}

We claim
\begin{align}
\sigma_d^{-1} \le \sqrt{\frac{1}{c_1 n}}. \label{eqn:term1}
\end{align}
Indeed, $\sum_{i=1}^d \sigma^2_i = O(n d)$, since the average squared norm of a word vector is $d$. The claim then follows from the first assumption. 
Furthermore, by the second assumption,
$\|P^T\zeta'\|_{\infty}\le \frac{c_2}{\sqrt{n}}\|\zeta'\|_2$, so
\begin{align}
\|P^T\zeta'\|_2^2 \le \frac{c_2^2 d}{n} \|\zeta'\|_2^2. \label{eqn:term2}
\end{align}


Plugging \eqref{eqn:term1} and \eqref{eqn:term2} into \eqref{eqn:bzeta}, we get 
$$ \|\bar{\zeta}\|_2 \le \sqrt{\frac{1}{c_1 n}} \sqrt{\frac{c^2_2 d}{n}\|\zeta'\|_2^2} = \frac{c_2 \sqrt{d}}{\sqrt{c_1}n}\|\zeta'\|_2$$ 
as desired. 	The last statement follows because the norm of the signal, which is $d \log(\nu_R)$ originally and is $V^{\dagger} d \log(\nu_R) = v_a-v_b$ after dimension reduction, also gets reduced by a factor of $\sqrt{n}$.


==> arxivjul22 copy/unification.tex <==
%!TEX root = semantic_vector_main.tex

\section{Training objective and relationship to other models}
\label{sec:unification}

To get a training objective out of  Theorem~\ref{thm:main}, we reason as follows.
% specifically (\ref{eqn:twowords_cooc}) and (\ref{eqn:PMI}).
% and how they ``explain'' several past methods, and why these methods yield similar vectors.
%Let $\LengthDocument$ be the corpus size, and $X_{w,w'}$ the number of times words $w, w'$ co-occur within a context of size $10$ in the corpus. According to the model, the probability of this event at any particular
%time is $\log p(w,w')  \propto \nbr{v_{w} +  v_{w'}}_2^2.$ Successive samples from a random walk are not 
%independent of course, but if the random walk mixes fairly quickly (and the mixing time of our random walk
%is related to the {\em logarithm} of $n$, the vocabulary size) then the 
%set of $X_{w,w'}$'s over all word pairs is distributed  up to a very close approximation as a multinomial distribution $\mul(\tilde{L}, \{p(w,w')\})$ where $\tilde{L} = \sum_{w,w'} X_{w,w'}$ is the total number of word pairs in consideration (roughly $10 \LengthDocument$). 
Let $X_{w,w'}$ be the number of times words $w$ and $w'$ co-occur within the same window in the corpus. The probability $p(w, w')$ of such a co-occurrence at any particular time is given by (\ref{eqn:twowords_cooc}). Successive samples from a random walk are not independent. But if the random walk mixes fairly quickly (the mixing time is related to the {\em logarithm} of the vocabulary size), then the distribution of $X_{w,w'}$'s is very close to a multinomial distribution $\mul(\tilde{L}, \{p(w,w')\})$, where $\tilde{L} = \sum_{w,w'} X_{w,w'}$ is the total number of word pairs.

Assuming this approximation, we show below that the maximum likelihood values for the word vectors correspond to the following optimization, 
\begin{align} %\label{eqn:SNobj}
\min_{\cbr{v_w}, C} & \sum_{w,w'} X_{w,w'} \rbr{ \log(X_{w,w'}) - \nbr{v_{w}\!+\! v_{w'}}_2^2 - C}^2 \nonumber 
%\\
% & \mbox{\qquad\qquad\qquad\qquad (Objective {\bf SN})}
\end{align}

As is usual, empirical performance is improved by weighting down very frequent word pairs,
possibly because very frequent words such as ``\emph{the}'' do not fit our model.
%found that in order to get better performance, one 
This is done by replacing the weighting $X_{w,w'}$ by its truncation $\min\{X_{w,w'}, X_\text{max}\}$ where $X_\text{max}$ is a constant such as $100$. 
We call this objective with the truncated weights \textbf{SN} ({\bf S}quared {\bf N}orm).

We now give its derivation.
Maximizing the likelihood of $\{X_{w,w'}\}$ is equivalent to maximizing
\begin{align*}
\ell & = \log\left(\prod_{(w, w')} p(w, w')^{X_{w,w'}} \right).
\end{align*}
Denote the logarithm of the ratio between the expected count and the empirical count as
\begin{align}
\Delta_{w,w'} = \log\left(\frac{\tilde{L} p(w, w')  }{ X_{w,w'} } \right).   \label{eqn:deltadefn}
\end{align}
Then with some calculation, we obtain the following where  $c$ is independent of the empirical observations $X_{w,w'}$'s.
\begin{align}
 \ell & =  c  +   \sum_{(w, w')}   X_{w,w'}  \Delta_{w,w'} \label{eqn:likelihood}
\end{align}


On the other hand, using $e^x \approx 1+x+x^2/2$ when $x$ is small,\footnote{This Taylor series approximation has an error of the order of $x^3$, but  ignoring it can be theoretically justified as follows. For a large $X_{w,w'}$, its value approaches its expectation and thus the corresponding $\Delta_{w,w'}$  is close to 0 and thus ignoring $\Delta_{w,w'}^3$ is well justified. The terms where $\Delta_{w,w'}$ is significant correspond to $X_{w,w'}$'s that are small.  But empirically, $X_{w,w'}$'s obey a power law distribution (see, e.g.~\newcite{pennington2014glove}) using which it can be shown that these terms  contribute a small fraction of the final objective (\ref{eqn:finalexpresion}). So we can safely ignore the errors. Full details appear in the ArXiv version of this paper~\cite{AroLiLiaMaetal15}.} we have
\begin{align*}
\tilde{L} 
& = \sum_{(w,w')} \tilde{L} p_{w,w'}  = \sum_{(w,w')} X_{w,w'} e^{\Delta_{w,w'} } \\
& \approx \sum_{(w,w')}  X_{w,w'} \left(1 + \Delta_{w,w'} + \frac{\Delta_{w,w'}^2}{2}\right).
\end{align*}
Note that $\tilde{L} = \sum_{(w,w')} X_{w,w'}$, so 
\begin{align*}
 \sum_{(w,w')}  X_{w,w'} \Delta_{w,w'}  \approx  - \frac{1}{2}\sum_{(w,w')}  X_{w,w'} \Delta_{w,w'}^2.
\end{align*}
Plugging this into (\ref{eqn:likelihood}) leads to
\begin{align}
2(c - \ell)  \approx \sum_{(w,w')}  X_{w,w'} \Delta_{w,w'}^2. \label{eqn:finalexpresion}
\end{align}
So maximizing the likelihood is approximately equivalent to minimizing the right hand side, which (by examining (\ref{eqn:deltadefn})) leads to our objective.


\iffalse 
(The reason this is not exact is that 
%(This is valid since the correlation between the counts $X_{w, w'} {\sc say something}.)

For any pair $(a, b)$ such that $ X_{a, b} \not= 0$, it holds that:


 \begin{eqnarray}\label{eq:weight}&& = \log\left( C_1  \left(\prod_{(w, w') \not= (a,b )}p(w,w')^{X_{w, w'}}\right) \left( 1- \sum_{(w, w') \not= (a,b )} p(w, w') \right)^{X_{a, b}} \right)
  \end{eqnarray}
Where $C_1$ is the number of documents of size $\LengthDocument$ such that co-occurence count of each $w, w'$ is $X_{w, w'}$. 

Substituting $ x_{w, w'} = \log[ \LengthDocument p(w,w')] $, we have: 
$$\log \Pr[\{X_{w, w'} \} \mid \{ p(w, w') \}]  = \log C_1 -  \LengthDocument \log \LengthDocument +  \frac{1}{\LengthDocument}\left(\sum_{(w, w') \not= (a,b )} X_{w, w'}   x_{w, w'}  \right)+ X_{a, b} \log  \left( 1- \sum_{(w, w') \not= (a,b )} p_{w, w'} \right)$$
 
The last term can be expanded as follows:
 \begin{eqnarray*}
&&  \log  \left( 1- \sum_{(w, w') \not= (a,b )} p_{w, w'} \right) =   \log  \left( 1- \frac{1}{\LengthDocument}\sum_{(w, w') \not= (a,b )} e^{x_{w, w'}}  \right) 
  \\
  &&= \log  \left( 1- \frac{1}{\LengthDocument}\sum_{(w, w') \not= (a,b )}X_{w, w'} e^{x_{w, w'} - \log X_{w, w'} }  \right) 
  \\
  &&=  \log  \left( 1- \frac{1}{\LengthDocument}\sum_{(w, w') \not= (a,b )}X_{w, w'} \left(1 + [x_{w, w'} - \log X_{w, w'}  ]+ [x_{w, w'} - \log X_{w, w'} ]^2/2 + O([x_{w, w'} - \log X_{w, w'} ]^3)\right)  \right) 
  \\
  &&= \log \left( X_{a, b} - \frac{1}{\LengthDocument} \sum_{(w, w') \not= (a,b )}X_{w, w'} \left([x_{w, w'} - \log X_{w, w'}  ]+ [x_{w, w'} - \log X_{w, w'} ]^2/2 + O([x_{w, w'} - \log X_{w, w'} ]^3)\right)  \right)
  \\
  &&= \log X_{a, b} +  \log \left( 1- \frac{1}{\LengthDocument X_{a,b}} \sum_{(w, w') \not= (a,b )}X_{w, w'} \left([x_{w, w'} - \log X_{w, w'}  ]+ [x_{w, w'} - \log X_{w, w'} ]^2/2 + O([x_{w, w'} - \log X_{w, w'} ]^3)\right)  \right)
  \\
  &&= \log X_{a, b}  - \frac{1}{\LengthDocument X_{a,b}} \sum_{(w, w') \not= (a,b )}X_{w, w'} \left([x_{w, w'} - \log X_{w, w'}  ]+ [x_{w, w'} - \log X_{w, w'} ]^2/2 + O([x_{w, w'} - \log X_{w, w'} ]^3)\right)  
  \\
  && \quad + O\left(\frac{1}{\LengthDocument^2 X_{a,b}^2} \left(\sum_{(w, w') \not= (a,b )}X_{w, w'} (x_{w, w'} - \log X_{w, w'}  )\right)^2 \right)
 \end{eqnarray*}


Putting this into \ref{eq:weight}, we get
\begin{eqnarray*}
&& = C - \frac{1}{2\LengthDocument} \left( \sum_{w, w' } X_{w, w'}(x_{w, w'} - \log X_{w, w'} )^2 \right) 
\\
&&+ O \left(  \frac{1}{\LengthDocument} X_{a, b}(x_{a, b} - \log X_{a, b})^2  +\frac{1}{\LengthDocument}\sum_{w, w'} X_{w, w'}(x_{w, w'} - \log X_{w, w'} )^3 + \frac{1}{\LengthDocument^2} \left( \sum_{w, w'}X_{w, w'} (x_{w, w'} - \log X_{w, w'}  )\right)^2 \right)
\end{eqnarray*}

\fi

\iffalse
%{\sc give the likelihood calculation!! also explain the remark about PMI}

Now we give the derivation of (\ref{eqn:SNobj}).
%Let $u_{w, w'}$ be the empirical estimate of $p_{w, w'}$, namely $X_{w, w'}/L$. 
%
According to the multinomial distribution, the probability of seeing the counts $\{X_{w,w'}\}$ is
\begin{equation}
C \prod_{(w, w')} p(w, w')^{X_{w,w'}} 
\label{eq:likelihood}
\end{equation}
where $C = {\frac{\tilde{L}!} {\Pi_{(w,w')} X_{w,w'}!}}$ is a multinomial coefficient that doesn't depend upon $p(w,w')$ and can
be treated as constant in the optimization. 
Noting that the $p(w,w')$'s sum to $1$, picking any arbitrary $(a, b)$ such that $ X_{a, b} \not= 0$ (and hence 
$p(a,b) \neq 0$) we can rewrite (\ref{eq:likelihood}) 
\begin{multline*}
C \left( 1-\sum_{(w,w') \neq (a,b)} p(w,w')\right)^{X_{a,b}} \\ 
\prod_{(w, w') \neq (a, b)} p(w, w')^{X_{w,w'}}
\end{multline*}
%Using ?? this is simplified to ??

%{\sc didn't understand this notation/proof at all.}


%Actually in the experiments we ignore words that appear less than a few hundred times. For the remaining
%words $X_{w, w'} \approx 
\iffalse 
% \log \Pr\sbr{\{X_{w, w'} \} \mid \{ p(w, w') \}} = $$ 
\begin{multline*} 
\log \Biggl(\left(\prod_{(w, w') \not= (a,b )}p(w,w')^{X_{w, w'}}\right) \\ 
\left( 1- \sum_{(w, w') \not= (a,b )} p(w, w') \right)^{X_{a, b}} \Biggr)
\end{multline*} 
\fi   
 Taking logarithm of this likelihood and ignoring the terms which do not depend on $p(w,w')$ we conclude the maximum likelihood solution maximizes the following objective, where $u_{w, w'} = \log[ \tilde{L} p(w,w')] $: 
%where $C_1$ is the number of documents of size $\LengthDocument$ such that co-occurence count of each $w, w'$ is $X_{w, w'}$. 
%Substituting $ x_{w, w'} = \log[ \LengthDocument p(w,w')] $, we have: 
%$$ \log \Pr\sbr{\{X_{w, w'} \} \mid \{ p(w, w') \} }   = $$ 
\begin{multline}  
\left(\sum_{(w, w') \not= (a,b )} X_{w, w'}   u_{w, w'}  \right) \\
 + X_{a, b} \log  \left( 1- \sum_{(w, w') \not= (a,b )} p(w, w') \right) 
 \label{eq:weights}
\end{multline} 

Rewriting $\log  \left( 1- \sum_{(w, w') \not= (a,b )} p(w, w') \right)$ by writing $p(w,w') = \exp(u_{w,w'})/\tilde{L}$, we get that it equals
 % $$ \log  \left( 1- \sum_{(w, w') \not= (a,b )} p_{w, w'} \right) = $$
 % $$ \log  \left( 1- \frac{1}{\LengthDocument}\sum_{(w, w') \not= (a,b )} e^{x_{w, w'}}  \right) = $$
  $$ \log\left( 1- \frac{1}{\tilde{L}}\sum_{(w, w') \not= (a,b )}X_{w, w'} \exp(u_{w, w'} - \log X_{w, w'} )  \right) $$
  
 Since $g_{w,w'} = u_{w, w'} - \log X_{w, w'} $  is expected to be small we use the approximation $e^{x} \approx 1 + x + \frac{x^2}{2}$ to obtain:  % the last expression is approximately 
 \small
 \begin{multline}  
 \log  \left( 1- \frac{1}{\tilde{L}}\sum_{(w, w') \not= (a,b )}X_{w, w'} (1 + g_{w,w'} + \frac{g^2_{w,w'}}{2})\right) = \\
 % [x_{w, w'} - \log X_{w, w'}  ]+ [x_{w, w'} - \log X_{w, w'} ]^2/2 )  \bigr) = \\
 \log \left( \frac{X_{a, b}}{\tilde{L}}\right) +  \log \left( 1- \frac{1}{X_{a,b}} \sum_{(w, w') \not= (a,b )}X_{w, w'} \left(  g_{w,w'} + \frac{g^2_{w,w'}}{2} \right) \right)\\
 \label{eq:weight-intermediate}
 %\left([x_{w, w'} - \log X_{w, w'}  ]+ [x_{w, w'} - \log X_{w, w'} ]^2/2 \right)  \bigr)
 \end{multline}
 \normalsize
 where we have used $X_{a,b} = \tilde{L} -\sum_{(w, w') \not= (a,b )}X_{w, w'}$. Now
 we claim we can use the approximation $\log(1+x) \approx x$ for the latter term. Indeed, with some algebraic manipulation and using  $p(w,w') = X_{w,w'} \exp(u_{w,w'} - \log X_{w,w'}) $ we get:   
 $$\sum_{(w,w') \neq (a,b)} X_{w,w'} \left(g_{w,w'} + \frac{g^2_{w,w'}}{2}\right)  $$ 
 $$ \approx \sum_{(w,w') \neq (a,b)} \left(\tilde{L} p(w,w') - X_{w,w'}\right) $$
 $$= \tilde{L} \left(1-p(a,b)\right) - (\tilde{L}-X_{a,b}) = X_{a,b} - \tilde{L}  p(a,b) $$ 
 
 Hence,
  $\frac{1}{X_{a,b}} \sum_{(w, w') \not= (a,b )}X_{w, w'} \left(  g_{w,w'} + \frac{g^2_{w,w'}}{2} \right) \approx 1 - \frac{\tilde{L} p(a,b)}{X_{a,b}}$.
 Picking an $(a,b)$ s.t. $X_{a,b}$ is close to its expectation $\tilde{L} p(a,b)$, we expect $1 - \frac{\tilde{L} p(a,b)}{X_{a,b}}$ to be small. With that in mind, (\ref{eq:weight-intermediate}) simplifies to
 \small       
 \begin{multline*}  
 \hspace*{-0.8cm}
 \log \left(\frac{X_{a, b}}{\tilde{L}}\right)  - \frac{1}{X_{a,b}} \sum_{(w, w') \not= (a,b )}X_{w, w'} \left(g_{w,w'} + \frac{g^2_{w,w'}}{2}\right)\\ 
  %\left([x_{w, w'} - \log X_{w, w'}  ]+ [x_{w, w'} - \log X_{w, w'} ]^2/2  \right)  
 \end{multline*} 
 \normalsize
Plugging this back into (\ref{eq:weights}), we get that maximizing $ \log \Pr[\{X_{w, w'} \} \mid \{ p(w, w') \}] $ is equivalent to minimizing
$$ \sum_{w, w' } X_{w, w'}(u_{w, w'} - \log X_{w, w'} )^2  $$
which implies that the objective (\ref{eqn:SNobj}) is equivalent to maximizing the likelihood. 
%Notice also the terms dropped when keeping the high-order Taylor terms are typically very small.   
\fi


\paragraph{Objective for training with PMI.}
A similar objective {\bf PMI} can be obtained from (\ref{eqn:PMI}), 
by computing an approximate MLE, using the fact that the error between the empirical and true value of $\mbox{PMI}(w, w')$ is driven by the smaller term $p(w,w')$, and not the larger terms $p(w), p(w')$.

\begin{align*} %\label{eqn:PMIfit}
\min_{\cbr{v_w}, C} & \sum_{w,w'} X_{w,w'} \rbr{\mbox{PMI}(w, w') - \inner{v_{w}}{v_{w'}}}^2 
\end{align*}
This is of course very analogous to classical VSM methods, with a novel reweighting method. 
% and was recently also suggested for analogy solving~\cite{levy2014linguistic}. We do not know if the  precise weighting $X_{w,w'}$ was explored before. 
%This model also works well and explains the earlier empirical findings of Levy and Goldberg. 

Fitting to either of the objectives involves solving a version of {\em Weighted SVD} which is NP-hard, but empirically seems solvable in our setting via AdaGrad~\cite{duchi2011adaptive}.
%$\min \sum_{w,w'} X_{w,w'} (v_w \cdot v_{w'} - \mbox{PMI}(w, w'))^2$.
% which we denote by
%{\bf PMI}.


\paragraph{Connection to GloVe.}
Compare  \textbf{SN} with the objective used by GloVe~\cite{pennington2014glove}:
\begin{equation*} %\label{eqn:glove1} 
\sum_{w,w'} f(X_{w,w'})( \log(X_{w,w'}) - \inner{v_w}{v_{w'}} - s_w - s_{w'} - C)^2
\end{equation*} 
with $f(X_{w,w'}) = \min\{ X_{w,w'}^{3/4}, 100\}.$
Their weighting methods and the need for {\em bias} terms $s_w, s_{w'},C$ were derived by trial and error; here
they are all predicted and given  meanings due to Theorem~\ref{thm:main}, specifically 
$s_w = \nbr{v_w}^2$. 
%In particular, our objective has essentially no \textquotedblleft knobs to turn.\textquotedblright 

%is very close to the matrix factorization objective used by~\citet{pennington2014glove}, which has %a couple of additional {\em bias} terms, and a slightly more complicated weighting (apparently derived by trial and error; our experiments also show slight changes of weighting are OK). 
%In the context of classical VSM methods, this can be seen as an SVD-like objective with a weighting %term $X_{w,w'}$, and matrix entries $\log(X_{w, w'}) - C$, where $C$ is a scalar. 




\paragraph{Connection to word2vec(CBOW).} 
The CBOW model in word2vec posits that the probability of a word $w_{k+1}$ as a function of the previous $k$ words $w_1, w_2, \ldots, w_k$:
$$
   p\rbr{ w_{k+1} \big|\cbr{w_i}_{i=1}^{k}} \propto \expinner{v_{w_{k+1}},  \frac{1}{k}\sum_{i=1}^{k} v_{w_i} }.
$$


This  expression seems mysterious since it depends upon the {\em average} word vector for the previous $k$ words. We show it  can be theoretically justified. Assume a simplified version of our model, where a small window of $k$ words is generated as follows: sample $c \sim \mathcal{C}$, where $\mathcal{C}$ is a uniformly random unit vector, then sample $\left(w_1, w_2, \dots, w_k\right) \sim \expinner{\sum^k_{i=1} v_{w_i}, c}/Z_c$. Furthermore, assume $Z_c = Z$ for any $c$.  
\begin{lem} In the simplified version of our model, the Maximum-a-Posteriori (MAP) estimate of $c$ given $\left(w_1, w_2, \dots, w_k\right)$ is $\frac{\sum_{i=1}^k v_{w_i}}{\|\sum_{i=1}^k v_{w_i} \|_2}$. 
\end{lem} 
\begin{proof} 
The $c$ maximizing $ p\rbr{ c | w_1, w_2, \dots, w_k } $ is the maximizer of $p(c) p\rbr{ w_1, w_2, \dots, w_k |c }$.
Since $p(c) = p(c')$ for any $c,c'$, and we have 
$
  p\rbr{ w_1, w_2, \dots, w_k | c } = \expinner{\sum_i v_{w_i}, c }/Z,
$ 
the maximizer is clearly $c = \frac{\sum_{i=1}^k v_{w_i}}{\|\sum_{i=1}^k v_{w_i} \|_2}$. 
\end{proof} 
Thus using the MAP estimate of $c_t$ gives  essentially the same expression as CBOW
apart from the rescaling, which is often omitted due to computational efficiency in empirical works.

%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse The weighted PMI model  corresponds to weighted 
least square fit to SVD with matrix entries $  \mbox{PMI}(w, w')$; this is very analogous to classical VSM methods and was recently also suggested for analogy solving~\cite{levy2014linguistic}. We do not know if the  precise weighting $X_{w,w'}$ was explored before. 
\fi 

%Now we see how our model gives theoretical explanation for some earlier methods for finding semantic embeddings.
%This is the partial \textquotedblleft unification\textquotedblright hinted at earlier. 
\iffalse 


\paragraph{Relationship to VSMs.}  A popular method for constructing word vectors in information retrieval is to create a matrix 
whose $w, w'$ entry is $PMI(w, w')$ (we are simplifying the  description; the full method has columns corresponding to {\em contexts} which can
be words or sequences of words). The explicit vector for word $w$ is then the row corresponding to $w$. But this is very high dimensional,
and therefore practitioners reduce the dimension by  performing rank $d$ SVD
for smaller $d$, like 100.  In practice these low-dimensional vectors are very good, and quality is further improved by  reweighting the terms of the matrix. (We do not know if the  precise weighting used in our method was explored before.) Hitherto there was no theoretical 
justification for the efficacy of such dimension reduction via SVD. Our theory, and Corollary~\ref{cor:isotropic}, part (2), provides a nice explanation since it shows that the squared distance between the low-dimensional embeddings of words $a, b$ correspond exactly to $\sum_w \left(PMI(a, w) - PMI(b,w)\right)^2$, which is  the distance between the corresponding explicit vectors. 
\fi 





==> arxivjul22 copy/weight.tex <==
\section{Maximum likelihood estimator for co-occurrence} \label{sec:mlecooc}

Let $\LengthDocument$ be the corpus size, and $X_{w,w'}$ the number of times words $w, w'$ co-occur within a context of size $10$ in the corpus. According to the model, the probability of this event at any particular
time is $\log p(w,w')  \propto \nbr{v_{w} +  v_{w'}}_2^2.$ Successive samples from a random walk are not 
independent of course, but if the random walk mixes fairly quickly (and the mixing time of our random walk
is related to the {\em logarithm} of the number of words) then the 
set of $X_{w,w'}$'s over all word pairs is distributed  up to a very close approximation as a multinomial distribution $\mul(\tilde{L}, \{p(w,w')\})$ where $\tilde{L} = \sum_{w,w'} X_{w,w'}$ is the total number of word pairs in consideration (roughly $10 \LengthDocument$). 

Assuming this approximation, we show below that the maximum likelihood values for the word vectors correspond to the following optimization, 
\begin{align*}  
\min_{\cbr{v_w}, C} & \sum_{w,w'} X_{w,w'} \rbr{ \log(X_{w,w'}) - \nbr{v_{w}\!+\! v_{w'}}_2^2 - C}^2   \mbox{\qquad\qquad\qquad\qquad (Objective {\bf SN})}
\end{align*} 

Now we give the derivation of the objective.
According to the multinomial distribution, maximizing the likelihood of $\{X_{w,w'}\}$ is equivalent to maximizing
\begin{align*}
\ell & = \log\left(\prod_{(w, w')} p(w, w')^{X_{w,w'}} \right) = \sum_{(w, w')} X_{w,w'} \log p(w, w').
\end{align*}

To reason about the likelihood, denote the logarithm of the ratio between the expected count and the empirical count as
\begin{align*}
\Delta_{w,w'} = \log\left(\frac{\tilde{L} p(w, w')  }{ X_{w,w'} } \right).   
\end{align*}
Note that 
\begin{align}
 \ell & = \sum_{(w, w')} X_{w,w'}\log p(w, w')  \nonumber \\
& =  \sum_{(w, w')}  X_{w,w'} \left[\log\frac{X_{w,w'}}{\tilde{L}}  +   \log\left(\frac{\tilde{L} p(w, w')  }{ X_{w,w'} } \right) \right]  \nonumber \\
& =  \sum_{(w, w')}  X_{w,w'}  \log\frac{X_{w,w'}}{\tilde{L}}  +   \sum_{(w, w')}  X_{w,w'}  \log\left(\frac{\tilde{L} p(w, w')  }{ X_{w,w'} } \right)  \nonumber\\
& =  c  +   \sum_{(w, w')}   X_{w,w'}  \Delta_{w,w'} \label{eqn:likelihood_app}
\end{align}
where we let $c$ denote the constant $\sum_{(w, w')}  X_{w,w'}  \log\frac{X_{w,w'}}{\tilde{L}}$. 
Furthermore, we have 
\begin{align*}
\tilde{L} 
& = \sum_{(w,w')} \tilde{L} p_{w,w'} \\
& = \sum_{(w,w')} X_{w,w'} e^{\Delta_{w,w'} } \\
& = \sum_{(w,w')}  X_{w,w'} (1 + \Delta_{w,w'} + \Delta_{w,w'}^2/2 + O(|\Delta_{w,w'}|^3) )
\end{align*}
and also $\tilde{L} = \sum_{(w,w')} X_{w,w'}$. So
\begin{align*}
 \sum_{(w,w')}  X_{w,w'} \Delta_{w,w'}  =  - \left(\sum_{(w,w')}  X_{w,w'} \Delta_{w,w'}^2/2 + \sum_{(w,w')}  X_{w,w'} O(|\Delta_{w,w'}|^3) \right).
\end{align*}
Plugging this into (\ref{eqn:likelihood}) leads to
\begin{align}
c - \ell  = \sum_{(w,w')}  X_{w,w'} \Delta_{w,w'}^2/2 + \sum_{(w,w')}  X_{w,w'} O(|\Delta_{w,w'}|^3). \label{eqn:finalexpresion_app}
\end{align}

When the last term is much smaller than the first term on the right hand side, maximizing the likelihood is approximately equivalent to minimizing the first term on the right hand side, which is our objective:
\begin{align*}
\sum_{(w, w')}   X_{w,w'}  \Delta_{w,w'}^2 \approx \sum_{(w, w')}   X_{w,w'} \left(\|v_w + v_{w'} \|_2^2/(2d) - \log X_{w,w'} + \log\tilde{L} - 2\log Z \right)^2
\end{align*}
where $Z$ is the partition function.

We now argue that the last term is much smaller than the first term on the right hand side in (\ref{eqn:finalexpresion_app}). For a large $X_{w,w'}$, the $\Delta_{w,w'}$  is close to 0 and thus the induced approximation error is small. Small $X_{w,w'}$'s only contribute a small fraction of the final objective (\ref{eqn:finalexpresion}), so we can safely ignore the errors. 
%More precisely, when the approximation error terms of the Taylor expansions are all spelled out, in the final expression~\ref{eqn:finalexpresion}, we have an error term $\sum_{(w,w')}  X_{w,w'} O(|\Delta_{w,w'}|^3)$. 
To see this, note that the objective $\sum_{(w,w')}  X_{w,w'} \Delta_{w,w'}^2$ and the error term $\sum_{(w,w')}  X_{w,w'} O(|\Delta_{w,w'}|^3)$ differ by a factor of  $|\Delta_{w,w'}|$ for each $X_{w,w'}$. 
For large $X_{w,w'}$'s,  $|\Delta_{w,w'}| \ll 1$, and thus their corresponding errors are much smaller than the objective. So we only need to consider the $X_{w,w'}$'s that are small constants. The co-occurrence counts obey a power law distribution (see, e.g.~\cite{pennington2014glove}). That is, if one sorts $\{X_{w,w'}\}$ in decreasing order, then the $r$-th value in the list is roughly
$$
  x_{[r]} = \frac{k}{r^{5/4}}
$$ 
where $k$ is some constant. Some calculation shows that 
$$
  \tilde{L} \approx 4k, ~~ \sum_{X_{w,w'} \le x} X_{w,w'} \approx 4 k^{4/5} x^{1/5},
$$
and thus when $x$ is a small constant 
$$
  \frac{\sum_{X_{w,w'} \le x} X_{w,w'} }{\tilde{L}} \approx \left(\frac{4x}{\tilde{L}}\right)^{1/5} = O\left(\frac{1}{\tilde{L}^{1/5}} \right).
$$
So there are only a negligible mass of $X_{w,w'}$'s that are small constants, which vanishes when $\tilde{L}$ increases. Furthermore, we empirically observe that the relative error of our objective is $5\%$, which means that the errors induced by $X_{w,w'}$'s that are small constants is only a small fraction of the objective. Therefore, $\sum_{w,w'} X_{w,w'} O(|\Delta_{w,w'}|^3)$ is small compared to the objective and can be safely ignored.

%\yingyu{
%I have a question: why not just directly maximize the likelihood
        %$$\sum_{w,w'}  X_{w,w'} \log p(w,w')  $$
%This is approximately 
        %$$\sum_{w,w'}  X_{w,w'} (||v_w + v_{w'}||^2  - 2 \log Z )$$
%If we replace $\log Z$ with a variable $C$ to be learned, we get an objective function. However, optimizing it will make no sense since we can scale $v_w$ or choose arbitrarily small $C$ to make the objective arbitrarily large.
%In our current SN objective, we also replace $\log Z$ with a variable $C$. I'm a bit confused about why we don't have the same issues? 
%In other words,  do we know that optimizing the objective indeed gives something close to the ground truth (suppose we can optimize the objective to the optimum) ?
%}

\iffalse
In this section, we present a simple calculation to provide justification for the weighting in our training objective. Let $\LengthDocument$ to be the corpus size, and $W$ be the set of all words. We assume that the co-occurrence counts $X_{w, w'}$ for word pairs are generated according to a multinomial distribution $\mul(m, p(w,w')_{w,w'\in W})$. Denoting $\{X_{w,w'}\}$ the set of random variables corresponding to co-occurrence counts for all of the word pairs $(w,w')$ and $\{p_{w,w'}\}$ the set of corresponding probabilities, we show that $ \log \Pr[\{X_{w,w'}\}| \{p(w,w')\}]$ is of the form: %($\LengthDocument$ is the corpus size)
$$ \log \Pr[\{X_{w,w'}\}| \{p(w,w')\}] \approx C - \frac{1}{2\LengthDocument}\sum_{w, w'} X_{w,w'}\left(x_{w, w'}-\log(X_{w,w'})\right)^2 $$%+ \textrm{lower order terms}$$
where $C$ is a constant that depends on the data but not $\{p_{w,w'}\}$, $x_{w, w'} =\log(\LengthDocument p(w, w') )$, and the approximation ignores the lower order terms obtained from the Taylor expansion. 

More, precisely: 
\begin{thm} %[Weight]
Suppose the random variables $\{X_{w, w'}\}$ are generated from $ \mul(m, p(w,w')_{w,w'\in W})$. Then:  %is generated by i.i.d. each time sample  $(w,w')$ with probability $p_{w, w'}$ for $\LengthDocument$ times, then 
\begin{eqnarray*}
&&\log \Pr[\{X_{w, w'} \} \mid \{ p(w, w') \}] = C - \frac{1}{2\LengthDocument} \rbr{ \sum_{w, w' } X_{w, w'}(x_{w, w'} - \log X_{w, w'} )^2 } 
\\
&&+ O \left(  \frac{1}{\LengthDocument} X_{a, b}(x_{a, b} - \log X_{a, b})^2 +  \frac{1}{\LengthDocument}\sum_{w, w'} X_{w, w'}(x_{w, w'} - \log X_{w, w'} )^3 + \frac{1}{\LengthDocument^2} \left( \sum_{w, w'}X_{w, w'} (x_{w, w'} - \log X_{w, w'}  ) \right)^2 \right)
\end{eqnarray*}
where $x_{w, w'} =\log(\LengthDocument p(w, w') )$, and $C$ only depends on $X$ but not $p$, and $(a,b)$ is an arbitrary pair such that $X_{a,b} \neq 0$. Typically, the terms inside the big-oh are much smaller than $\frac{1}{2\LengthDocument} \left( \sum_{w, w' } X_{w, w'}(x_{w, w'} - \log X_{w, w'} )^2 \right) $. 

\end{thm}




\begin{proof}
For any pair $(a, b)$ such that $ X_{a, b} \not= 0$, it holds that:


 \begin{eqnarray*}
\log \Pr\sbr{\{X_{w, w'} \} \mid \{ p(w, w') \}} = \log\left( C_1  \left(\prod_{(w, w') \not= (a,b )}p(w,w')^{X_{w, w'}}\right) \left( 1- \sum_{(w, w') \not= (a,b )} p(w, w') \right)^{X_{a, b}} \right)
  \end{eqnarray*}

where $C_1$ is the number of documents of size $\LengthDocument$ such that co-occurence count of each $w, w'$ is $X_{w, w'}$. 

Substituting $ x_{w, w'} = \log[ \LengthDocument p(w,w')] $, we have: 
\begin{eqnarray}
\log \Pr\sbr{\{X_{w, w'} \} \mid \{ p(w, w') \} }  & = & \log C_1 -  \LengthDocument \log \LengthDocument +  \frac{1}{\LengthDocument}\left(\sum_{(w, w') \not= (a,b )} X_{w, w'}   x_{w, w'}  \right) \nonumber\\
& & + X_{a, b} \log  \left( 1- \sum_{(w, w') \not= (a,b )} p_{w, w'} \right) \label{eq:weight}
\end{eqnarray}
 
The last term can be expanded as follows. Let $\xi$ denote $O([x_{w, w'} - \log X_{w, w'} ]^3)$.
 \begin{eqnarray*}
&&  \log  \left( 1- \sum_{(w, w') \not= (a,b )} p_{w, w'} \right) \\
  &=& \log  \left( 1- \frac{1}{\LengthDocument}\sum_{(w, w') \not= (a,b )} e^{x_{w, w'}}  \right) 
  \\
  &=& \log  \left( 1- \frac{1}{\LengthDocument}\sum_{(w, w') \not= (a,b )}X_{w, w'} e^{x_{w, w'} - \log X_{w, w'} }  \right) 
  \\
  &=&  \log  \left( 1- \frac{1}{\LengthDocument}\sum_{(w, w') \not= (a,b )}X_{w, w'} \left(1 + [x_{w, w'} - \log X_{w, w'}  ]+ [x_{w, w'} - \log X_{w, w'} ]^2/2 + \xi\right)  \right) 
  \\
  &=& \log \left( X_{a, b} - \frac{1}{\LengthDocument} \sum_{(w, w') \not= (a,b )}X_{w, w'} \left([x_{w, w'} - \log X_{w, w'}  ]+ [x_{w, w'} - \log X_{w, w'} ]^2/2 + \xi\right)  \right)
  \\
  &=& \log X_{a, b} +  \log \left( 1- \frac{1}{\LengthDocument X_{a,b}} \sum_{(w, w') \not= (a,b )}X_{w, w'} \left([x_{w, w'} - \log X_{w, w'}  ]+ [x_{w, w'} - \log X_{w, w'} ]^2/2 + \xi\right)  \right)
  \\
  &=& \log X_{a, b}  - \frac{1}{\LengthDocument X_{a,b}} \sum_{(w, w') \not= (a,b )}X_{w, w'} \left([x_{w, w'} - \log X_{w, w'}  ]+ [x_{w, w'} - \log X_{w, w'} ]^2/2 + \xi\right)  
  \\
  && \quad + O\left(\frac{1}{\LengthDocument^2 X_{a,b}^2} \left(\sum_{(w, w') \not= (a,b )}X_{w, w'} (x_{w, w'} - \log X_{w, w'}  )\right)^2 \right).
 \end{eqnarray*}

Putting this into (\ref{eq:weight}), we get the final bound.
%\begin{eqnarray*}
%&& \log \Pr[\{X_{w, w'} \} \mid \{ x_{w, w'} \}] = C - \frac{1}{2\LengthDocument} \left( \sum_{w, w' } X_{w, w'}(x_{w, w'} - \log X_{w, w'} )^2 \right) 
%\\
%&&+ O \left(  \frac{1}{\LengthDocument} X_{a, b}(x_{a, b} - \log X_{a, b})^2  +\frac{1}{\LengthDocument}\sum_{w, w'} X_{w, w'}(x_{w, w'} - \log X_{w, w'} )^3 + \frac{1}{\LengthDocument^2} \left( \sum_{w, w'}X_{w, w'} (x_{w, w'} - \log X_{w, w'}  )\right)^2 \right)
%\end{eqnarray*}
\end{proof} 

\fi


%
%\section{Maximum Likelihood Estimator for log of Binomial Distribution}
%
%
%
%%To get the word embedding, several of the existing methods re-weight the concurrence during the training process. In this section we argue that this is because the ``measurement'' are noisy (i.e. we don't get the exact moments, but moments with some noise.)  
%
%
%%According to our generative model, we can assume that for every pair of words $w_i, w_j$, for every $t , \not= t' \in \N^*$, the events that we see word $(w_i, w_j)$ cooccur in position $t, t+1$ and position $t', t'+1$ in document $T$ are independent. Therefore, the cooccurence count $x_{i, j}$ of words $w_i$ and $w_j$ follows binomial distribution $\bin(\LengthDocument, p_{i, j})$ where $\LengthDocument$ is the size of the document. We have the following theorem: 
%
%In this section, we present a very simple calculation that show that the weight function $f_{w,w'}$ in GloVe makes sense. Concretely, we assume that the co-occurrence count $X_{w,w'}$ for words pair $w,w'$ is from binomial distribution $\bin(|T|, p(w,w'))$. We show that the likelihood of $\log X_{w,w'}$ given on $p(w,w') = x/|T|$ is of the form 
%$$C+ \frac{X_{w,w'}}{|T|- X_{w,w'}}\left(x-\log(X_{w,w'})\right)^2 + \textrm{high order term}$$
%where $C$ is a fixed constant (that depends on the data $X_{w,w'}$ but not $x$ or $p$. )
%
%\begin{thm} %[Weight]
%Suppose $X$ is from binomial distribution $\bin(m, p)$ with $p = x/m$, then we have that the likelihood of $X$ is of the form
%$$\Pr[X \mid p] = C+ \frac{X}{m- X}\left(x-\log(X)\right)^2 + O\left(\left(x-\log(X)\right)^3\right)$$
%where $x =\log(pm)$, and $C$ only depends on $X$ but not $p$ or $x$. 
%%Let $x_{i, j}, i , j\in [W]$ be independent random variables with $x_{i, j} \sim \bin(\LengthDocument, p_{i, j})$. Then the maximum likelihood estimator $y$ for $\{\log(\LengthDocument p_{i,j }) \}_{i, j \in [W]}$ is given by: 
%
%%$$\min_y \sum_{i, j} \left( \frac{x_{i, j}}{\LengthDocument - x_{i, j}} \right)\left( y_{i, j} - \log x_{i, j} \right)^2 +  O\left( \sum_{i, j}\left( y_{i, j} - \log x_{i, j} \right)^3 \right) $$
%\end{thm}
%
%
%
%\begin{proof}
%
%Let $X \sim \bin(\LengthDocument, p)$, then we know that the probability mass is $\Pr[X = k\mid p] =  { \LengthDocument \choose k} (1 - p)^{\LengthDocument - k} p^k, k \in \{ 0, 1, ..., \LengthDocument \}$. 
%
%Therefore, the log-likelihood is given by: 
%$$\log \Pr[X = k\mid p]=  \log { \LengthDocument \choose k}  + (\LengthDocument - k) \log (1 - p) + k \log p, k \in \N$$
%
%
%Let $x = \log (\LengthDocument p)$, we have: for $k \in \N$,
%$$  \log \Pr[X = k\mid p] =   \log { \LengthDocument \choose k}  + (\LengthDocument - k) \log  \left(1 - \frac{e^x}{\LengthDocument} \right) + k \log  \frac{e^x}{\LengthDocument}$$
%
%We take the Taylor expansion w.r.t $x$ at point $\log k$, and conclude
%$$ \log \Pr[X = k\mid p]   = \log { \LengthDocument \choose k}    - \frac{k  \LengthDocument }{2 (\LengthDocument - k)} (x - \log k)^2 + \LengthDocument O\left((x - \log k)^3 \right)$$
%
%
%%Therefore, we know $\log$ of the joint distribution of $x_{i, j}$ are given by
%%$$ \log F = \sum_{i, j} \log f_{p_{i, j}} (x_{i, j}) = \sum_{i, j} \left(  \log { \LengthDocument \choose x_{i, j}}  - \frac{ x_{i, j}  \LengthDocument }{2 (\LengthDocument -  x_{i, j})} (y_{i, j} - \log  x_{i, j})^2 + \LengthDocument O\left((y_{i, j} - \log  x_{i, j})^3 \right) \right)$$
%
%
%%Therefore, we need to find $y$ to minimize
%%$$\min_y \sum_{i, j} \left( \frac{x_{i, j}}{\LengthDocument - x_{i, j}} \right)\left( y_{i, j} - \log x_{i, j} \right)^2 -  O\left( \sum_{i, j}\left( y_{i, j} - \log x_{i, j} \right)^3 \right) $$
%
%%Let take taylor expansion 
%%$$\frac{d \log f_p(k)}{d y} =  \frac{ \LengthDocument(k - e^y)}{\LengthDocument - e^y} = \LengthDocument  \frac{1 - e^{y - \log k}}{\frac{\LengthDocument}{k} - e^{y - \log k}}   = \LengthDocument \left( \frac{y - \log k}{1 - \frac{\LengthDocument}{k}} + O\left((y - \log k)^2\right) \right)$$
%%
%%
%%We have a maximum likelihood estimator $y$ for $\{ \log(\LengthDocument p_{i, j}) \}$:
%%$$\argmin_y \sum_{i, j} \left(\frac{d \log f_{p_{i, j}}(x_{i, j})}{d y_{i, j}} \right)^2 = \argmin_y \sum_{i, j} \left( \frac{x_{i, j}}{\LengthDocument - x_{i, j}} \right)^2\left( y_{i, j} - \log x_{i, j} \right)^2 +  O\left( \sum_{i, j}\left( y_{i, j} - \log x_{i, j} \right)^3 \right) $$
%
%
%\end{proof}



 
%\end{document}

==> arxivjul22 copy/zc.tex <==
%!TEX root = supplementary.tex
\subsection{Analyzing partition function $Z_c$}\label{sec:zc}

In this section, we prove Lemma~\ref{thm:Z_c}. We basically first prove that for the means of $Z_c$ are all $(1+o(1))$-close to each other, and then prove that $Z_c$ is concentrated around its mean. It turns out the concentration part is non trivial because the random variable of concern, $\expinner{v_w,c}$ is not well-behaved in terms of the tail. Note that $\expinner{v_w,c}$ is NOT sub-gaussian for any variance proxy. %\Anote{The previous sentence is a little vague. I think just saying the tail is not well-behaved is saying enough... }
This essentially disallows us to use an existing concentration inequality directly. We get around this issue by considering the truncated version of $\expinner{v_w,c}$, which is bounded, and have similar tail properties as the original one, in the regime that we are concerning. 

We bound the mean and variance of $Z_c$ first in the Lemma below. 
%we prove that under our assumption, $Z_c$ are all $1+ \epsilon_z$-close to each other 

%\begin{thm}\label{thm:Z_c}
%	There exists $Z$ such that for any context $c$, with high probability $(1-4\exp(-d^{0.8}))$ over the choice of $v_w$'s, $Z_c$ is close $Z$: 
%	
%	$$(1-\epsilon_z)Z\le Z_c\le (1+\epsilon_z) Z $$%\ge 1 - 2e^{- 2n^{0.4}}$$
%	with $\epsilon_z = o(1)$.
%\end{thm}




\begin{lem}\label{lem:exp_var_Z_c}
	For any fixed unit vector $c\in \R^d$,  we have that $\Exp[Z_c]\ge n$ and $\mathbb{V}[Z_c] \le O(n)$. 
\end{lem}

\begin{proof}[Proof of Lemma~\ref{lem:exp_var_Z_c}]
		%\Tnote{Spherical Gaussian distribution should mean Gaussian with variance $I$. }
		%\Anote{What is this referring to?} 
		
		Recall that by definition $$Z_c = \sum_{w}\exp(\langle v_w, c\rangle).$$ We fix context $c$ and view $v_w$'s as random variables throughout this proof. %For convenience, we denote the norm of $c$ by  $\ell = \|c\|$.  
		Recall that $v_w$ is composed of $v_w = s_w \cdot \hat{v}_w$, where $s_w$ is the scaling and $\hat{v}_w$ is from spherical Gaussian with identity covariance $I_{d\times d}$. Let $s$ be a random variable that has the same distribution as $s_w$.  %and thus almost a unit vector. 
	
	%We calculate the mean of $Z_c$ as follows: 
	%Just as a warm-up, 
	We lowerbound the mean of $Z_c$ as follows: 
	
	$$\Exp[Z_c] =n\Exp\left[\exp(\langle v_w,c\rangle)\right]\ge n\Exp\left[1+\langle v_w,c\rangle\right] = n$$
	where the last equality holds because of the symmetry of the spherical Gaussian distibution.  
	On the other hand, to upperbound the mean of $Z_c$, we  condition on the scaling $s_w$, 
	\begin{align*}
		\E[Z_c] &= n\Exp[\exp(\langle v_w, c\rangle)] \\
		&=n \Exp\left[\Exp\left[\exp(\langle v_w, c\rangle)\mid s_w\right]\right]
	\end{align*}
	
	Note that conditioned on $s_w$, we have that $\langle v_w, c\rangle$ is a Gaussian random variable with variance %$\sigma^2 = \|c\|^2 s_w^2 = \ell^2 s_w^2$. 
	$\sigma^2 = s_w^2$. Therefore,
	\begin{align*}
		\Exp\left[\exp(\langle v_w, c\rangle)\mid s_w\right] &= \int_x \frac{1}{\sigma\sqrt{2\pi}} \exp(-\frac{x^2}{2\sigma^2}) \exp(x)dx \\
		&=\int_x \frac{1}{\sigma\sqrt{2\pi}} \exp(-\frac{(x-\sigma^2)^2}{2\sigma^2} + \sigma^2/2)dx \\
		&= \exp(\sigma^2/2) 
	\end{align*} 
	
	%It follows that $$\Exp[Z_c] = n\Exp[\exp(\sigma^2/2) ] = n\Exp[\exp(s_w^2\ell^2/2)]= n\Exp[\exp(s^2\ell^2/2)].$$
	
	It follows that $$\Exp[Z_c] = n\Exp[\exp(\sigma^2/2) ] = n\Exp[\exp(s_w^2/2)]= n\Exp[\exp(s^2/2)].$$
	%	
	%	Let $Z: = n\Exp[\exp(s^2/{2d})]$. By Proposition~\ref{prop:cnorm}, we have that $1-o(d^{-0.4})\le \|c\| \le 1+o(d^{-0.4})$. Therefore, for any $c$, 
	%	$$\Exp[Z_c] = n\Exp[\exp(s^2\|c\|^2/{2d})]\le n\Exp[\exp(s^2/2d) \cdot \exp(o(d^{-0.4})s^2/{2d})] \le n(1+o(d^{-0.4})\kappa^2/2)Z = (1+o(1))Z$$
	%	where the last inequality follows from the fact that $e^x \leq 1+2x$ for $x = o(1)$, and the absolute bound on $\|s\|$ in terms of $\kappa$. Similarly we can prove that $\Exp[Z_c] \ge (1-o(1))Z$ for any $c$.  %\le \Exp[\exp(s_w^2/d)]\le 1+o(1).$$
	%	%where we use the assumption (\ref{eqn:epsilon1}) in the last inequality. 
	%%	
	%%	
	%%	Therefore, we have that 
	%%	
	%%	
	%%	\begin{align*}
	%%	\E[Z_c] &=n \Exp\left[\Exp\left[\exp(\langle v_w, c\rangle)\mid s_w \right]\right]\\
	%%	& = n\Exp\left[\exp(\sigma^2/2)\right] =  n\Exp\left[\exp(\ell^2\|s_w\|^2/(2d))\right]
	%%	\end{align*}
	%	
	
	We calculate the variance of $Z_c$ as follows: 
	
	\begin{align*}
		\mathbb{V}[Z_c] & = \sum_w\mathbb{V}\left[\exp(\langle v_w, c\rangle)\right] \le n\Exp[\exp(2\langle v_w, c\rangle)] \\
		&=n \Exp\left[\Exp\left[\exp(2\langle v_w, c\rangle)\mid s_w\right]\right]
	\end{align*}
	By a very similar calculation as above, using the fact that $2\langle v_w,c\rangle$ is a Gaussian random variable with variance %$4\sigma^2 = 4\ell^2 s_w^2$, 
	$4 \sigma^2 = 4 s_w^2$, 
	%Note that conditioned on $s_w$, we have that $\langle v_w,c\rangle$ is a guassian random variable with variance $\sigma^2 = \ell^2 \|s_w\|^2/d$. Therefore,
	\begin{align*}
		\Exp\left[\exp(2\langle v_w, c\rangle)\mid s_w\right] %&= \int_x \frac{1}{\sigma\sqrt{2\pi}} \exp(-\frac{x^2}{2\sigma^2}) \exp(2x)dx \\
		%&=\int_x \frac{1}{\sigma\sqrt{2\pi}} \exp(-\frac{(x-2\sigma^2)^2}{2\sigma^2} + 2\sigma^2)dx \\
		&= \exp(2\sigma^2) 
	\end{align*} 
	
	
	
	
	Therefore, we have that 
	
	
	%\begin{align*}
	%	%		\E[(Z_c-\E Z_c)^2]
	%	\mathbb{V}[Z_c]&\le n \Exp\left[\Exp\left[\exp(2\langle v_w, c\rangle)\mid s_w \right]\right]\\
	%	& = n\Exp\left[\exp(2\sigma^2)\right] =  n\Exp\left[\exp(2\ell^2s^2)\right]\le \Lambda n
	%\end{align*}
	
	\begin{align*}
		%		\E[(Z_c-\E Z_c)^2]
	\mathbb{V}[Z_c]&\le n \Exp\left[\Exp\left[\exp(2\langle v_w, c\rangle)\mid s_w \right]\right]\\
	& = n\Exp\left[\exp(2\sigma^2)\right] =  n\Exp\left[\exp(2s^2)\right]\le \Lambda n
  \end{align*}
	
	for $\Lambda = \exp(8 \kappa^2)$ a constant, and at the last step we used the facts that $s\le \kappa$ a.s.
\end{proof}

Now we are ready to prove Lemma~\ref{thm:Z_c}. 
\begin{proof}[Proof of Lemma~\ref{thm:Z_c}]
	
	We fix the choice of $c$, and the proving the concentration using the randomness of $v_w$'s first. 
		Note that that $\exp(\langle v_w,c\rangle) $ is neither sub-Gaussian nor sub-exponential (actually the Orlicz norm of random variable $\exp(\langle v_w,c\rangle) $ is never bounded).
		%\Anote{Not sure how well-known Orlicz norms are... I actually had to look this up :) } 
		This prevents us from applying the usual concentration inequalities. The proof deals with this issue in a slightly more specialized manner. 
		
		Let's define $\mathcal{F}_w$ be the event that $|\langle v_w,c\rangle|\le \frac{1}{2}\log  n$. %for some small constant $\eta > 0$ (e.g. $\eta = 0.001$ will suffice). 
		We claim that $\Pr[\mathcal{F}_w] \ge 1-\exp(-\Omega(\log^2n))$. Indeed note that $\inner{v_w}{c} \mid s_w$ has a Gaussian distribution with standard deviation 
		%$s_w\|c\| = s_w \ell \le 2\kappa$ a.s. \Anote{This should be $\frac{s_w \|c\|}{\sqrt{d}}$ no? } \Tnote{see notes in the beginning of Thoerem 1}%\Tnote{Sphereical Gaussian means }
		$s_w \|c\| = s_w \leq 2\kappa$ a.s. 
		Therefore by the Gaussianity of $\inner{v_w}{c}$ we have that $$\Pr[|\langle v_w,c\rangle|\ge \eta \log  n\mid  s_w]\le 2\exp(-\Omega(\frac{1}{4}\log^2 n/\kappa^2)) = \exp(-\Omega(\log^2 n)),$$
		where $\Omega(\cdot)$ hides the dependency on $\kappa$ which is treated as absolute constants. 
		%\Anote{This is as far as I've gotten with careful reading.} 
		Taking expectations over $s_w$, we obtain that  $$\Pr[\mathcal{F}_w ]  = \Pr[|\langle v_w,c\rangle|\le \frac 1 2 \log  n]\ge 1- \exp(-\Omega(\log^2 n)).$$
		 Note that by definition, we in particular have that conditioned on $\mathcal{F}_w$, it holds that $\exp(\inner{v_w}{c})\le \sqrt{n}$. 
		
		
		%Observe that $\mathcal{F}$ is a very high probability event with $\Pr[\mathcal{F}_w] \ge 1- \exp(-d^{0.2}/\kappa^2)$ . 
		Let the random variable $X_w$ have the same distribution as $\exp(\langle v_w,c\rangle) \vert_{\mathcal{F}_w}$. We prove that the random variable $Z'_c = \sum_{w}X_w$ concentrates well.  By convexity of the exponential function, we have that the mean of $Z_c'$ is lowerbounded
		
		$$\Exp[Z_c'] =n\Exp\left[\exp(\langle v_w,c\rangle)\vert_{\mathcal{F}_w}\right]\ge n\exp( \Exp \left[\langle v_w,c\rangle \vert_{\mathcal{F}_w} \right])= n$$
		
		and the variance is upperbounded by 
		
		\begin{align*}
		\mathbb{V} [Z_c'] &\le n\Exp\left[\exp(\langle v_w,c\rangle)^2\vert_{\mathcal{F}_w}\right] \\
		&\le \frac{1}{\Pr[\mathcal{F}_w]} \Exp\left[\exp(\langle v_w,c\rangle)^2\right] \\
		&\le  \frac{1}{\Pr[\mathcal{F}_w]}\Lambda n \le 1.1 \Lambda n
		\end{align*}
		
		where the second line uses the fact that 
		\begin{eqnarray*}
		\Exp\left[\exp(\langle v_w,c\rangle)^2\right]  &&= \Pr[\mathcal{F}_w]\Exp\left[\exp(\langle v_w,c\rangle)^2\vert {\mathcal{F}_w}\right] + \Pr[\overline{\mathcal{F}}_w]\Exp\left[\exp(\langle v_w,c\rangle)^2\vert {\overline{\mathcal{F}}_w}\right] \\
		&& \ge \Pr[\mathcal{F}_w]\Exp\left[\exp(\langle v_w,c\rangle)^2\vert {\mathcal{F}_w}\right]. 
		\end{eqnarray*}
		
		Moreover, by definition, for any $w$, $|X_w|\le \sqrt{n}$. Therefore by Bernstein's inequality, we have that 
		$$\Pr\left[|Z_c' -\Exp[Z_c']| > \epsilon n \right]\le \exp(-\frac{\frac{1}{2}\epsilon^2 n^2}{1.1\Lambda n + \frac{1}{3}\sqrt{n}∑\cdot \epsilon n})$$
		%\Anote{Since we put constants in the second term ($1/3$ ...), maybe we should make the first term $1.1 \Lambda n$?} 
		
		
		Note that $\Exp[Z_c']\ge n$, therefore for $\epsilon \gg \frac{\log^2 n}{\sqrt{n}}$, we have, %we have that for $\epsilon = 1/\log n$, 
				\begin{align}
					\Pr\left[|Z_c' -\Exp[Z_c']| > \epsilon \Exp[Z_c']\right] & \le \Pr\left[|Z_c' -\Exp[Z_c']| > \epsilon n \right] \le \exp(-\frac{\frac{1}{2}\epsilon^2 n^2}{\Lambda n + \frac{1}{3}\sqrt{n}\cdot \epsilon n})\nonumber \\
					& \le \exp(-\Omega(\min\{  \epsilon^2n/\Lambda, \epsilon \sqrt{n}\})) \nonumber\\
					& \le \exp(-\Omega(\log^2 n)) \nonumber
				\end{align}
				
					% \exp(-\Omega(\log^2 n)), $$
			%where we used the fact that $1 > \eta > 0$ is a fixed constant and $\Lambda$ is also a constant.  
			%	\Tnote{Constant maybe a bit wrong}
				
		Let $\mathcal{F} = \cup_w \mathcal{F}_w$ be the union of all $\mathcal{F}_w$. Then by union bound, it holds that $\Pr[\bar{\mathcal{F}}]\le \sum_{w}\Pr[\bar{\mathcal{F}_w}] \le n\cdot \exp(-\Omega(\log^2n)) = \exp(-\Omega(\log^2n))$.  We have that by definition, $Z_c'$ has the same distribution as $Z_c\vert_{\mathcal{F}}$. Therefore, we have that 
		
		\begin{equation}
		\Pr[|Z_c -\Exp[Z_c']| > \epsilon \Exp[Z_c']\mid \mathcal{F}]\le \exp(-\Omega(\log^2 n)) \label{eqn:eqn12}
		\end{equation}
		
		and therefore
				\begin{align}
					\Pr[|Z_c -\Exp[Z_c']| > \epsilon  \Exp[Z_c']] &= \Pr[\mathcal{F}]\cdot \Pr[|Z_c -\Exp[Z_c']| > \epsilon  \Exp[Z_c']\mid \mathcal{F}] + \Pr[\bar{\mathcal{F}}]  \Pr[|Z_c -\Exp[Z_c']| > \epsilon  \Exp[Z_c']\mid \bar{\mathcal{F}}] \nonumber\\
					& \le \Pr[|Z_c -\Exp[Z_c']| > \epsilon  \Exp[Z_c']\mid \mathcal{F}]  + \Pr[\bar{\mathcal{F}}] \nonumber\\
					& \le \exp(-\Omega(\log^2n)) \label{eqn:eqn13}
					\end{align}
			where at the last line we used the fact that $\Pr[\bar{\mathcal{F}}]\le\exp(-\Omega(\log^2n))$ and equation~\eqref{eqn:eqn12}. 
			
			Let $Z =  \Exp[Z_c'] =  \Exp[\exp(\inner{v_w}{c})\mid |\inner{v_w}{c}| < \frac{1}{2}\log n]$ (note that $\Exp[Z_c']$ only depends on the norm of $\|c\|$ which is equal to 1). Therefore we obtain that with high probability over the randomness of $v_w$'s, 
			
			\begin{equation}
				(1-\epsilon_z)Z\le Z_c\le (1+\epsilon_z)Z\label{eqn:lem_zc_proof}
			\end{equation}
			Taking expectation over the randomness of $c$, we have that 
			\begin{equation*}
			\Pr_{c,v_w}[\textrm{~\eqref{eqn:lem_zc_proof} holds} ]\ge 1-\exp(-\Omega(\log^2 n))
			\end{equation*}
			
			Therefore by a standard averaging argument (using Markov inequality), we have 
			\begin{equation*}
			\Pr_{v_w}\left[\Pr_c[\textrm{~\eqref{eqn:lem_zc_proof} holds} ]\ge 1-\exp(-\Omega(\log^2 n))\right] \ge 1-\exp(-\Omega(\log^2 n))
			\end{equation*}
			For now on we fix a choice of $v_w$'s so that $\Pr_c[\textrm{~\eqref{eqn:lem_zc_proof} holds} ]\ge 1-\exp(-\Omega(\log^2 n))$ is true. Therefore in the rest of the proof, only $c$ is random variable, and with probability $1 - \exp(-\Omega(\log^2 n))$ over the randomness of $c$, it holds that, 
			%which says that there exists $Z$ such that, with probability $1 - \exp(-\Omega(\log^2 n))$, 
			\begin{equation}
			(1-\epsilon_z)Z\le Z_c\le (1+\epsilon_z)Z. \label{eqn:good}
			\end{equation}
			%where $\epsilon_
			
			
	
	\iffalse
	Finally we show that $\Exp[Z_c']$ are close to each other as well. We take $c$ that satisfies that $\|c\| = 1 \pm o(d^{-0.4})$. %and $\|c_2\| = 1 \pm d^{-0.1}$, 
	Observe that consider $\Exp[Z_{c}'] = n\Exp[\expinner{v,c}\vert \mathcal{E}]$ %and $\Exp[Z_{c_2}'] = \Exp[\expinner{v,c_2}\vert \mathcal{F}]$, 
	, where $v$ is from the same distribution where $v_w$ is generated, and $\mathcal{E}$ is the event that $|\inner{v}{c}|\le \eta \log n$.  %and $\expinner{v,c_2}\le d^{0.2}\|c_2\|$. 
	Note that random variable $\expinner{v,c}\vert \mathcal{E}$ only depends on the length of $c$.  Therefore we have that  
	$\Exp[Z_{c}'] = n\Exp[\expinner{v,\|c\|z}\vert \mathcal{E}]$, %nd $\Exp[Z_{c_2}'] = \Exp[\expinner{v,\|c_2\|z}\vert \mathcal{F}]$, 
	where $z$ is any unit vector in the space. Then we have  %and $\mathcal{F}'$ is the event that $\expinner{v,z}\le d^{0.2}$. %and  $\mathcal{F}_2$ is the event that $\expinner{v,z}\le d^{0.2}\|c_2\|$Therefore we have that 
	\begin{eqnarray}
	\Exp[Z_{c}'] &&\le n\Exp[\expinner{v,\|c\|z}\vert \mathcal{E}] \le n\Exp[\expinner{v,z}\vert \mathcal{E}] \sup \{\expinner{v,(\|c\|-1)z}\vert \mathcal{E}\}\nonumber \\
	&&= \Exp[\expinner{v,\|c\|z}\vert \mathcal{E}] \exp(d^{-0.4}\cdot n^{\eta})\nonumber \\
	&& = n(1+o(1)) \Exp[\expinner{v,\|c\|z}\vert \mathcal{E}] \label{eqn:eqn15}
	\end{eqnarray}
	
	where the last line uses the fact that $d > n^{.01}$, and $\eta$ is small enough constant. 
	
	Similarly we can prove that 
	
		\begin{eqnarray}
		\Exp[Z_{c}'] &&\ge n\Exp[\expinner{v,\|c\|z}\vert \mathcal{E}] \le n\Exp[\expinner{v,z}\vert \mathcal{E}] \inf \{\expinner{v,(\|c\|-1)z}\vert \mathcal{E}\}\nonumber \\
		&&= n\Exp[\expinner{v,\|c\|z}\vert \mathcal{E}] \exp(-d^{-0.4}\cdot n^{\eta}) \nonumber\\
		&& = n(1-o(1)) \Exp[\expinner{v,\|c\|z}\vert \mathcal{E}] \label{eqn:eqn14}
		\end{eqnarray}
%		\begin{eqnarray}
%		\Exp[Z_{c_1}'] %&&\le \Exp[\expinner{v,\|c\|z}\vert \mathcal{F}'] \le \Exp[\expinner{v,z}\vert \mathcal{F}'] \sup \{\expinner{v,(\|c\|-1)z}\vert \mathcal{F}'\} \\
%		%&&= \Exp[\expinner{v,\|c\|z}\vert \mathcal{F}'] \exp(d^{-0.2}) \\
%		&& \ge (1-o(1)) \Exp[\expinner{v,\|c\|z}\vert \mathcal{F}'] 
%		\end{eqnarray}
		
		Therefore, let $Z = n\Exp[\expinner{v,\|c\|z}\vert \mathcal{E}] $, we have by equation~\eqref{eqn:eqn14} and~\eqref{eqn:eqn15} that for $c$ with $\|c\| = 1 \pm o(d^{.4})$, we have that $\Exp[Z_c'] = (1\pm o(1))Z$. Recall that by equation~\eqref{eqn:eqn13}, we have that
		$\Pr[Z_c = (1\pm \epsilon)\Exp[Z_c']] \ge 1- \exp(-\Omega(\log^2 n))$. Therefore altogether we obtain that for $c$ with $\|c\| = 1\pm o(d^{.4})$, 		$\Pr[Z_c = (1\pm \epsilon)Z] \ge 1- \exp(-\Omega(\log^2 n))$, for $\epsilon =  1/\log n$, as desired. 
%			$$\Exp[Z_c'] =n\E$xp\left[\exp(\langle v_w,c\rangle)\vert \mathcal{F}_w\right]\ge n\Exp\left[1+\langle v_w,c\rangle\vert \mathcal{F}_w\right] = n$$
%			
%		\Tnote{}
%		On the other hand, we upper bound $\Exp[Z_c']$ by relating $\Exp[Z_c]$ and $\Exp[Z_c']$. 
%		$$\Exp[Z_c']\le \frac{1}{\Pr[\mathcal{F}]}\Exp[Z_c] \le (1 + o(1)). $$
%		
%		Therefore, let $Z= n$ and we have that 
%		$$\Pr[|Z_c -n| > (1+o(1))n] \le \Pr[Z_c - \Exp[Z_c']]\le 2e^{- 2n^{0.4}} $$
		
		
		%Let $\mu = \Exp\left[Z_c\right]$.  Observe that $\mu \ge n$ We also checked that indeed $\langle v_w,c \le $ 
	
	%We lowerobund $Z_c$ first by using the fact that $\exp(x)\ge 1+x+x^2/2$ for $x\ge 0$, 
%	
%	\begin{align*}
%		Z_c &\ge \sum_{w\in W}\left( 1 + \langle v_w,c\rangle + \frac{1}{2}\langle v_w,c\rangle^2\right) \\
%		&= n + \langle\sum_{w} v_w , c\rangle + \frac{1}{2}c^T \left(\sum_{w}v_wv_w^T\right) c \\
%		& \ge n + \frac{\gamma n}{2}\|c\|^2
%		\end{align*}
%		where we used the assumptions that $v_w$'s are centered and $v_w$'s are at isotropic position. 

%Now, recall that  $\E[Z_c ]= \E[\exp(s^2 \|c^2 \| / 2d)]$ with $s \le \kappa \sqrt{d}$. Therefore, for $c$ and $c'$ such that $| \| c\| - 1 | <  d^{- 0 . 1}; | \| c'\| - 1 | <  d^{- 0 . 1}$, we have $\frac{\E[Z_c]}{\E[Z_{c'}]} \le \exp(\kappa^2 d^{- 0 .1} ) = o(1)$. Putting together, we get that with probability $1 - 2\exp(-2n^{0.4}) - 2 \exp(-d^{0.8}) \ge 1 - 4 \exp(-d^{0.8})$ (by assumption $d < n^{0.5}$), 

%$$(1-\epsilon_z)Z\le Z_c\le (1+\epsilon_z) Z $$%\ge 1 - 2e^{- 2n^{0.4}}$$
	%with $\epsilon_z = o(1)$.
	\fi
	\end{proof}
%
%\begin{prop}\label{prop:cnorm}
%	When $c\sim \mathcal{C}$ is at stationary distribution of the random walk, we have that 
%	$$\Pr_{c\sim \mathcal{C}}\left[\left|\|c\| - 1\right| > 2d^{-0.4}\right] \le2 \exp(-d^{0.2})$$
%\end{prop}
%\begin{proof}
%	By assumption, each coordinate of $c$ is independent with $\E [c_i^2] = \frac{1}{d}$ and $|c_i|^2 \le \frac{4}{d}$, so the Proposition \ref{prop:cnorm} follows from standard Chernoff bound. 
%\end{proof}


